Computation and Bribery of Voting Power in Delegative Simple Games

Following Zhang and Grossi~(AAAI 2021), we study in more depth a variant of weighted voting games in which agents' weights are induced by a transitive support structure. This class of simple games is notably well suited to study the relative importance of agents in the liquid democracy framework. We first propose a pseudo-polynomial time algorithm to compute the Banzhaf and Shapley-Shubik indices for this class of game. Then, we study a bribery problem, in which one tries to maximize/minimize the voting power/weight of a given agent by changing the support structure under a budget constraint. We show that these problems are computationally hard and provide several parameterized complexity results.

==> Contribution/DynamicProgramming/banzafindex.tex <==

\section{Banzhaf Index}


In what follows, we provide a dynamic programming approach to compute the Banzaf index in polynomial time when voters all start with weight one. 


\begin{theorem}\label{thShBaPolynomial}
Given a delegative simple game of $V=<N, d, q>$ and a voter $i \in N$, $DB_i$ can be computed in $O(n^3)$, respectively. 
\end{theorem}

\begin{proof}

We decompose the proof in two sub-cases : 

\paragraph{Case 1: voter $n$ is a guru.} 
Consider a guru $n$ with weight $w_d(n)$. For every $k \in \{0, ..., w_d(n)-1\}$, let $T_d(n,k)$ be the set of all subtrees $T$ rooted in $n$ such that $|T|=k+1$, i.e., each subtree $T \in T_d(n,k)$ represents a possible way that $n$ obtains a weight $k+1$ by getting $k$ delegations. It is worth noticing that there may be more than one subtree $T \in T_d(n,k)$ in which voter $n$ receives weight $k+1$. For instance, in Example~\ref{exNotations}, $T_d(8)$ has two subtrees with weight $3$ and rooted in $8$ : the first (resp. second) subtree is composed of vertices in $\{6,7,8\}$ (resp. $\{4,7,8\}$). Given a sub-tree $T$, let $ch(T)$ be the set of children of nodes in $T$. To compute $DB_n$, we need to compute, for every $T \in T_d(n,k)$, $N^k(T)$ the number of subsets of $N\setminus (T \cup ch(T))$ that have weight in $\{q-k-1, ..., q-1\}$, where $k=0, ..., w_n-1$. More formally,  for every $T \in T_d(n,k)$, we have 

$$N^k(T)=\sum_{\substack{C\subseteq N\setminus (T \cup ch(T))}} \mathbbm{1}_{q-k-1 \le w_{d}(C) \le q-1},$$

where $\mathbbm{1}_{\phi}$ is equal to $1$ if $\phi$ is true, and $0$ otherwise. %Note that for every $j\in C$, if $j$ is an active agent in $C$, $w(j)=1$, otherwise $w(j)=0$. Furthermore, each voter $j\in T_d(n)\setminus T$ could only join $C$ as inactive voter except when $k\ge q$. It means that when $k\ge q$, voters in $T_d(n)\setminus T$ could join $C$ as active or inactive agents. We highlight this point later. 
Let $N^k =\sum_{T \in T_d(n,k)} N^k(T)$. %\sum^{w_n}_{k=1}\sum_{T \in T_d(n,k)} N^k_s(T)$. 
Now we can compute the $DB_n$ as follows. 

\begin{align}\label{alignShapely}
    DB_n = \frac{1}{2^{n-1}}\sum_{k=0}^{w_d(n)-1}N^k.
\end{align}

Let $t_j=|T_d(j)|$, i.e., the size of the tree $T_d(j)$ rooted in $j$. 
Moreover, let $Anc(j)$ be the set of ancestors of $j$ in the delegation graph.
To compute $DB_n$ efficiently, we use a dynamic programming approach. 
Given a forest $\mathcal{F}$ with $n$ vertices, we define a table $X_{\mathcal{F}}$ where $X_{\mathcal{F}}[j, w]$ is the number of sets $C\subset \{1,...,j\}$ such that $w_d(Anc(j)\cup C) = w_d(Anc(j)) + w$, where $j$ range from $0$ to $n$ and $w$ ranges from $0$ to $n$. In words, we count the number of subsets in $\{1,...,j\}$ who will contribute a weight $w$ when added to a coalition containing all ancestors of $j$. This table entries will be filled as follows.

First, for $j=0$, we have
\begin{align*}
X_{\mathcal{F}}[0, w] \!=\! \left\{ \begin{array}{c c}
1 & \text{ if } w= 0\\
0 & \text{ otherwise.}
\end{array} \right.
\end{align*}
%More generally, $X_{\mathcal{F}}[j, w] = 0$ if $s > j$ or $w > s$. Second, if $s = 0$, then $F_{\mathcal{F}}[j, w, s] = 0$ if $w > 0$ and $1$ otherwise.
In the special case $w=0$, we have
\begin{align}\label{alignWZeroVoters}
         X_{\mathcal{F}}[j, 0]&=\sum_{x = 0}^{ t_j-1} {t_j-1 \choose x}X_{\mathcal{F}}[j - t_j, 0]
\end{align}

Now for $j=1,\ldots, n$, and $w=1, \ldots, q-1$, $F[j, w]$ will be computed as follows.

\begin{equation}\label{eqRecursiveFB}
      \begin{split}
         X_{\mathcal{F}}[j, w]&=\sum_{x = 0}^{ t_j-1} {t_j - 1 \choose x}X_{\mathcal{F}}[j - t_j, w]\\&+ X_{\mathcal{F}}[j-1,w-1]
      \end{split}
\end{equation}
We recall that $X_{\mathcal{F}}[j, w]$ is the number of sets $C\subset \{1,...,j\}$ such that $w_d(Anc(j)\cup C) = w_d(Anc(j)) + w$. Here, the two summands correspond to the cases $j\notin C$ and $j\in C$ respectively.  Note that in the first case, successors of $j$ can only join $C$ as inactive agents. Hence in the first summand, we consider all possible ways of adding to $C$ inactive agents from the tree rooted in $j$ before moving to the next subtree (rooted in $j - t_j$).

We use this dynamic programming equations considering two forests $\mathcal{F}_1 = \{T_d(n)\}$ and $\mathcal{F}_2 = H_d - T_d(n)$ of sizes $n$ and $n-t_n$, respectively. We conclude by noticing that:
\begin{equation}
N^k = \sum_{w = q-k-1}^{q-1} X_{\mathcal{F}_2}[n-t_n,w] (X_{\mathcal{F}_1}[t_n,k]).\label{eq:Nk computation}
\end{equation}

\paragraph{Case 2: voter $n$ is a delegator.}
If $n$ is a delegator, then $n$ can only be a swing agent for coalition $C$ if $Anc(n) \subseteq C$. 
Hence, we should count only coalitions which meet this condition. 
To take this fact into account we use our dynamic programming approach on the delegation graph $H_d[V\setminus Anc(n)]$. 
Moreover, in this case $N^k$ is obtained by a different formula. Let $\alpha = |Anc(n)|$, then  we use the formula:   
\begin{equation} \label{eq:Nk computation2}
N^k = \sum_{w =q_\alpha-k-1 }^{q_\alpha-1} X_{\mathcal{F}_2}[n-t_n,w] (X_{\mathcal{F}_1}[t_n,k]),
\end{equation}
where $q_\alpha = q - \alpha$.

We move to the complexity analysis. Equation \ref{eqRecursiveFB} can be computed in $O(n)$ operations. This leads to a complexity of $O(n^3)$ for computing tables $F_{\mathcal{F}_1}$ and $F_{\mathcal{F}_2}$. As Equations \ref{eq:Nk computation} and \ref{eq:Nk computation2} can be computed in $O(n)$, computing all values $N^k$ can be performed with $O(n^2)$ operations. Therefore, computing the Banzaf value requires $O(n^3)$ operations.
\end{proof}


==> Contribution/DynamicProgramming/oldindexvalue.tex <==

%In the first term, $F[j-t_j,w, s-x] $ counts the number of subsets in $\{1, \ldots, j-t_j\}$ that have weight $w$ and size $s-x$ ($0\le x\le t_j-1$) and do not contain $j$ nor her followers. Note that in the case voter $j$ does not join a coalition $C$, each possible subset $S$ of her followers (i.e., $S \subseteq T_d(j)\setminus \{j\}$) could join $C$ as inactive agents. $F[j-1,w-1, s-1]$ counts the number of subsets $C' \subset \{1,\ldots, j-1\}$ such that $|C'| = s$ $w_d(C'\cup C) = w_d(C)+ w$ and size $s$ that contain $j$.

%For instance in Example~\ref{exNotations}, when $C=\{2,3,8\}$, we can move to the subtree $T_d(1)$, $1$ cannot join $C$, but her followers could join $C$ as inactive voters. In this case, $|T_d(1)\setminus\{1\}|=0$.
  
In order to add a subtree $T$ of $T_d(n)$ rooted in $n$ to the resulting coalitions of table $F$, we use another table $X[j',w',s']$ to be the number of $s'$-element subsets of $\{1,..., n-t_n,..., j'\}$ in which voters in $\{1,...,n-t_n\}$ have weight $y'\in \{w',...,q-1\}$, i.e., each $s'$-element subset contains $w'\le y'\le q-1$ active voters of $\{1,...,n-t_n\}$. Here, $j'$ ranges from $t_n$ to $n-1$, $s$ ranges from $0$ to $n-1$ and $w'$ ranges from $0$ to $q-1$. Note that $t_n$ is the last child of $n$.

For $j'=t_n,...,n-1$, $w'=1,...,q-1$ and $s'=1,...,n-1$, $X[j',w',s']$ will be filled as follows. We distinguish two cases.

\begin{enumerate}
    \item $j'-t_{j'}=t_n$. Let $y=q-w'-1$. In this case, we have
    \begin{equation}\label{eqRecursiveHCase1}
      \begin{split}
         X[j', w', s']&=\sum_{y'=0}^{y}\sum_{x = 0}^{ t_{j'}-1} {t_{j'}-1 \choose x}F[n-t_n, w'+y', s' - x] \\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation}
     Let us explain each term separately.
     \paragraph{First term.}  $F[n-t_n,w'+y', s'-x] $ counts the number of subsets that have weight $w'+y'$ ($0\le y' \le y$) and size $s-x$ ($0\le x \le t_j-1$) and do not contain $j'$ nor her followers. Note that if voter $j'$ does not join a coalition $C$, each possible subset $S$ of her followers (i.e., $S \subseteq T_d(j)\setminus \{j\}$) could join $C$ as inactive agents. Furthermore, the interpretation of the first summation that is over weight $y'$ ranges from $0$ to $y$ is as follows. $j'-t_{j'}=t_n$ means that the the rest of voters $\{t_n,...,j'\} \in T_d(n)$ do not join, so a subset of voters in $\{j'+1,..., t_n-1\} \subseteq T_d(n)$ with weight $q-w'$ could join a subset of voters in $\{1,...,n-t_n\}$ with weight $w'+y'$ such that $0\le y'\le q-w'-1$. In other words, when $n$ has a weight $q-w'$ in a $s'$-element subset $C$, all possible subsets of the gurus in $Gu_d\setminus \{n\}$ and their followers that have a weight $y'\in \{w',...,q-1\}$ could join $C$. 
     
     \paragraph{Second term.}The second term $X[j'-1,w'-1, s'-1]$ counts the number of subsets that contain $j'$ and voters in $\{1,...,n-t_n\}$ have weight $y'\in \{w',...,q-1\}$. 
     
     To illustrate the two terms, consider Example~\ref{exNotations}. To compute $DB_8$, when $C=\{8\}$, for $s'=1,...,7$, we have
     \begin{equation*}
      \begin{split}
         X[7, 2, s']&=\sum_{y'=0}^{0}\sum_{x = 0}^{ 3} {3\choose x}F[3, 2+y', s' - x] + X[6,1, s'-1]
      \end{split}
     \end{equation*}
    The first term shows that if voters $7$ does not join $C$ (i.e., $w_8(C)=1$), the rest of voters in $\{1,2,3,4,5,6\}$ with a weight of $2$ could join $C$. Note that voters in $\{4,5,6\}$ could only join $C$ as inactive voters. The second term shows the case where voter $7$ joins $C$.  
       
     \item Otherwise (i.e., $ j'-t_{j'} > t_n$),
     \begin{equation}\label{eqRecursiveHCase2}
      \begin{split}
         X[j', w', s']&=\sum_{x = 0}^{ t_{j'}-1} {t_{j'} - 1 \choose x}X[j' - t_{j'}, w', s' - x]\\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation}
     
     This case concerns those cases in which we move from a subtree in $T_d(n)$ to another subtree in $T_d(n)$. The first term counts the number of $s'$-element subsets a subtree $T \in T_d(n,q-w')$ and $j'\notin T$ (but contain the followers of $j'$ as inactive voters). The second term counts the number of $s'$-element subsets that contain a subtree $T \in T_d(n,q-w')$ and $j'\in T$. voter As an instance, in Example~\ref{exNotations} when $C=\{7,8\}$, we have
     
     \begin{equation*}
      \begin{split}
         X[6,1, s']&=\sum_{x = 0}^{ 1} {1 \choose x}X[4, 1, s' - x]+ X[5,0, s'-1]
      \end{split}
     \end{equation*}
     The first term represents the case where voter $6$ does not join $C$. In this case, voter $5$ could join $C$ as inactive voters and we move to subtree $T_d(4)$. The second term shows the case where $6$ joins $C$.
\end{enumerate}

We need to examine the especial case $w=0$, $j$ ranges from $t_n$ to $n-1$ and $s'$ range from $0$ to $n-1$ separately. Let $y=q-1$, we distinguish three cases.

\begin{enumerate}

 \item $j'- T_d(j')>0$. In this case, we have
     \begin{align}\label{alignWZeroCase1}
         X[j', 0, s']&=\sum_{x = 0}^{ t_{j'}} {t_{j'} \choose x}X[j' - t_{j'}, 0, s' - x]
      \end{align}
     As an example, when $C=\{6,7,8\}$ in Example~\ref{exNotations}, we can move from $5$ to subtree $T_d(4)$, however all voters in subtree $T_d(5)$ could join $C$. 
     \HG{At this point it becomes quite clear that $F[j, 0, s]$ is not well defined !}
   \item $j'-t_{j'}=t_n$. In this case, we have
    \begin{align}\label{alignWZeroCase2}
         X[j', 0, s']&=\sum_{y'=0}^{y}\sum_{x = 0}^{ t_{j'}} {t_{j'} \choose x}F[n-t_n, y', s' - x]
    \end{align}
     For instance in Example~\ref{exNotations}, when going from $5$ to subtree $T_d(4)$, we have this coalition $C=\{6,7,8\}$ ($5$ and her followers may join $C$). Now from $4$ we can move to subtree $T_d(3)$. In this case, voter $8$ could have weight greater than $q=3$ (by joining $5$ and $4$ to $C$), so $4$'s followers and a subtree of $T_d(3)$ with weight $y' \in \{0,1,2\}$ could join $C$.
     
     \item  $j'=t_n$ and $T_d(j')=\emptyset $, i.e., the last child of $T_d(n)$ in the ordering $\pi_d$.
        \begin{align}\label{alignWZeroCase3}
         X[t_n, 0, s']=\sum_{y'=0}^{y} F[n-t_n, y',s]
       \end{align}
        This term shows those cases where the last child of $T_d(n)$ joins a coalition $C\subseteq T_d(n)\setminus \{j'\}$ and $w_n(C)=q$. So a subset of $\{1,..., n-t_n\}$ with weight of $y'=\{0,1,...,q-1\}$ could join $C$. For instance in Example~\ref{exNotations}, when we have this coalition $C=\{7,8\}$ and if $4$ which is the last child of $8$ joins $C$, voters in $\{1,..., n-T_d(n)\}$ with weight of $y' \in \{0, 1,2\}$ could join $C$.
\end{enumerate}

Now, $N_s$, for $s=0, 1, ..., n-1$, can be computed as 

\begin{align*}
    N_s=X[t_n-1, q-1, s].
\end{align*}

In the case $n \notin Gu_d$, in order for $n$ to be an active agent in a coalition $C$, voters $\delta_d(n, d^{*}_n) \cup \{d^{*}_n\}$ have to be contained in $C$. To do so, we consider the set $c_d(n, d^{*}_n)$ as a new node $n'$ and define a new delegation profile $d'$ as follows. For every voter $j$, if $d_j\in c_d(n, d^{*}_n)$, we set $d'_j=n'$; $d'_j=d_j$ otherwise. So, we consider $n'$ as a guru in $H_{d'}$ and the last voter in the ordering $\pi_{d'}$ of $H_{d'}$. For simplicity, we assume that voters $T_d(n)\setminus \{n\}$ precede $n'$ in $\pi_{d'}$, meaning that voters in $T_d(n)\setminus \{n\}$ visited after $n'$ in a depth-first search of $H_{d'}$ starting from $n'$. Also, in this case, we define new quota $q'=q-|\delta_d(n, d^{*}_n) \cup \{d^{*}_n\}|$. Hence, to compute the index value for a voter $n \notin Gu_d$, we can simply consider the delegative simple game of $V'=<N', d', q'>$, where $N'=N \cup \{i'\}\setminus c_d(n, d^{*}_n)$. For instance, to compute $B_6$ in Fig.~\ref{figNotation}, we consider the set $\{6, 7, 8\}$ as a new voter $6'$ and define a new delegation profile $d'=(3,3,3,6',6',6')$ ( see Fig.~\ref{figDelegator'sIndex}). Also, $\pi_{d'}=<1,2,3,4,5,6'>$ in which set $T_d(6)\setminus\{6\}=\{5\}$ precede $6'$. %Therefore, in the rest of the proof, for the sake of simplicity, we assume that $n \in Gu_d$. %One last piece of assumption: here for the sake of simplicity, we assume that voters in $c_d(n, d^{*}_n)$ are first visited in a depth first search, meaning that $\delta_d(n, d^{*}_n)\cup \{n\}$ precede $d^{*}_n$ in $\pi_d$. 

\begin{figure}[h]
		\centering
		\begin{tikzpicture}
				\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white}}
				\tikzset{edge/.style = {->,> = latex'}}
				
				\node[vertex] (6') at  (0,3) {$6'$};
				\node[vertex] (5) at  (-.5,2) {$5$};
				\node[vertex] (4) at (.5,2) {$4$};
				
				\node[vertex] (3) at  (2.5,3) {$3$};
				\node[vertex] (2) at  (2,2) {$2$};
				\node[vertex] (1) at  (3,2) {$1$};
				
				
				
				%edges
				\draw[edge] (5) to (6');
				\draw[edge] (4) to (6');
				
				\draw[edge] (1) to (3);
				\draw[edge] (2) to (3);
		\end{tikzpicture}

		\caption{ The new delegation graph $H_{d'}$ with $q'=1$ is used to compute the voter $6$'s (i.e., the original voter $6$) index power in Example~\ref{exNotations}.} \label{figDelegator'sIndex}
	\end{figure}


 In this case, the table $X$ is only defined on $T_d(n)$. So, Equation~\ref{eqRecursiveHCase1} and~\ref{eqRecursiveHCase2} should respect the delegation profile $d$, meaning that for $j'$ ranges from $t_d(n), ..., n'-1$, $w'=1, ..., q'-1$ and $s'$ ranges from $1$ to $n'-1$, we have:


\begin{enumerate}
    \item $j'- t_{j'}=t_n$. Let $y=q'-1-w'$. In this case, we have
    \begin{equation*}
      \begin{split}
         X[j', w', s']&=\sum_{y'=0}^{y}\sum_{x = 0}^{ t_{j'}-1} {t_{j'} - 1 \choose x}F[j' - t_{j'}, w+y', s' - x] \\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation*}
    For instance in Example~\ref{exNotations}, to compute $B_6$, if voter $5$ does not join the coalition $C=\{6,7,8\}$, we can move to subtree $T_d(4)$ rooted in voter $4 \notin T_d(6) \cap T_d(6')$ (see Figures~\ref{figDelegator'sIndex} and~\ref{figNotation}), but since $q=3$, voter $4$ (and voter $3$) cannot join $C$. However, voters $1$, $2$ and $5$ could join $C$.
     
     \item Otherwise (i.e., $ j'-t_{j'} > t_n$),
     \begin{equation*}
      \begin{split}
         X[j', w', s']&=\sum_{x = 0}^{ t_{j'}-1} {t_{j'}- 1 \choose x}X[j' - t_{j'}, w', s' - x]\\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation*}
     
\end{enumerate}

In the same way, in the special case $w'=0$, $j'$ ranges from $t_n$ to $n'-1$ and $s'$ range from $1$ to $n'-1$, Equations~\ref{alignWZeroCase1},~\ref{alignWZeroCase2} and~\ref{alignWZeroCase3} have to respect the delegation function $d$ too. 



Recall that $q'=q-|\delta_d(i, d^{*}_i) \cup \{d^{*}_i\}|$. Now, $N_s$, for $s=0, 1, ..., n-1$, can be computed as follows:

\begin{align*}
 N_s \!=\! \left\{ \begin{array}{c c}
0 & \text{ if } q'\le 0\\
X[n'-1, q'-1, s-|\delta_d(i, d^{*}_i) \cup \{d^{*}_i\}|] & \text{ otherwise.}
\end{array} \right.
\end{align*}

Note that in the case $q' \le 0$, $i'$ is a distant voter and will not be a swing agent for any coalition. For instance, in Example~\ref{exNotations}, voter $5$ is a distant voter since a necessary condition for her to be in any coalition $C$ is that $\{6,7,8\}\subseteq C$, meaning that $\sum_{j \in \hat{D}(C)\setminus \{5\}}w(j) \ge 3$. Thus, $B_5=Sh_5=0$.

We can now compute the shapely value of voter $i=n$. Thus, with memoization, the Shapley value of a voter can be computed in $O(n^{5})$. Because two tables $F$ and $X$ have $n^3$ entries in total and in the worst case, it takes $O(n^2)$ for each entry to be filled.

For the Banzaf index, we can simply omit the third parameter $s$ and compute a voter value, which can be computed in $O(n^{3})$.

%We denote by $d^*(i)$ the guru of voter $i$, i.e., the guru that is found by following delegations from $i$.
%For $C \subseteq N$, let $C^d = \{i\in C| d(i) = i\}$. 
%For any $C \subseteq N$, we write $D(C) = \{j\in N | \exists k\in C, d^*(j) = k\}$.

==> Contribution/Modification/DTO.tex <==
In the next step, we show that we are able to apply the approximation algorithm given by Ghuge and Nagarajan~\cite{ghuge2020quasi} to the optimization version of \textbf{WmaxP}, called \textbf{OWmaxP}. Indeed, Ghuge and Nagarajan~\cite{ghuge2020quasi} investigated the following problem, called \textbf{STO}. Given a directed graph $G=(V, E)$ with edge costs $c:E \rightarrow \mathbb{Z}^{+}$, a root vertex $r^* \in V$, a budget $B$, and a monotone submodular function $f:2^V \rightarrow \mathbb{R}_{+}$. For any subgraph $G'$ of $G$, let $V(G')$ and $E(G')$ represent the set of nodes and edges in $G'$. The goal in \textbf{STO} is to find an out-directed arborescence $T^*$ rooted at $r^*$ maximizing $f(V(T^*))$ such that $\sum_{e \in E(T^*)} c(e) \le B$. They provided a factor $O(\frac{\log n'}{\log \log n'})$-approximation algorithm for \textbf{STO}, where $n'$ is the number of vertices in an optimal solution. Note that the authors mentioned that this factor is tight for \textbf{STO}.

Now we aim to show that \textbf{OWmaxP} is closely related to a special case of \textbf{STO}. % as studied by Ghuge and Nagarajan~\cite{ghuge2020quasi}. 
In particular, consider special instances $I'=\langle D'= (V', A'), r^*, c, f, B \rangle$ of \textbf{STO}, where for any edge $e \in A'$, $c(e)=\{0, 1\}$. More importantly, there is no cycle $C$ in $D'$ with total cost $\sum_{e \in E(C)}c(e)=0$, i.e., there exists at least one edge $e \in C$ with $c(e)=1$. %for any $e \in E(C)$, $c(e)=0$, i.e., $\sum_{e \in C}c(e)=0$. %there exists at least one edge $e \in C$ with $c(e)=1$. 
Also, for any $S \subseteq V'$, $f(S)=\sum_{i \in S}w_i$, where $w_i$ is the weight of $i \in V'$. %the cost of each outgoing edge is either $1$ or $0$.
We term \textbf{STO} on these special instances \textbf{SSTO}.

%\paragraph{Connections to \textbf{STO}.} 

\begin{theorem}
Let $\alpha$, $0<\alpha<1$, be a constant. The following statements are equivalent:

\begin{enumerate}
    \item[(i)] There is an $\alpha$-approximation algorithm for \textbf{SSTO}.\label{alpha-SSTO}
    
    \item[(ii)] There is an $\alpha$-approximation algorithm for \textbf{OWmaxP}.\label{alpha-WmaxP}
\end{enumerate}
\end{theorem}

\begin{proof}
To prove that (i) implies (ii), we proceed as follows. Let $I=\langle D= (V, A), \omega, d,i^*, k \rangle$ be an instance of \textbf{OWmaxP}. Without loss of generality, we suppose that $d_{i^*}=i^*$; otherwise we define a new delegation graph $d'$ such that $d'_{i^*}=i^*$, $d'_i=d_i$ for any $i \in V \setminus \{i^*\}$ and $k=k-1$. Let $I'=\langle D'= (V', A'), r^*, c, f, B \rangle$ be an instance of \textbf{SSTO} obtained from $I$ as follows. We set $V'=V$, $r^*=i^*$ and $A'=\{(i,j):(j,i) \in A\}$, i.e., we reverse the edges. For any $e=(i,j) \in A'$ in $I'$, if $d(j)=i$ in $I$, $c(e)=0$; $c(e)=1$ otherwise. For any $S \subseteq V'$, let $f(S)=\sum_{i \in S}\omega(i)$. Lastly, $B=k$. Consider a solution $T^*$ to \textbf{SSTO} on $I'$. We can simply reverse the edges in $T^*$ and obtain a subtree rooted in $i^*=r^*$ with maximum weight such that $c(T^*) \le B=k$ in $I'$. We conclude by noticing that any edge $e=(i, j) \in E(T^*)$ either costs $0$ if $d(j)=i$ or $1$ otherwise.

To prove that (ii) implies (i), we give a polynomial-time reduction from \textbf{SSTO} to \textbf{OWmaxP} as follows. Let $I'=\langle D'= (V', A'), r^*, c, f, B \rangle$ be an instance of \textbf{SSTO}. Let $I=\langle D= (V, A), \omega, d,i^*, k \rangle$ be an instance of \textbf{OWmaxP} obtained from $I'$ as follows. We set $V'=V$, $r^*=i^*$ and $A=\{(i,j):(j,i) \in A'\}$, i.e., reversing edges. For any voter $i \in V \setminus \{i^*\}$ if there exists an incoming edge $e=(j, i) \in A'$ with cost $c(e)=0$, we set $d_i=j$; $d_i=i$ otherwise. We set $d_{i^*}=i^*$. For any $i \in V$, let $\omega(i)=w_i$. Lastly, we set $k=B$. As there exists no cycle $C \in D'$ with $\sum_{e \in C}c(e)=0$ and for any $i \in V'$ there is at most one incoming edge $e$ with cost $c(e)=0$, the resulting delegation graph $H_d$ is feasible. Now consider another delegation graph $H_{d'}$ such that $|\{i\in V : d(i)\neq d'(i)\}|\le k$ and $\alpha_{d'}(i^*)$ being maximized. By reversing the edges in subtree rooted at $i^*$ in $H_{d'}$ we get an out-directed arborescence $T^*$ that is rooted at $r^*$ with maximum $f(V(T^*))$ in $I'$.
\end{proof}

In the next step, we show that \textbf{OWmaxP} is NP-hard even when the out-degree and in-degree of every vertex in an SN is at most $2$ and the weight assigned to each vertex is either $0$ or $1$.

\begin{theorem}
\textbf{OWmaxP} is NP-hard even when in a given graph $G=(V,E)$, for any voter $i \in V$, $|\mathtt{Nb}_{out}(i)| \le 2$, \ $|\mathtt{Nb}_{in}(i)| \le 2$ and $\omega(i) \in \{0, 1\}$.
\end{theorem}

\begin{proof}
To prove the theorem, we give a reduction from the vertex cover problem to \textbf{WmaxP}. Recall that in the vertex cover problem we are given a graph $G=(V, E)$ and a budget $k$, and the goal is to select a set of vertices $S \subset V$ with size $|S| \le k$ such that for any edge $e=\{i, j\} \in E$, $|\{i, j\} \cap S| \ge 1$. Let $E_i$ be the set of incident edges $e \in E$ to node $i$ and $n_V=|V|$. We order $E_i$ for any node $i$ and let $e_j^i$ be the $j$th edge in $E_i$. %In the following, when we write $e=e_j^i$, it means that $e$ is the $j$th edge in $E_i$.

Given an instance $I=(G=(V,E), k)$ of the vertex cover problem, an instance $I=\langle D= (\bar V, A), \omega, d,i^*, \bar k \rangle$ of \textbf{OWmaxP} obtained as follows. We create a digraph $D = (\bar V, \bar A)$ where: 
\begin{itemize}
    \item $\bar V = V_1 \cup V_2 \cup \{V_3\} \cup \{i^*\} $ with $V_1 = \{u'_i, 
    u_i^1,\ldots, u_i^{|E_i|} : i\in V\}$, $V_2 = \{w_e : e \in E\}$ and $V_3=\{u_i: i\in V\}$.
    \item $\bar A = \{(u_i,u'_i) : i\in V\} \cup \{(u'_i, u'_{i+1}): i \in [n_V-1]\} \cup \{(u'_{n_V}, i^*)\} \cup \{(w_e,u^j_i) : e\in E, e=e^i_j, i\in V\} \!\cup\! \{(u_i^1,u_i),\ldots,$ $(u_i^{|E_i|},u_i^{|E_i|-1}) : i \in V\}$.
\end{itemize}

Note that 
%\begin{enumerate}
     (i) for any voter $v \in V_1 \cup V_3 \setminus \{i^*\}$, we have $|\mathtt{Nb}_{out}(v)|=1$ and $|\mathtt{Nb}_{in}(v)|=1$, (ii) $|\mathtt{Nb}_{out}(i^*)|=0$ and $|\mathtt{Nb}_{in}(i^*)|=1$, and (iii) for any voter $v \in V_2$, $|\mathtt{Nb}_{out}(v)|=2$ and $|\mathtt{Nb}_{in}(v)|=0$.
    %\item For any voter $v \in V_3$, $|\mathtt{Nb}_{out}(v)|=1$ and $|\mathtt{Nb}_{in}(v)|=1$.
%\end{enumerate}

For any  $v \in V_1 \setminus \{i^*\}$, let $\omega(v)=0$ and $d_{v}=v_{out}$, where $v_{out} \in \mathtt{Nb}_{out}(v)$. For any $v\in V_2 \cup \{i^*\}$, we set $\omega(v)=1$ and $d_v=v$. For any voter $v \in V_3$, $d_v=0$ and $\omega(v)=0$. Let $\bar k=k+|E|$. Note that $i^*$ has the maximum weight when all voters in $V_2$ indirectly delegate to $i^*$ as only voters in $V_2 \cup \{i^*\}$ have weight $1$. Let us consider a delegation function $d'$, such that $|\{i\in V:d(i)\neq d'(i)\}|\le \bar k$. We say that node $w_e \in V_2$ in $H_d'$ is activated node for $d'$ if there exists a delegation path $P$ from $w_e$ to $i^*$ in $H_{d'}$. We call $P$ an activated delegation path. Note that there are only two delegation paths that make $w_e$ activated and each activated delegation path for $w_e$ represents one of the endpoints $e \in E$.

Suppose $I$ is a `yes'-instance for the vertex cover problem and $S \subset V$ is a solution. We define new delegation function $d'$ as follows. For any $i \in S$, $d'_{u_i}=u'_i$; denote these voters by $V_3^S$. Now for any $w_e \in V_2$, we select a delegation path that makes $w_e$ activated, i.e., $w_e$ delegates to $i^*$ indirectly through an activated delegation path (the choice of activated delegation path can be made arbitrarily if there are two of them). For any voter $v \in \bar V \setminus (V_2 \cup V_3^S)$, $d'_v=d_v$. Obviously, this is an optimal solution to \textbf{OWmaxP} as all voters with weight $1$ delegate to $i^*$ indirectly.

In the other direction, suppose that we find an optimal delegation $d'$ obtained from $d$ such that all voters in $V_2$ are activated. It means that there exists a set of voters $V_3^{OPT} \subset V_3$ with size $k$ who transfer the weight of all voters in $V_2$ toward $i^*$. Let $S$ be a solution to the vertex cover problem that obtained as follows: $S=\{i:u_i \in V_3^{OPT}\}$. Clearly, this is an optimal solution to the vertex cover problem as for each node $w_e \in V_2$ there exists at least one voter in $V_3^{OPT}$ who transfers her weight toward $i^*$, i.e., its corresponding edge $e \in E$ is covered by at least one node $i \in S$.
\end{proof}


More positively, \textbf{OWmaxP} becomes tractable when in a given graph $D=(V, A)$ for any voter $v \in V$, $|\mathtt{Nb}_{out}(v)| \le 1$.

\begin{theorem}
There is a polynomial-time algorithm for \textbf{OWmaxP} when the out-degree of each vertex is at most $1$.
\end{theorem}

\begin{proof}
Let $I = (\langle D = (V,A),\omega, d , k\rangle, i^*, k)$ be an instance of \textbf{OWMaxP} in which for any voter $v \in V$ $|\mathtt{Nb}_{out}(v)| \le 1$. Note that, without loss of generality, we suppose that $r^*$ is a guru in $H_d$, also we remove out-edges of $r^*$ if there is one. We first note that one can collapse each subtree $T$ in $H_d$ rooted in $r_T$ in one vertex $rc_T$ with weight $\alpha_d(r_T)$. Now we direct an edge from node $rc_T$ to $rc_{T'}$ if there exists an edge from $r_T$ to $r_{T'}$ in $A$. We denote this new graph by $CD=(CV, CA)$. Note that $CV$ contains only the root of subtrees in $H_d$ with possible new weights. We note that the subgraph of $CD$ in which there exists a path from each node $v \in CV$ to $i^*$ is a tree; otherwise at least one of the vertices has out-degree with size $2$ which contradicts our assumption that $|\mathtt{Nb}_{out}(v)| \le 1$. Let $T$ be the tree rooted at $i^*$ in $CD$. If $\sum_{e \in T} c(e) \le k$, we are done. Suppose it is not the case. Then we proceed as follows. Let $V(T)=\{1,2,\dots, n\}$ be the set of voters in $T$ and $n=i^*$. We run a depth-first search of $T$ starting from $i^*$. Let $\pi_d$ be the ordering of voters in $T$ such that voters are sorted in decreasing order of their discovering times in the depth first search. 
As $n$ is first visited in the depth first search, it is the last voter in the ordering $\pi_d$. We define a table $F$ where $F[i,c]$ is the subtree with maximum weight composed of a set $S \subseteq \{1,2,\dots, i\}$ with cost at most $c$, where $i$ ranges from $0$ to $n-1$ and $c$ ranges from $1$ to $k$. Let $T(j) \subseteq T$ be the subtree rooted in a vertex $j$ and $t_j=|T(j)|$. The entries of this table will be filled as follows. For $i=0$, we have $F[0,c]=0$. For $c=1$, we have $F[i,0]=0$ and $F[i,1]=\omega_i$. $F[i,c]=\max \{F[i-1, c-1]+w_i, F[i-t_i, c]\}$. The first summand corresponds to the case that $i$ will be in the solution and delegates to $n$ (directly or indirectly). The second summand indicates that $i$ does not delegate to $i$, so $i$ and the subtree $T(i)$ will be removed from further consideration. After filling the table entries, comparing the first summand and the second summand will enable us to find out $i$ (and its subtree) is in the final solution. It takes $O(nk)$ to find an optimal solution.
\end{proof}

==> Contribution/Modification/iminpbs.tex <==
\HG{//TO CORRECT AND THEN PUT BACK IN PLACE}
More positively, \textbf{IMinP} becomes tractable when $D$ is complete. We start with the following observation from Zhang and Grossi~\cite{zhang2020power}.


%\begin{fact}[Fact 2 in~\cite{zhang2020power}]\label{factMonotonocity}
%For any pair of agents $i, j \in V(D)$, such that $d_i=j$, $DB_i \le DB_j$.
%\end{fact}

\begin{fact}[Fact 3 in~\cite{zhang2020power}]\label{Direct vs. Indirect Delegation}
given a delegative simple game $V=<N,d,q>$, in
which there exists three agents $i, j, k \in N$, such that $d_i =
j$ and $d_k = i$. Let then $V=<N,d',q>$, such that for any $v \in N\setminus \{k\}$
$d'_v=d_v$ and $d'_k=j$. Then, $DB_k(V')\ge DB_k(V)$.
\end{fact}

The following two modifying operations will be helpful.
\begin{definition}[$Cut(V, j)$]
A modifying operation that, given a delegative simple game $V=<N,d,q>$ in which there exists a follower $j$, outputs another delegative simple game $V=<N,d',q>$ such that for any $i \in N\setminus \{j\}$ $d'_i=d_i$, and $d'_j=j$.
\end{definition}

\begin{definition}[$Join(V,g,j)$]
A modifying operation that, given a delegative simple game $V=<N,d,q>$ in which there exists a guru $g \in Gu_d$, a voter $j$ and $j \notin T_d(g)$, outputs another delegative simple game $V=<N,d',q>$ such that for any $i \in N\setminus \{g\}$ $d'_i=d_i$, and $d'_g=j$. 
\end{definition}

Let $\Delta$ be the running time of computing the index power $f_i(\mathcal{E})$ of any voter $i$ . Let $Leaves(H)$ be the set of all leaves in $H$. 

 The following observation implies that during the procedure of minimizing $f_u$, when it comes to applying the Join operation, we only perform $Join(V,d^*_u,j)$, where $j \in Leaves(H_d)\setminus T_d(d^*_u)$.

\begin{obs}\label{obsDelegatingtoLeaves}
Consider a delegative simple game $V=<N,d,q>$, a voter $u$ and a leaf $l \in Leaves(H_d) \setminus T_d(d^*_u)$. $Join(V,d^*_u,l)$ minimizes $f_u$ more than $Join(V,d^*_u,v)$, where $v \in c_d(l,d^*_l)$.
\end{obs}
\begin{proof}
By the same argument as Zhang and Garossi Showed in Fact 3 in ~\cite{zhang2020power}, we can show that Fact~\ref{Direct vs. Indirect Delegation} holds when $f=DS$. Then, using Fact~\ref{Direct vs. Indirect Delegation}, we see that delegating $d^*_u$ to $l$ results in another delegative simple game in which $f_u \le f_l \le ...\le f_{d^*_l}$. This concludes the proof.
\end{proof}

The following lemma says that $Join(V,d^*_u,j)$ minimizes $f_u$ more than $Join(V,g,j)$, where $g \ne d^*_u$.
\begin{lemma}\label{lmDelegatingu}
Consider a delegative simple game $V=<N,d,q>$, and three voters $u, j$ and $g$, where $d^*_g \ne d^*_u \ne d^*_j$. Consider two delegative simple games $V_1=Join(H_d,d^*_u,j)$ and $V_2=Join(H_d,g,j)$. Then $f_u(V_1) \le f_u(V_2)$.
\end{lemma}
\begin{proof}
Let $C$ be a coalition in $V_1$ for which $u$ is a swing agent. Then, we must have $c(j,d^*_j) \subset C$.  The proof follows by noticing that the active voters in $C$ and $C\setminus\{u\}$ are the same.  
\end{proof}

Consider two gurus $g_1, g_2$ in a delegation graph $H_d$. The following observation says that if $d^*_u$ delegates to a leaf $l_1 \in T_d(g_1)$ and then $g_1$ delegates to a leaf $l_2 \in T_d(g_2)$ decreases $f_u$ as much as $d^*_u$ first delegates to a leaf $l_2 \in T_d(g_2)$ and then $g_2$ delegates to a leaf $l_1 \in T_d(g_1)$.
\begin{obs}\label{obsOrderOfSubtree}
Consider a delegative simple game $V=<N,d,q>$, in which there exists a follower $u$ and two gurus $g_1, g_2$, where $g_1 \ne g_2 \ne d^*_u$. Consider two leaves $l_1 \in T_d(g_1)$ and $l_2 \in T_d(g_2)$. Suppose $V_1=<N,d_1,q>=Join(Join(V, d^*_u, l_1), g_1,l_2)$ and $V_2=<N,d_2,q>=Join(Join(V, d^*_u, l_2), g_2,l_1)$. Then $f_u(V_1) = f_u(V_2)$.
\end{obs}
\begin{proof}
It is easy to see that in both $V_1$ and $V_2$, $c_{d_1}(u,d^*_u)=c_{d_2}(u,d^*_u)$. So, the number of coalitions that $u$ is swing is the same in both $V_1$ and $V_2$.
\end{proof}


\begin{obs}\label{obsUnnecessaryCutIntermediate}
Consider a delegative simple game $V=<N,d,q>$, in which there exists a follower $u$. During the procedure of minimizing $f_u$, it is unnecessary to apply the $Cut(V,j)$ operation, where $j \in c_d(u, d^*_u)$.
\end{obs}

\HG{Why ?}
\begin{proof}
Let $\mathcal{A}$ be an algorithm that applies the $Cut(V,j)$ operation for some $j \in c_d(u, d^*_u)$ at some point to minimize $f_u$. Let $H_{d'}$ be the resulting delegation graph after applying $Cut(V,j)$. Keep in mind that $j$ is now the guru of $u$ in $H_{d'}$, i.e., $d'^*_u=j$ and $d'^*_u \ne d^*_u$. The only reason $\mathcal{A}$ would apply this operation is that to delegate $j$ to another leaf in subtree $T_d(d^*_u) \setminus T_d(j)$ in the future. Suppose that this is not the case, i.e., $\mathcal{A}$ will not delegate $j$ to another leaf $l \in T_d(d^*_u)\setminus T_d(j)$ in the next steps. So, $\mathcal{A}$ will delegate $j$ to some other leaves $l \in Leaves(H_d) \setminus T_d(d^*_u)$. Now let $\mathcal{A'}$ be another algorithm that does not apply $Cut(V,j)$ and follows the same sequence of operations as $\mathcal{A}$ after performing $Cut(V,j)$ does. We see that $f_u$ is decreased by $\mathcal{A'}$ more than by $\mathcal{A}$, as the number of intermediate voters between $u$ and her guru in the delegation graph resulting from $\mathcal{A'}$ is more than the number of intermediate voters between $u$ and her guru in the resulting graph from $\mathcal{A}$. This implies that the only reason $\mathcal{A}$ would perform the operation $Cut(V,j)$ in $H_d$ is that to delegate $j$ to another leaf in subtree $T_d(d^*_u) \setminus T_d(j)$ in the future. Consider the graph $H_{d'}$ resulting from $Cut(V,j)$. After applying $Cut(V,j)$, using Observation~\ref{obsOrderOfSubtree}, suppose that $\mathcal{A}$ delegates $d'^*_u=j$ to one of the leaves $l \in T_d(d^*_u) \setminus T_d(j)$. Let $i$ be the voter where $d_i \in c_d(u, d^*_u)$ and $l \in T_d(i)$. Let $\mathcal{A''}$ be the algorithm that does not apply $Cut(V,j)$ and instead applies $Cut(V,i)$ and then delegates $d^*_u$ to $l$. Let $H_{d''}$ be the resulting graph. We see that $c_{d''}(u,d''^*_u)=c_{d'}(u, d'^*_u)$. After this, suppose that $\mathcal{A''}$ would follow the same sequence of operations as $\mathcal{A}$ does. This concludes the proof.
\end{proof}


The following observation implies that to minimize $f_u$, it is unnecessary to execute the $Cut(V,j)$ operation for $j \in V \setminus T_d(d^*_u)$.
\begin{obs}\label{obsUnnecessaryCut}
Consider a delegative simple game $V=<N,d,q>$, in which there exists a follower $u$. During the procedure of minimizing $f_u$, it is unnecessary to apply the $Cut(V,j)$ operation, where $j \notin T_d(d^*_u)$ and the budget $k \ge 2$.
\end{obs}

\begin{proof}
Let $\mathcal{A}$ be the algorithm that applies $Cut(V,j)$ for some $j \notin T_d(d^*_u)$ at some point when $k \ge 2$. We distinguish two cases:
\begin{enumerate}
    \item $\mathcal{A}$ would perform $Cut(V,j)$ to delegate the guru of $u$ to a leaf $l \in T_d(j)$ in the future, using Observation~\ref{obsDelegatingtoLeaves}. After applying $Cut(V,j)$, using Observation~\ref{obsOrderOfSubtree}, $\mathcal{A}$ would delegate $j$ to a leaf $l \in T_d(d^*_j) \setminus T_d(j)$ and then delegates the guru of $u$ to a $l' \in T_d(j)$ (or, using Observation~\ref{obsOrderOfSubtree}, first delegates the guru of $u$ to $l$ and then delegates $d^*_j$ to $l'$). We see that we can first delegate the guru of $u$ to $l'$, so now $j$ is in the same subtree $T$ as $u$ is and then delegates $j$ to $l$, which concludes the proof.
    
    \item After applying $Cut(V,j)$, $\mathcal{A}$ would \textbf{not} delegate the guru of $u$ to a leaf $l \in T_d(j)$ in the next steps. Let $\mathcal{A'}$ be another algorithm that instead of applying $Cut(V,j)$, performs $Join(V,d^*_u,l)$ and then follows the same sequence of operations that $\mathcal{A}$ would perform after applying the $Cut(V,j)$ operation. It is easy to see that $\mathcal{A'}$ works better, which implies the observation.
\end{enumerate}
 %
\end{proof}
Now we are ready to present the greedy algorithm that minimizes $f_u$. We term this algorithm GreedyMin. GreedyMin considers the following sub-cases:

\begin{enumerate}
    \item If $k=1$. Using Lemma~\ref{lmDelegatingu}, Observation~\ref{obsDelegatingtoLeaves},~\ref{obsOrderOfSubtree},~\ref{obsUnnecessaryCutIntermediate},~\ref{obsUnnecessaryCut}, GreedyMin only has two options: it should either apply $Cut(V, j)$ for any $j \in V \setminus c(u, d^*_u)$ \HG{Why not $Cut(V, j)$ for $j \in V \setminus T_d(d^*_u)$} or perform $Join(V, d^*_u, l)$ for any $l \in Leaves(H_d) \setminus T_d(d^*_u)$. \HG{Why not $Join(V, t, l)$ for $t\in T_d(d^*_u)$. (this is not taken into account in your lemma)} \HG{It is not proven also that we must also consider leaves}. Now it can compare in which option $f_u$ is minimized the most. This step takes $O(n\Delta)$. \label{casePowerMin: k=1}
    
    \item $k=2$. Using Lemma~\ref{lmDelegatingu}, Observation~\ref{obsDelegatingtoLeaves},~\ref{obsOrderOfSubtree},~\ref{obsUnnecessaryCutIntermediate},~\ref{obsUnnecessaryCut}, GreedyMin follows two strategies. In the first strategy, it first performs $Join(V, d^*_u, l)$ for any leaf $l \in Leaves(H_d) \setminus T_d(d^*_u)$. Now, it follows Case~\ref{casePowerMin: k=1}. In the second strategy, for any $j \in T_d(d^*_u)$, it first performs the $Cut(V, j)$ operation and now proceeds as Case~\ref{casePowerMin: k=1}. \HG{I don't get why this would be optimal.} It takes $O(n^2\Delta)$ to realize which strategy minimizes $f_u$ the most. \label{casePowerMin: k=2} \HG{In any case, if $k\le 2$, you can try all possibilities.}
    
     \item If $k \ge 3$. In this case, GreedyMin first assumes that $k=2$ and then follows the same strategy stated in Case~\ref{casePowerMin: k=2}. Then it decreases the budget $k$ by $2$, i.e., $k=k-2$. Now if $k=1$, it follows Case~\ref{casePowerMin: k=1}; it follows Case~\ref{casePowerMin: k=2} otherwise. GreedyMin repeats this strategy until $k=0$. This takes $O(kn^2\Delta)$. 
\end{enumerate}



\begin{lemma}\label{lmIMinComplete}
GreedyMin solves \textbf{IMinP} optimally in $O(n^3\Delta)$ time when the social network is complete.
\end{lemma}

\begin{proof}
Using Lemma~\ref{lmDelegatingu}, Observation~\ref{obsDelegatingtoLeaves},~\ref{obsUnnecessaryCutIntermediate},~\ref{obsUnnecessaryCut}, to minimize $f_u$, we only need to apply a sequence of operations $Cut(V, j)$ and $Join(V,g,j)$, where in the first operation $j \in T_d(d^*_u) \setminus c_d(u, d^*_u)$, and in the second operation $g=d^*_u$ and $j \in Leaves(H_d) \setminus T_d(d^*_u)$. Keep in mind that after each delegation, the guru of $u$ will be updated. So, in each step, we only need to check which possible operation makes $u$ more powerless as GreedyMin does. Note that maybe there exists another algorithm $\mathcal{A}$ that delegates the guru of $u$ to the same set of subtrees as GreedyMin does but in a different order. Using Observation~\ref{obsOrderOfSubtree}, both GreedyMin and $\mathcal{A}$ work the same. Thus GreedyMin returns an optimal solution for \textbf{IMinP} in $O(n^3\Delta)$ as $k \le n$. 
\end{proof}

%GreedyMin returns an optimal solution to \textbf{IMinP} when $k=1,2$. It remains to show that this holds when $k \ge 3$. In the following, by having $d^*_u$ delegating to a subtree $T$, we mean that $d^*_u$ will delegate to one of the leaves $l \in T$ that minimizes $f_u$ the most. Let $T_i$ be the tree that $d^*_u$ delegating to it in the $i$'s step. Suppose that $T_1, T_2, ..., T_{k'}$ be the sequence of trees that GreedyMin selects to have $d^*_u$ delegating to them. Keep in mind that after each delegation, $d^*_u$ will be updated. Let $f^{T_i}_u$ be the index power of voter $u$ after delegating to subtree $ T_i$ in $i$'s step. Consider an optimal algorithm $\mathcal{A}$ for \textbf{IMinP}. Let $T'_1, T'_2, ..., T'_{k''}$ be the sequence of trees that algorithm $\mathcal{A}$ picks to have $d^*_u$ delegating to them. For the sake of simplicity, we suppose that $k'=k''$. Suppose that for any $j <i< k$, $T_j=T'_j$ in both GreedyMin and algorithm $\mathcal{A}$. Now assume that at step $j+1$, $T'_{j+1} \ne T_{j+1}$. We distinguish two cases.
%\begin{enumerate}
 %   \item $f^{T'_{j+1}}_u=f^{T_{j+1}}_u$. In this case, GreedyMin works optimally \HG{I would say this is wrong. Because even if $f^{T'_{j+1}}_u=f^{T_{j+1}}_u$, the fact that $T_{j+1}\neq T'_{j+1}$ could have an impact at further iterations of the algorithm.}.
    
  %  \item Otherwise, since GreedyMin selects each subtree with respect to $f^{T_i}_u$, $f^{T_{j+1}}_u < f^{T'_{j+1}}_u$. Since algorithm $\mathcal{A}$ is an optimal algorithm, it will select $T_{j+1}$ in the future \HG{Again this argument seems wrong to me or not explained because it is unclear that $f^{T_j+1}_u$ does not depend on previous choices}. By contradiction, suppose that for any $i \in j+2, \dots, k''$, $T'_{i} \ne T_{j+1}$. We see that $\mathcal{A}$ can replace one of $T'_{i}$ by $T_{j+1}$ to decrease $f_u$ more, which contradicts the assumption that $\mathcal{A}$ is an optimal algorithm. So, there exists $T'_{i}=T_{j+1}$ and by using Observation~\ref{obsOrderOfSubtree}$, \mathcal{A}$ could first have $u$ delegating to $T_{j+1}$ and then to $T'_{j+1}, T'_{j+2}, \dots, T'_{i-1}$.
%\end{enumerate}

==> NewResults.tex <==
\section{New Results}


\subsection{On Axiomatic Properties}
Consider a delegation graph $H_d$ and two voters $i, j \in V$ such that $i \in c_d(j, d^*_{j})$ (i.e., $i$ is an ancestor of $j$). In the next step, we introduce a new axiom which says that in a new delegation graph $d'$ obtained from $d$ in which all voters have the same delegation strategies as $d$ except that $j$ delegates to a voter $l \in c_d(j, d^*_j) \setminus c_d(i, d^*_i)$, $i$ gets more powerful. In other words, this axiom says that if the people who support a specific voter $i$, support $i$ through a smaller set of intermediaries, $i$ gets more powerful.

\begin{axiom}[Monotonicity w.r.t. Intermediaries (\textbf{MI})]
Consider two LDEs $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$ and $\mathcal{E}' = \langle D', \omega', d', q' \rangle$ and three agents $i,j, k \in V$ such that $k \in c_d(j, d^*_j)$, $i \in c_d(k, d^*_k)$, $\forall l\in V\setminus \{j\}, d_l=d'_l$ and $d'_j=k$, $D=D'$, $\omega = \omega'$ and $q=q'$. Then, $f_i(\mathcal{E}') \ge f_i(\mathcal{E})$. 
\end{axiom}

\begin{proposition}\label{prMonotonicityIntermediary}
The delegative Banzhaf and Shapley-Shubik indices satisfy axiom \textbf{MI}.
\end{proposition}
\begin{proof}
One may use the same argument as that of Proposition~\ref{prMonotonicityDirectDelegation} to prove the proposition.% Consider two LDEs $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$ and $\mathcal{E}' = \langle D', \omega', d', q' \rangle$ and three agents $i,j, k \in V$ such that $k \in c_d(j, d^*_j)$, $i \in c_d(k, d^*_k)$, $\forall l\in V\setminus \{j\}, d_l=d'_l$ and $d'_j=k$, $D=D'$, $\omega = \omega'$ and $q=q'$. Let us consider a coalition $C\subseteq V\setminus\{i\}$ such that $\nu_{\mathcal{E}}(C \cup\{ i \}) - \nu_{\mathcal{E}}(C) = 1$. This implies that $c_d(i,d_i^*)\subseteq C\cup\{i\}$. 
%From $\nu_{\mathcal{E}}(C \cup\{ i \}) = 1$, it is straightforward that $\nu_{\mathcal{E}'}(C \cup\{ i \}) = 1$ as $d(l) = d'(l)$ for $l\neq j$, $d'(j)=k \in c_d(i,d_i^*)$ and $c_d(i,d_i^*)\subseteq C\cup\{ i \}$. Moreover, from $\nu_{\mathcal{E}}(C) = 0$, it is also easy to see that $\nu_{\mathcal{E}'}(C) = 0$ as $d(l) = d'(l)$ for $l\neq j$, $d'(j)=k \in c_d(i,d_i^*)$ and $i\not\in C$. 
%Because this reasoning holds for any coalition for which $i$ is a swing agent, we obtain that  $DS_i(\mathcal{E}') \ge DS_i(\mathcal{E})$ and $DB_i(\mathcal{E}') \ge DB_i(\mathcal{E})$. 
\end{proof}

\subsection{On \textbf{BMaxP} and \textbf{SMaxP}}

We show that \textbf{BMaxP} and \textbf{SMaxP} are in-approximately on trees.

\begin{theorem}
\textbf{BMaxP} and \textbf{SMaxP} are in-approximately on trees.
\end{theorem}

\begin{proof}
Consider a general version of the Partition problem. Given a set of items $S=\{a_1, \dots, a_n\}$, and two integers $M$ and $l$. We say that $I'=\langle S, M, k\rangle$ is a ``yes''-instance of the Partition problem if there exists a subset $J \subseteq S$ such that $\sum_{a_i \in J}a_i=M$ and $|J|\le l$. To prove the theorem, we transform an instance $I'=\langle S, M, k\rangle$ of the Partition problem to an instance $I=\langle \mathcal{E} = \langle D= (V, A), \omega, d , q \rangle , v^*, k, \tau \rangle$ of \textbf{BMaxP} (resp. \textbf{SMaxP}). We create a tree $D$ where: 
\begin{itemize}
    \item $V = V_1 \cup V_2 \cup \{v^*\}$ with $V_1 = \{u_i : a_i \in S\}$ and $V_2=\{v, v_1,\dots, v_l\}$.
    \item $ A = \{(u_i, v): a_i \in S \} \cup \{(v_i, v_{i+1}): i \in [l-1]\} \cup \{(v, v_1)\} \cup \{(v_l, v^*)\}$.
\end{itemize}

We set $q=2M+1$, $k=l$ and $\tau=1/2^N$ for \textbf{BMaxP} ($\tau=\frac{1}{N!}$ for \textbf{SMaxP}), where $N=|V|$. The weight function $\omega$ is set as follows. $\omega(v^*)=1$, $\omega(u_i)=2a_i$ for any $u_i \in V_1$, $\omega(v_j)=0$ for any $v_j \in V_2\setminus\{v\}$ and $\omega(v)=2M+1$. The initial delegation function $d$ is set as follows. $d_{v^*}=v^*$, $d_{u_i}=v$ for any $u_i \in V_1$ and $d_{v_j}=v_j$ for any $v_j \in V_2$. We say that $I$ is a ``yes''-instance of \textbf{BMaxP} (resp. \textbf{SMaxP}) if there exists another delegation function $d'$ obtained from $d$ such that $DB_{v^*}(\mathcal{E}') \ge \tau=1/2^N$ (resp. $DS_{v^*}(\mathcal{E}') \ge \tau=\frac{1}{N!}$), where $\mathcal{E}' = \langle D= (V, A), \omega, d' , q \rangle$ and $|\{i\in V : d(i)\neq d'(i)\}|\le k$.

Now we show that $I'$ is a ``yes''-instance of the Partition problem if and only if $I$ is a ``yes''-instance of \textbf{BMaxP} (resp. \textbf{SMaxP}). Indeed, suppose that there is a subset $J \subseteq S$ of size $l$ such that $\sum_{a_i \in J}a_i=M$. Then we obtain a delegation function $d'$ from $d$ as follows. Let $V'=\{u_i:a_i \in J\} \subseteq V_1$. We set $d'_{u_i}=u_i$ for any $u_i \in V'$ and $d'_{v'}=d_{v'}$ for any $v' \in V\setminus V'$. So, $\omega(V')=2M$ and $\omega(V' \cup\{v^*\})=2M+1=q$, implying that $v^*$ is a swing agent for at least one coalition, i.e., $DB_{v^*}(\mathcal{E}') \ge \tau=1/2^N$ (resp. $DS_{v^*}(\mathcal{E}') \ge \tau=\frac{1}{N!}$). Conversely, suppose that $DB_{v^*}(\mathcal{E}') \ge \tau=1/2^N$ (resp. $DS_{v^*}(\mathcal{E}') \ge \tau=\frac{1}{N!}$) in $\mathcal{E}' = \langle D= (V, A), \omega, d' , q \rangle$ and $|\{i\in V : d(i)\neq d'(i)\}|\le k$, then there is some winning coalition $C$ for which $v^*$ is swing in. Then we have $\omega(C\setminus\{v^*, V''\})=2M$, where $V''$ is the set of all inactive voters in $C$. Note that: 1) for any coalition $C$ for which $v^*$ is swing in we have $\omega(C\setminus\{v^*, V''\})=2M$ since $\omega(v^*)=1$, 2) all voters in $V_2\setminus\{v\}$ have weight $0$ and can join $C$ as in active voters and 3) voters who follow $v$ in $H_{d'}$ can only join $C$ as inactive voters as $\omega(v)=2M+1=q$. Let $S'=\{a_i:u_i \in C\setminus\{v^*, V''\}\}$. Then we have $\sum_{a_i \in S'}a_i=M$. This concludes the proof.
\end{proof}

In the next step, when the input is a complete graph and voters have an identical weight, we provide an approximation algorithm for \textbf{BMaxP} and \textbf{SMaxP}. The algorithm works as follows. It iteratively picks the guru $g$ with the maximum weight (if there are some gurus with the same weight, it selects one of them arbitrarily), set $d_g=v^*$ and $k=k-1$. This process continues until $k=0$ or no guru remains to delegate to $v^*$. We call this algorithm GAMW, standing for Greedy Algorithm with Maximum Weight. Let $t_{v^*}(r) \subseteq t_{v^*}$ be a subtree of size $r$ rooted in $v^*$, where $r \in \{1,\dots, |t_{v^*}|\}$. Keep in mind that all voters have the same weight.

\begin{theorem}\label{thApproximationAlgorithmMaximumWeight}
Consider an unsuccessful coalition $C\subseteq V \setminus t_{v^*}$. Let $r\in \{1,\dots, |t_{v^*}|\}$ be the minimum number such that $C'=C\cup t_{v^*}(r)$ is an successful coalition. GAMW is a factor $\frac{1}{2^{n+r-s-1}}$ (resp. $\frac{2^{s-r}}{n!}$) approximation algorithm for \textbf{BMaxP} (resp. \textbf{BMaxP}) on complete graphs, where $s$ is the total number of voters delegating to $v^*$ in GAMW. %selected by GAMW to delegate to $v^*$ (directly or indirectly).
\end{theorem}

To prove Theorem~\ref{thApproximationAlgorithmMaximumWeight}, we need some observations. Consider an LDE $\mathcal{E}$ and let $t_{v^*}(\mathcal{E})$ be the subtree rooted in $v^*$ in $\mathcal{E}$. Let $\mathcal{J}$ be all LDEs $\mathcal{E}$ in which $v^*$ is a guru, for any two distinct LDEs $\mathcal{E}_i=\langle D^i = (V , A), \omega^i, d^i, q^i \rangle$ and $ \mathcal{E}_j=\langle D^j = (V , A), \omega^j, d^j, q^j \rangle$ in $\mathcal{J}$, $t_{v^*}(\mathcal{E}_i)=t_{v^*}(\mathcal{E}_j)$, for any voter $v \in V\setminus t_{v^*}(\mathcal{E}_i)$ (or $v \in V\setminus t_{v^*}(\mathcal{E}_j)$), $d^i_v=d^j_v$, $q^i=q^j$ and for any $v' \in V$, $\omega^i(v')=\omega^j(v')$. Let $\mathcal{E}_{min}=\min_{\mathcal{E} \in \mathcal{J}} f_{v^*}(\mathcal{E}), \mathcal{E}_{max} =\max_{\mathcal{E} \in \mathcal{J}} f_{v^*}(\mathcal{E})$, i.e., $v^*$ has the minimum power in  $\mathcal{E}_{min}$ and maximum power in $\mathcal{E}_{max}$. Then, we have

\begin{obs}\label{obsMinandMaxPossiblePower}
In $\mathcal{E}_{min}$ ($\mathcal{E}_{max}$), $t_{v^*}(\mathcal{E}_{min})$ (resp. $t_{v^*}(\mathcal{E}_{max})$) is a path (resp. a star) with length $|t_{v^*}(\mathcal{E}_{min})|$ (resp. with $|t_{v^*}(\mathcal{E}_{min})|-1$ leaves).
\end{obs}

\begin{proof}
First note that $t_{v^*}(\mathcal{E}_{min})=t_{v^*}(\mathcal{E}_{max})$ as $\mathcal{E}_{min}, \mathcal{E}_{max} \in \mathcal{J}$. By Propositions~\ref{prMonotonicityDirectDelegation} and~\ref{prMonotonicityIntermediary}, one can prove the observation.
\end{proof}

We need to find an upper bound on the optimal solution. To do so, we propose another algorithm, called VBCA, stands for Violated Budget Constraint Algorithm in which the budget constraint maybe violated. In particular, VBCA constructs a delegation graph $H_{d''}$ obtained from the input delegation graph $H_d$ in which we may have $|\{i\in V : d(i)\neq d''(i)\}|\ge k$ (i.e, it my violate the budget constraint) as follows. Let $t_i$ be the subtree (i.e., $t_i$ represents guru $g_i$) that is selected by GAMW at iteration $i$. In VBCA, all voters in $t_i$ delegate to $v^*$ directly. So, VBCA outputs a delegation graph $H_{d''}$ in which $s$ voters delegate to $v^*$ directly. Recall that $s=|\bigcup_{t \in T'}t_i|$ where $T'$ is the set of subtrees selected by GAMW to delegate to $v^*$. We show that VBCA outputs a delegation graph $H_{d''}$ in which $v^*$'s delegative Banzhaf and delegative Shapley-Shubik value is an upper on the optimum solutions to \textbf{BMaxp} and \textbf{SMaxP}.


\begin{lemma}\label{lmViolatedBudgetConstraint}
Let $DB''_{v^*}$ (resp. $DS''_{v^*}$) be the value for \textbf{BMaxP} (resp. \textbf{SMaxP}) in VBCA. Then, $DB''_{v^*} \ge OPT$ (resp. $DS''_{v^*} \ge OPT'$), where $OPT$ (resp. $OPT'$) is the optimum $v^*$'s delegative Banzhaf (resp. delegative Shapley-Shubik) value, when respecting the budget constrain.
\end{lemma}

\begin{proof}
Recall that in VBCA a subtree $t_i$ with the maximum number of voters is selected at each iteration. Consider an optimal algorithm $OA$ for \textbf{BMaxP} (and \textbf{BMaxP}), which respects the budget. Let $t'_i$ be the subtree selected by $OA$ at each iteration $i$. Obviously, we have $|t_i| \ge |t'_i|$. As all voters in $t_i$ delegate to $v^*$ directly, by Proposition~\ref{prMonotonicityDirectDelegation}, at each iteration $i$, $v^*$ in VBCA is more powerful than $v^*$ in $OA$. This concludes the proof. 
\end{proof}

\begin{obs}\label{obsSameDelegation}
Let $H_{d'}$ and $H_{d''}$ be the delegation graphs output by GAMW and VBCA. Let $t_{v^*}(GAMW)$ (resp. $t_{v^*}(VBCA)$) be the subtree rooted in $v^*$ in GAMW (resp. VBCA). Then, $H_{d'} \setminus t_{v^*}(GAMW)=H_{d''}\setminus t_{v^*}(VBCA)$.
\end{obs}

\begin{proof}
Let $H_d$ be the initial delegation graph. Let $S=\{t_1,\dots, t_{k'}\}$ be all trees picked by GAMW to delegate to $v^*$. Since at each iteration VBCA only delegates all voters in tree $t_i \in S$ to $v^*$. Then $H_d\setminus S$ remain unchanged. We conclude by noticing that $t_{v^*}(GAMW)=t_{v^*}(VBCA)=S$.
\end{proof}


Now we are ready to prove Theorem~\ref{thApproximationAlgorithmMaximumWeight}.

\begin{proof}[Proof of Theorem~\ref{thApproximationAlgorithmMaximumWeight}]
Let $H_{d'}$ be the delegation graph output by GAMW. First note that for any guru $g \in Gu_{d'}$, $\alpha_d(g) \le \alpha_d(v^*)$, as the guru with the maximum weight in GAMW is chosen to delegate to $v^*$ and the budget $k \ge 1$. %Let $H_{d'}$ be the delegation graph output by an optimal algorithm for \textbf{BMaxP}. Obviously, $\alpha_{d'}(v^*) \le \alpha_d(v^*)$, otherwise it contradicts the assumption that GAMW picks the guru with the maximum weight to delegate to $v^*$. 
Let $H_{d''}$ be the delegation graph output by VBCA. Consider the LDE $\mathcal{E}'=\langle D = (V , A), \omega, d', q \rangle$ and let $|t_{v^*}(\mathcal{E}')|=s$. We will use $t_{v^*}(\mathcal{E}')$ and $t_{v^*}(GAMW)$ interchangeably.
By Observation~\ref{obsMinandMaxPossiblePower}, $t_{v^*}(GAMW)$ is a path of length $s$ in the worst case. Recall that $r$ is the minimum number of $v^*$'s followers required to make a coalition $C\setminus t_{v^*}$ a winning coalition.

Let us first focus on the approximation factor of GAMW for \textbf{BMaxP}. Since $t_{v^*}(GAMW)$ is a path there exists only one subtree in $t_{v^*}(GAMW)$ having a weight $w \in \{r, \dots, \alpha_d(v^*)\}$. Let $r'\in \{r, \dots, s-1\}$ be the number of $v^*$'followers who join a coalition $C$ as active voters to have $C$ successful. Thus, for any $r'$, $2^{s-r'-1}$ followers of $v^*$ can join $C$ as inactive voters since $t_{v^*}$ is a path of length $s$. This implies that the total number of coalitions that $v^*$ can be swing in is at least $1+2+2^2+\dots+2^{s-r-1}$. Since in VBCA all voters delegate to $v^*$ directly, for any $r'$, ${s \choose r'}$ followers of $v^*$ can join $C$ as active voters. Let $N_{r'}$ be the number of unsuccessful coalitions $C \subseteq \setminus t_{v^*}$ such that after joining subtree $t \subseteq t_{v^*}$ of size $r'$ to $C$, coalitions $C'=C \cup t$ become successful. Note that by Observation~\ref{obsSameDelegation}, for any $r'$, the number of such coalitions $C$, i.e., $N_{r'}$, for two algorithms GAMW and VBCA are equal. Thus, we have
\begin{align*}
    \frac{2^{s-r-1}+2^{s-r}+\dots +2^1+1+1}{{s \choose r}+{s \choose r+1}+\dots+ {s \choose s}} \times \frac{1}{2^{n-s}}\\\ge \frac{2^{s-r}}{2^{n-1}}=\frac{1}{2^{n+r-s-1}}.
\end{align*} 

By Lemma~\ref{lmViolatedBudgetConstraint}, we conclude the proof for \textbf{BMaxP}. 

We now turn our attention to analyze the approximation factor of GAMW for \textbf{SMaxP}. Recall that a subtree $t \subseteq t_{v^*}$ of size  at least $r$ has to join an unsuccessful coalition $C \subseteq V\setminus t_{v^*}$ to make it successful. Now let $\pi$ be a permutation of all voters and $\pi_i$ be the voters who precede $i$ in $\pi$. Then $v^*$ is pivotal for $\pi_{v^*} \cup \{v^*\}$ if $t_{v^*}(r) \subseteq \pi_{v^*}$. Recall that, by Observation~\ref{obsMinandMaxPossiblePower}, in the worst case, $t_{v^*}$ is a path in GAMW, then the number of subsets $t_{v^*}$ of size $s' \in \{r, \dots, s\}$ such that $v^*$ is pivotal for $\pi$ is $s-r \choose s'-r$. In other words, the number of permutations $\pi$ in which subtrees $t_{v^*}(s') \subseteq \pi_{v^*}$ and $v^*$ is pivotal is $s-r \choose s'-r$ in GAMW. Then, GAMW returns at least the value $DS_{v^*}(GAMW) \ge \frac{\sum_{s'=r}^{s}{s-r \choose s'-r}}{n!}=\frac{2^{s-r}}{n!}$ as a solution to \textbf{SMaxP}. We conclude by noticing that $DS_{v^*} \le 1$ in an optimal solution.
%As for any guru $g \in Gu_d$, $\alpha_d(g) \le \alpha_d(v^*)$, for any subtree $t \subseteq t^*(\mathcal{E})$ rooted in $v^*$ with a weight $w$, there exists at least one coalition $C \subset V\setminus t$, where $v^*$ is a swing agent in. Let $|t|=s'\le s$. Note that $s'$ is the number of active agents in $C$ from $t_{v^*}(\mathcal{E})$. Hence, $s-s'-1$ (when $s' \le s-1$) voters from $t_{v^*}(\mathcal{E})$ can join $C$ as inactive agents when $t \subseteq C$. This implies that the total number of coalitions that $v^*$ can be swing in is $1+2+2^2+\dots+2^{s-2}=O(2^{s-2})$. We know that in an optimal solution, there are at most $2^{n-1}$ coalitions that $v^*$ can be swing in. This concludes the proof.
    
    %\item $q \le |t_{v^*}(\mathcal{E})|$. One may use the same analysis of the previous case and achieve the same ratio as the previous case.
%\end{enumerate}

%By considering the two cases, the proof is complete.
\end{proof}


\subsection{On \textbf{WmaxP}}
We call the optimization version of \textbf{WmaxP}, \textbf{OWmaxP}. Surprisingly, a more general case of \textbf{OWmaxP}, called \textbf{DTO}, has been investigated by Ghuge and Nagarajan~\cite{ghuge2020quasi}. %Now we aim to show that \textbf{OWmaxP} is closely related to \textbf{DTO}, which is studied by Ghuge and Nagarajan~\cite{ghuge2020quasi}. 
In \textbf{DTO}, we are given a directed graph $D=(V, A)$ with edge costs $c:E \rightarrow \mathbb{Z}^{+}$, a root vertex $r^* \in V$, a budget $B$, and a weight function $\omega:V \rightarrow \mathbb{Z}$. For any subgraph $G'$ of $G$, let $V(G')$ and $E(G')$ represent the set of nodes and edges in $G'$. The goal here is to find an out-directed arborescence $T^*$ rooted at $r^*$ maximizing $\omega(V(T^*))$ such that $\sum_{e \in E(T^*)} c(e) \le B$. Ghuge and Nagarajan~\cite{ghuge2020quasi} provided a quasi-polynomial time $O(\frac{\log n'}{\log \log n'})$-approximation algorithm for \textbf{DTO}, where $n'$ is the number of vertices in an optimal solution. Note that the authors mentioned that this factor is tight for \textbf{DTO}. It is worth mentioning that the undirected version of \textbf{DTO} has been investigated by Paul et al.~\cite{paul2020budgeted}, termed \textit{budgeted prize-collecting minimum spanning tree}, in which we are given an undirected graph and the task is to find a tree $T^*$ containing a root vertex $r^*$ with the maximum weight $\omega(T^*)$ such that $c(T^*) \le B$. Paul et al.~\cite{paul2020budgeted} proposed a 2-approximation algorithm for budgeted prize-collecting minimum spanning tree.

Here we show that any approximation algorithm for a specific version of \textbf{DTO} also can solve \textbf{OWmaxP}, preserving
the approximation factor. In particular, consider special instances $I'=\langle D'= (V', A'), r^*, c, f, B \rangle$ of \textbf{DTO}, where for any edge $e \in A'$, $c(e)=\{0, 1\}$. More importantly, there is no cycle $C$ in $D'$ with total cost $\sum_{e \in E(C)}c(e)=0$, i.e., there exists at least one edge $e \in C$ with $c(e)=1$. For any node $v \in V'$, there exists at most one incoming edge $e$ of cost $c(e)=0$. %for any $e \in E(C)$, $c(e)=0$, i.e., $\sum_{e \in C}c(e)=0$. %there exists at least one edge $e \in C$ with $c(e)=1$. 
%Also, for any $S \subseteq V'$, $f(S)=\sum_{i \in S}w_i$, where $w_i$ is the weight of $i \in V'$. %the cost of each outgoing edge is either $1$ or $0$.
Let us call \textbf{DTO} on these restricted instances \textbf{RDTO}.

%\paragraph{Connections to \textbf{STO}.} 

\begin{theorem}
Let $\alpha$, $0<\alpha<1$, be a constant. The following statements are equivalent:

\begin{enumerate}
    \item[(i)] There is an $\alpha$-approximation algorithm for \textbf{RDTO}.\label{alpha-RDTO}
    
    \item[(ii)] There is an $\alpha$-approximation algorithm for \textbf{OWmaxP}.\label{alpha-WmaxP}
\end{enumerate}
\end{theorem}

\begin{proof}
To prove that (i) implies (ii), we proceed as follows. Let $I=\langle D= (V, A), \omega, d,i^*, k \rangle$ be an instance of \textbf{OWmaxP}. Without loss of generality, we suppose that $d_{i^*}=i^*$; otherwise we define a new delegation graph $d'$ such that $d'_{i^*}=i^*$, $d'_i=d_i$ for any $i \in V \setminus \{i^*\}$ and $k=k-1$. Let $I'=\langle D'= (V', A'), r^*, c, f, B \rangle$ be an instance of \textbf{RDTO} obtained from $I$ as follows. We set $V'=V$, $r^*=i^*$ and $A'=\{(i,j):(j,i) \in A\}$, i.e., we reverse the edges. For any $e=(i,j) \in A'$ in $I'$, if $d(j)=i$ in $I$, $c(e)=0$; $c(e)=1$ otherwise. For any $S \subseteq V'$, let $f(S)=\sum_{i \in S}\omega(i)$. Lastly, $B=k$. Consider a solution $T^*$ to \textbf{RDTO} on $I'$. We can simply reverse the edges in $T^*$ and obtain a subtree rooted in $i^*=r^*$ with the maximum weight such that $c(T^*) \le B=k$ in $I'$. We conclude by noticing that any edge $e=(i, j) \in E(T^*)$ either costs $0$ if $d(j)=i$ or $1$ otherwise.

To prove that (ii) implies (i), we give a polynomial-time reduction from \textbf{RDTO} to \textbf{OWmaxP} as follows. Let $I'=\langle D'= (V', A'), r^*, c, f, B \rangle$ be an instance of \textbf{RDTO}. Let $I=\langle D= (V, A), \omega, d,i^*, k \rangle$ be an instance of \textbf{OWmaxP} obtained from $I'$ as follows. We set $V'=V$, $r^*=i^*$ and $A=\{(i,j):(j,i) \in A'\}$, i.e., reversing edges. For any voter $i \in V \setminus \{i^*\}$ if there exists an incoming edge $e=(j, i) \in A'$ with cost $c(e)=0$, we set $d_i=j$; $d_i=i$ otherwise. We set $d_{i^*}=i^*$. For any $i \in V$, let $\omega(i)=w_i$. Lastly, we set $k=B$. As there exists no cycle $C \in D'$ with $\sum_{e \in C}c(e)=0$ and for any $i \in V'$ there is at most one incoming edge $e$ with cost $c(e)=0$, the resulting delegation graph $H_d$ is feasible. Now consider another delegation graph $H_{d'}$ such that $|\{i\in V : d(i)\neq d'(i)\}|\le k$ and $\alpha_{d'}(i^*)$ being maximized. By reversing the edges in subtree rooted at $i^*$ in $H_{d'}$ we get an arborescence $T^*$ that is rooted at $r^*$ with maximum $f(V(T^*))$ in $I'$.
\end{proof}



==> old/Conclusion.tex <==
\section{Conclusion}
Following a recent work by Zhang and Grossi~\cite{zhang2020power}, we investigated the delegative Banzhaf and Shapley-Shubik indices. We proposed a pseudo-polynomial time algorithm to compute these power indices. % and could characterize the delegative Shapley-Shubik index.
Moreover, we investigated a bribery problem in which we aim to maximize/minimize the power index or the voting power of a given voter. We showed that the destructive problem where one attempts to decrease the voter's power is NP-hard even when the weights of all voters are identical to one. In the constructive version, we proved that maximizing the agent's power is NP-hard even when voters' weights and the quota are given in unary. These hardness results comes from the fact that an agent's power does not only depend on the voting weight distribution, but also on the structure of the supports she receives from her followers. So, we considered a seemingly easier version of the constructive problem, where the goal is to maximize the voting weight of the agent. For this problem, we were able to show that designing an approximation algorithm with approximation ratio better than $1-1/e$ is not possible, unless P=NP and we also provided some parameterized complexity results. Lastly, we proved that finding a delegation graph with a certain number of gurus that maximizes the minimum power an agent can have is an NP-hard problem.

Several directions of future work are conceivable. First, for both destructive and constructive problems, designing some algorithms that would provide approximation guarantees under some conditions is one direction. It would be interesting to investigate problems related to distribution of power among agents as finding a delegation graph with a fixed number of gurus that maximizes the minimum power a guru has. 


==> old/Contribution/Characterisation/axiom.tex <==

\section{Axiomatic Properties of $DS$}

In this section, we provide further properties of the delegative Shapley-Shubik index. 
We follow notations and techniques from several other papers in the literature~\cite{barua2005new,chalkiadakis2011computational, einy2011characterization, neyman1989uniqueness, shapley1953value,zhang2020power}. 
Let $\nu_{\mathcal{E}}$ be the characteristic function of a delegative simple game $\mathcal{G}_{\mathcal{E}}$ induced by an LDE $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$. In the following $f$ denotes a generic delegative power measure and $f_i$ is the delegative power index value of agent $i$.


\begin{definition}[Dummy Agent]\label{defDummy}
An agent $i \in V$ is called a \emph{dummy} agent if for any $C \subseteq V$, $\nu_{\mathcal{E}}(C)=\nu_{\mathcal{E}}(C\setminus \{i\})$.
\end{definition}

Put another way, when a voter $i$ cannot contribute anything to any coalition of $V$, she is said to be a dummy agent. For instance, an agent is dummy when she is a distant agent. %Moreover, when all voters have weight one For instance, an agent is dummy iff she is a distant agent.
In Example~\ref{exNotations}, voter $5$ is a distant agent, so she is dummy.

\begin{definition}[Efficient Index Power]\label{defEfficiency}
An index power $f$ is said to be \emph{efficient} if $\sum_{i\in V}f_i(\mathcal{E})=\nu_\mathcal{E}(V)$.
\end{definition}


\begin{definition}[Symmetric Agents]\label{defSymmetry}
Two agents $i$ and $j$ are said to be \emph{symmetric} if for any coalition $C\subseteq V\setminus \{i,j\}$, $\nu_\mathcal{E}(C\cup \{i\})=\nu_\mathcal{E}(C\cup \{j\})$.
\end{definition}

That is, two voters are symmetric if they both are pivotal for the same coalitions of $V$. For example, voters $1$ and $2$ are symmetric in Example~\ref{exNotations} as they are pivotal for the same coalitions. We borrow the following two definitions from Zhang and Grossi~\cite{zhang2020power}. 
%\begin{definition}[Unanimity]
%$\mathcal{E}$ is a unanimity LDE if $q=\sum_{i \in V}\omega(i)$, denoted by $\mathcal{UE}$.
%\end{definition}

%Thus, in a unanimity delegative simple game $\mathcal{G}_{\mathcal{UE}}$, a coalition $C$ wins if $\alpha_d(C) \ge \sum_{i \in V}\omega(i)$.

\begin{definition}[Composition]\label{defComposition}
Let two LDEs $\mathcal{E}_1 = \langle D_1 = (V_1 , A_1), \omega_1, d^1, q_1 \rangle$ and $\mathcal{E}_2 = \langle D_2 = (V_2 , A_2), \omega_2, d^2, q_2 \rangle$, such that for any $i \in V_1\cap V_2$, if $d^1(i)=j$ (resp. $d^2(i)=j$), then $j\in V_2$ (resp. $j \in V_1$) and $d^2(i)=j$ (resp. $d^1(i)=j$), and $\omega_1(i)=\omega_2(i)$. We define two new delegative simple games $\mathcal{E}_1 \land \mathcal{E}_2=\langle D_{1\land 2}(V_1 \cup V_2, A_1 \cup A_2), \omega_{1\land 2}, d_{1\land 2}, q_1 \land q_2 \rangle$ and $\mathcal{E}_1 \lor \mathcal{E}_2=\langle D_{1\lor 2}(V_1 \cup V_2, A_1 \cup A_2), \omega_{1\lor 2}, d_{1\lor 2}, q_1 \lor q_2 \rangle$, where:

\begin{itemize}
    \item for any $i \in V_1$ (resp. $i \in V_2$), $\omega_{1\lor 2}(i)=\omega_{1 \land 2}(i)=\omega_1(i)$ (resp. $\omega_{1\lor 2}(i)=w_{1 \land 2}(i)=\omega_2(i)$);
    
    \item for any $i \in V_1 \setminus V_2$ (resp. $V_2\setminus V_1$), $d_{1\lor 2}(i)=d_{1 \land 2}(i)=d^1(i)$ (resp. $d_{1\lor 2}(i)=d_{1 \land 2}(i)=d^2(i)$), and for any $i \in V_1 \cap V_2$, as $d^1(i)=d^2(i)$ by initial conditions, then $d_{1\lor 2}(i)=d_{1 \land 2}(i)=d^1(i)=d^2(i)$;%, otherwise $d_{1\lor 2}(i)=d_{1 \land 2}(i)=d^k(i)$ where $k \in \{1,2\}$ and $d^k(i)\ne 0$;
    
    \item $q_1\land q_2$ (resp. $q_1\lor q_2$) is met iff $\sum_{i \in \hat{D}(C\cap V_1)}\omega_1(i)\ge q_1$ and (resp. or) $\sum_{i \in \hat{D}(C\cap V_2)}\omega_2(i)\ge q_2$.

\end{itemize}
\end{definition}

Put another way, when two LDEs $\mathcal{E}_1$ and $\mathcal{E}_2$ coincide in their intersection, by composing $\mathcal{E}_1$ and $\mathcal{E}_2$, we obtain two new LDEs $\mathcal{E}_1 \land \mathcal{E}_1$ and $\mathcal{E}_1 \lor \mathcal{E}_2$. Let $\mathcal{G}_{\mathcal{E}_1 \lor \mathcal{E}_2}$ (resp. $\mathcal{G}_{\mathcal{E}_1 \land \mathcal{E}_2}$) be the delegative simple game induced by $\mathcal{E}_1 \lor \mathcal{E}_2$ (resp. $\mathcal{E}_1 \land \mathcal{E}_1$). In $\mathcal{G}_{\mathcal{E}_1 \lor \mathcal{E}_2}$ (resp. $\mathcal{G}_{\mathcal{E}_1 \land \mathcal{E}_2}$), a coalition $C \subseteq V_1 \cup V_2$ wins if $C$ wins in $\mathcal{G}_{\mathcal{E}_1}$ or (resp. and) $\mathcal{G}_{\mathcal{E}_2}$. Note that according to our setting, Definition~\ref{defComposition} does not consider the case where voters abstain, which is the only difference between Definition~\ref{defComposition} and the one given by Zhang and Grossi~\cite{zhang2020power}. 

\begin{definition}[Bloc formation]
Given $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$ and for any $i,j \in V$ such that $d(i)=j$ or $i,j \in Gu_d$, $\mathcal{E}' = \langle D' = (V' , A'), \omega', d', q' \rangle$ is called the bloc LDE joining $i$ and $j$ into a bloc $ij$, where 
\begin{itemize}
    \item $V'=V\cup \{ij\}\setminus \{i,j\}$;
    
    \item %Let $N_{ij}=\mathtt{Nb}_{in}(i) \cup \mathtt{Nb}_{out}(i) \cup \mathtt{Nb}_{in}(j) \cup \mathtt{Nb}_{out}(j)$. 
    Let $E_{ij}=\{(a_1,i),(i,a_2),(j,b_1),(b_2,j)| a_1\in\mathtt{Nb}_{in}(i), a_2\in \mathtt{Nb}_{out}(i),b_1 \in \mathtt{Nb}_{out}(j),b_2 \in \mathtt{Nb}_{in}(j)\}$. Let $A''=\{(ij, a), (b, ij)| a \in \mathtt{Nb}_{out}(i) \cup \mathtt{Nb}_{out}(j) \setminus\{i,j\} \text{ and } b \in \mathtt{Nb}_{in}(i) \cup \mathtt{Nb}_{in}(j)\setminus\{i,j\} \}$. Then, $A'=A \cup A''\setminus E_{ij}$.
    
    \item for $d'$, for any $a \in V\setminus\{i,j\}$, such that $d(a)=i$ or $d(a)=j$, $d'(a) = ij$; if $d(i) = j$, and $j\notin Gu_d$, then $d'(ij)=d(j)$, else $d'(ij)=ij$. %if $d_i=j$, $d'_{ij}=d_j$, and for any $a \in V$, such that $d_a=i$ or $d_a=j$, $d'_a=ij$, but if $i,j \in Gu_d$, for any $a \in V$ such that $d_a=i$ or $d_a=j$, $d'_a=ij$;
    
    \item $\omega'(ij)=\omega(i)+\omega(j)$.
\end{itemize}
\end{definition}

When two voters $i$ and $j$ are adjacent or they are both gurus, i.e., $i,j \in Gu_d$, a bloc LDE joins $i$ and $j$, and considers them as a new agent $ij$.

We are now in position to present several axioms. %involved in our characterization.

\begin{axiom}[Dummy Player (\textbf{DP})]\label{axiomDP}
If $i$ is a dummy player, then $f_i(\mathcal{E})=0$.
\end{axiom}

\begin{axiom}[Efficient Index (\textbf{EI})]\label{axiomEI}
For any LDE $\mathcal{E}$, $\sum_{i\in V}f_i(\mathcal{E})=\nu_\mathcal{E}(V)$.
\end{axiom}

\begin{axiom}[Symmetric Agents (\textbf{SA})]\label{axiomSA}
If agents $i$ and $j$ are symmetric, $f_i(\mathcal{E})=f_j(\mathcal{E})$.
\end{axiom}

\begin{axiom}[Sum Principle (\textbf{SP})]\label{axiomSP}
For any two LDEs ${\mathcal{E}}_1$ and ${\mathcal{E}}_2$, such that any $i \in V_1 \cup V_2$ satisfies the condition in Definition~\ref{defComposition}, $f_i(\mathcal{E}_1 \land \mathcal{E}_2)+f_i(\mathcal{E}_1 \lor \mathcal{E}_2)=f_i(\mathcal{E}_1)+f_i(\mathcal{E}_2)$.
\end{axiom}

\begin{axiom}[Bloc Principle (\textbf{BP})]\label{axiomBP}
For any two agents $i,j \in V$ such that $d(i) = j$, or $i, j \in Gu_d$, let $\mathcal{E}'$ be the bloc LDE obtained by joining $i$ and $j$ into bloc $ij$. Then $f_{ij}(\mathcal{E}')=f_i(\mathcal{E})+f_j(\mathcal{E})$.
\end{axiom}

\begin{axiom}[Monotonicity w.r.t. Direct Delegations (\textbf{MDD})]
Consider two LDEs $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$ and $\mathcal{E}' = \langle D', \omega', d', q' \rangle$ and two agents $i,j \in V$ such that $j \not\in  c_d(i,d_i^*)$,  $D=D'$, $\omega = \omega'$, $q=q'$, $d'(j)=i$ and $d(l) = d'(l)$ for $l\neq j$. Then, $f_i(\mathcal{E}') \ge f_i(\mathcal{E})$.
\end{axiom}

\begin{axiom}[Monotonicity w.r.t. Delegations (\textbf{MD})]
Consider two LDEs $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$ and $\mathcal{E}' = \langle D', \omega', d', q' \rangle$ and three agents $i,j,k \in V$ such that $j \not\in  c_d(k,d_k^*)$, $i \not\in  c_d(j,d_j^*)$, $i \in  c_d(k,d_k^*)$,  $D=D'$, $\omega = \omega'$, $q=q'$, $d'(j)=k$ and $d(l) = d'(l)$ for $l\neq j$. Then, $f_i(\mathcal{E}') \ge f_i(\mathcal{E})$.
\end{axiom}

Before proceeding, we note that there are different ways in which the Shapley value of an agent can be expressed. We recall the following one. Let $\Pi[n]$ (or $\Pi$ when the value $n$ is clear from the context) be all possible permutations of voters in $[n]$. For any $\pi \in \Pi$, let $C_{\pi}(i)$ denote the set of all voters preceding i in $\pi$. Let $m^{\nu_\mathcal{E}}_{\pi}(i)$ be the marginal contribution of voter $i$ with respect to $\pi \in \Pi$ which is defined as follows:
\begin{align}\label{alignMarginalContribution}
    m^{\nu_\mathcal{E}}_{\pi}(i) := \nu_\mathcal{E}(C_{\pi}(i)\cup \{i\})-\nu_\mathcal{E}(C_{\pi}(i)).
\end{align}
When $\nu_\mathcal{E}$ is clear from the context, we write $m_{\pi}(i)$ instead of $m^{\nu_\mathcal{E}}_{\pi}(i)$. It is well known that the Shapley value of voter $i$ can be rewritten as follows:
\begin{align}\label{alignShapelySecond}
    DS_i=\frac{1}{n!}\sum_{\pi \in \Pi} m_{\pi}(i).
\end{align}
Recall that in a delegative simple game $\mathcal{G}_{\mathcal{E}}$, $\nu_\mathcal{E}(C)=1$ iff $\sum_{i\in \hat{D}(C)}\omega(i)\ge q$, where $\hat{D}(C)$ represents the set of all active voters in $C$.

\begin{lemma}\label{lmAxiomsSatisfaction}
The delegative Shapley-Shubik value satisfies \textbf{DP}, \textbf{EI}, \textbf{SA}, \textbf{SP} and \textbf{MDD}.

\begin{proof}
Note that axioms \textbf{DP}, \textbf{EI}, \textbf{SA} have nothing specific to delegative simple games and hence the standard proof to show that the Shapley-Shubik index satisfies them apply. For completeness, we recall these proofs. 
Consider an arbitrary permutation $\pi$. By definition, for any dummy agent $i$, we have $\nu_{\mathcal{E}}(C_{\pi}(i))=\nu_\mathcal{E}(C_{\pi}(i)\cup \{i\})$, and hence $m_{\pi}(i) = 0$. Since this holds for any permutation $\pi$, $DS$ satisfies axiom \textbf{DP}.\\

To show that $DS$ satisfies axiom \textbf{EI}, we proceed as follows. First note that the sum of marginal contributions of voters with respect to $\pi \in \Pi$ is $\nu_\mathcal{E}(V)$. More formally, let $a_i$ be the $i$th player in $\pi$, then
\begin{align*}
    \sum_{i\in V}m_{\pi}(i)&=\nu_\mathcal{E}(\{a_1\})-\nu_\mathcal{E}(\emptyset)+\nu_\mathcal{E}(\{a_1,a_2\})-\nu_\mathcal{E}(\{a_1\})+\ldots\\&+\nu_\mathcal{E}(\{a_1,\ldots,a_n\})-\nu_\mathcal{E}(\{a_1,\ldots,a_{n-1}\})=\nu_\mathcal{E}(\{a_1,\ldots,a_n\})=\nu_\mathcal{E}(V).
\end{align*}
Hence, we have
\begin{align*}
    \sum_{i\in V} DS_i&=\frac{1}{n!}\sum_{i\in V}\sum_{\pi \in \Pi} m_{\pi}(i)= \frac{1}{n!}\sum_{\pi \in \Pi} \sum_{i\in V}m_{\pi}(i)\\&=\frac{1}{n!}\sum_{\pi \in \Pi} \nu_\mathcal{E}(V)=\nu_\mathcal{E}(V).
\end{align*}

To prove axiom \textbf{SA}, we proceed as follows. Consider a permutation $\pi \in \Pi$, let $\pi(k)$ denote the position of the $k^{th}$ voter in $\pi$. We now create a permutation $\pi'$ as follows: $\pi'(i)=\pi(j)$, $\pi'(j)=\pi(i)$ and for any $k\ne i,j$, $\pi'(k)=\pi(k)$. In words, $\pi'$ is obtained from $\pi$ by swapping agents $i$ and $j$. Now, we show that $m_{\pi}(i)=m_{\pi'}(j)$ by distinguishing two cases.

\begin{enumerate}
    \item $i$ precedes $j$ in $\pi$. So, we have $C_{\pi}(i)=C_{\pi'}(j)$. Let $S=C_{\pi}(i)=C_{\pi'}(j)$. We have 
    \begin{align*}
      m_{\pi}(i)= \nu_\mathcal{E}(S\cup \{i\})-\nu_\mathcal{E}(S)\ \text{and}\  m_{\pi'}(j)= \nu_\mathcal{E}(S\cup \{j\})-\nu_\mathcal{E}(S).
    \end{align*}

Since $i$ and $j$ are symmetric agents, i.e., $\nu_\mathcal{E}(S\cup \{i\})=\nu_\mathcal{E}(S\cup \{j\})$, $m_{\pi}(i)=m_{\pi'}(j)$ in this case.

\item $j$ precedes $i$ in $\pi$. Let $S=C_{\pi}(i) \setminus \{j\}$. We have
    \begin{align*}
       m_{\pi}(i)= \nu_\mathcal{E}(S\cup \{i,j\})-\nu_\mathcal{E}(S\cup \{j\})\ \text{and}\  m_{\pi'}(j)= \nu_\mathcal{E}(S\cup \{i,j\})-\nu_\mathcal{E}(S\cup{i}).
    \end{align*}
Again by symmetry, we have $\nu_\mathcal{E}(S\cup \{i\})=\nu_\mathcal{E}(S\cup \{j\})$, which results in $m_{\pi}(i)=m_{\pi'}(j)$ in this case.
\end{enumerate}
As this holds for any permutation, $DS$ satisfies axiom \textbf{SA}.

To show that $DS$ satisfies axiom \textbf{SP}, we recall that for any $C \subseteq V_1 \cup V_2$, $\nu_{\mathcal{E}_1 \land \mathcal{E}_2}(C)=1$ (resp. $\nu_{\mathcal{E}_1 \lor \mathcal{E}_2}(C)=1$) iff $\nu_{\mathcal{E}_1}(C \cap V_1)=1$ and (resp. or) $\nu_{\mathcal{E}_2}(C \cap V_2)=1$. 
Let $P_i^{\mathcal{E}_j}$ (with $j\in \{1,2\}$) be the set of permutations for which agent $i$ is a swing agent in $\mathcal{G}_{\mathcal{E}_j}$, i.e., $P_i^{\mathcal{E}_j}=\{\pi \in \Pi_j: m^{\nu_{\mathcal{E}_j}}_{\pi}(i) = 1\}$, %\nu_{\mathcal{E}_j}(C_{\pi}(i))= 0\text{ and } \nu_{\mathcal{E}_j}(C_{\pi}(i) \cup \{i\})=1\}$, 
where $\Pi_j$ is the set of all permutations of $V_j$. 
Let $n_1=|V_1|$, $n_2=|V_2|$ and $n = |V_1 \cup V_2|$. Consider a permutation $\pi$ of $V_j$ ($j \in \{1,2\}$). Let $\pi'_\pi$ be a permutation of $V_1 \cup V_2$ in which voters in $V_j$ has the same order as in $\pi$. The number of such permutations $\pi'_\pi$ is $\frac{n!}{n_j!}$. 


Given a permutation $\pi$ of $V_1 \cup V_2$, we will denote by $\pi[V_1]$ (resp. $\pi[V_2]$) the restriction of $\pi$ to $V_1$ (resp. $V_2$). We will now count the permutations for which $i$ is a swing in $ \mathcal{G}_{\mathcal{E}_1 \lor \mathcal{E}_2}$. 
Note that a necessary condition for $i$ to be swing in $\pi$ for $\mathcal{G}_{\mathcal{E}_1 \lor \mathcal{E}_2}$ or $\mathcal{G}_{\mathcal{E}_1 \land \mathcal{E}_2}$ is that $i$ should be a swing in $\pi[V_1]$ for $\mathcal{G}_{\mathcal{E}_1}$ or $i$ should be a swing in $\pi[V_2]$ for $\mathcal{G}_{\mathcal{E}_2}$.

Given a permutation $\pi \in V_1$, for which $i$ is a swing agent in $\pi$ for $\mathcal{G}_{\mathcal{E}_1}$, then $\pi$ can be extended in $\frac{n!}{n_1}$ permutations $\pi'_\pi$ such that $\nu_{\mathcal{E}_1}(C_{\pi'_\pi}(i) \cup \{i\} \cap V_1) = 1 $ and $\nu_{\mathcal{E}_1}(C_{\pi'_\pi}(i) \cap V_1) = 0 $. 
For such a permutation $\pi'_\pi$, $i$ will be swing for $\mathcal{G}_{\mathcal{E}_1 \lor \mathcal{E}_2}$ if $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2) = 0 $. 
Moreover $i$ will then be a swing in $\pi'_\pi$ for $\mathcal{G}_{\mathcal{E}_1 \land \mathcal{E}_2}$ if $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2) = 1 $ or if $i$ is also a swing in $\pi'_{\pi}[V_2]$ for $\mathcal{G}_{\mathcal{E}_2}$. Hence, note that if $i$ is not a swing for $\pi'_\pi$ in $\mathcal{G}_{\mathcal{E}_1 \lor \mathcal{E}_2}$, then $i$ is a swing for $\pi'_\pi$ in $\mathcal{G}_{\mathcal{E}_1 \land \mathcal{E}_2}$.

A symmetric analysis can be  applied for permutations $\pi \in V_2$, for which $i$ is a swing agent in $\pi$ for $\mathcal{G}_{\mathcal{E}_2}$. From this analysis, we can derive the following formula:
\begin{equation}
        |P_{i}^{\mathcal{E}_1 \lor \mathcal{E}_2} |= \frac{n!}{n_1!}|P_i^{\mathcal{E}_1}| + \frac{n!}{n_2!} |P_i^{\mathcal{E}_2}| - |P_{i}^{\mathcal{E}_1 \land \mathcal{E}_2}|. \label{alignSPGeneral}
\end{equation}
As a last comment to justify the formula, note that if a permutation $\pi \in \Pi[n]$ is counted twice in the two first summands because $i$ is both a swing in $\pi[V_1]$ for $\mathcal{G}_{\mathcal{E}_1}$ and a swing in $\pi[V_2]$ for $\mathcal{G}_{\mathcal{E}_2}$, then this is corrected by the fact that $i$ is also a swing in $\pi$ for $\mathcal{G}_{\mathcal{E}_1 \land \mathcal{E}_2}$.  

%Suppose that $i$ is a swing agent in $\pi \in \Pi_1$ in $\mathcal{G}_{\mathcal{E}_1}$. Let $\pi'_{\pi}$ be a permutation of $ V_1 \cup V_2$ in which voters in $V_1$ has the same order as in $\pi$. We distinguish two cases. 
%\HG{I still cannot understand this part !}
%\begin{enumerate}
%    \item $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2)=0$. Let $P_{i0}^{\mathcal{E}_1 \land \mathcal{E}_2} \subseteq P_{i}^{\mathcal{E}_1 \land \mathcal{E}_2}$ and $P_{i0}^{\mathcal{E}_1 \lor \mathcal{E}_2} \subseteq P_{i}^{\mathcal{E}_1 \lor \mathcal{E}_2}$ be the set of permutations for which $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2)=0$. Since $i \in V_1\setminus V_2$, clearly $P_i^{\mathcal{E}_2}=\emptyset$ and $P_{i0}^{\mathcal{E}_1 \land \mathcal{E}_2}=\emptyset$ \HG{Why ?} as $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2)=0$ (by assumption). Also, $i$ will be a swing agent in $\mathcal{G}_{\mathcal{E}_1} \lor \mathcal{G}_{\mathcal{E}_2}$ for $\frac{n!}{n_1!}$ different permutations when $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2)=0$. Thus, $|P_{i0}^{\mathcal{E}_1 \lor \mathcal{E}_2}|=|P_i^{\mathcal{E}_1}| \frac{n!}{n_1!}$. %, using permutation properties of objects Grimaldi~\cite[Ch.\ 1]{grimaldi2006discrete} \HG{But $n$ is not equal to $n_1+ n_2$?}.
%    Therefore, 
%    \begin{align}\label{alignSP0}
%      |P_{i0}^{\mathcal{E}_1 \lor \mathcal{E}_2} |= \frac{n!}{n_1!}|P_i^{\mathcal{E}_1}| + \frac{n!}{n_2!} |P_i^{\mathcal{E}_2}| - |P_{i0}^{\mathcal{E}_1 \land \mathcal{E}_2}|.
%    \end{align}
    
%    \item $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2)=1$. Let $P_{i1}^{\mathcal{E}_1 \land \mathcal{E}_2} \subseteq P_{i}^{\mathcal{E}_1 \land \mathcal{E}_2}$ and $P_{i1}^{\mathcal{E}_1 \lor \mathcal{E}_2} \subseteq P_{i}^{\mathcal{E}_1 \lor \mathcal{E}_2}$ be the set of permutations for which $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2)=1$. Since $i \in V_1\setminus V_2$, clearly $P_i^{\mathcal{E}_2}=\emptyset$ and $P_{i1}^{\mathcal{E}_1 \lor \mathcal{E}_2}=\emptyset$ as $\nu_{\mathcal{E}_2}(C_{\pi'_\pi}(i) \cap V_2)=1$ by assumption. Thus, $|P_{i1}^{\mathcal{E}_1 \land \mathcal{E}_2}|=|P_i^{\mathcal{E}_1}| \frac{n!}{n_1!}$. Again, we can use the idea in Equation~\ref{alignSP0} to represent this relation between $P_{i1}^{\mathcal{E}_1 \land \mathcal{E}_2}$ and $P_i^{\mathcal{E}_1}$. It means that
    
%    \begin{align}\label{alignSP1}
%      |P_{i1}^{\mathcal{E}_1 \lor \mathcal{E}_2} |= \frac{n!}{n_1!}|P_i^{\mathcal{E}_1}| + \frac{n!}{n_2!} |P_i^{\mathcal{E}_2}| - |P_{i1}^{\mathcal{E}_1 \land \mathcal{E}_2}|.
%    \end{align}
%\end{enumerate}

%By the same argument, Equations~\ref{alignSP0} and~\ref{alignSP1} can be used for voters $i \in V_2 \setminus V_1$. Now consider $i \in V_1\cap V_2$. It is not hard to see that for any $i \in V_1\cap V_2$, there exists a permutation $\pi'$ of $V_1 \cup V_2$ for which $i$ is swing agent in at least one of the two weighted voting games $\mathcal{G}_{\mathcal{E}_1} \lor \mathcal{G}_{\mathcal{E}_2}$ and $\mathcal{G}_{\mathcal{E}_1} \land \mathcal{G}_{\mathcal{E}_2}$ if at least in one of the two games $\mathcal{G}_{\mathcal{E}_1}$ and $\mathcal{G}_{\mathcal{E}_2}$ there is one permutation $\pi$ for which $i$ is a swing agent in. In particular, suppose that $i \in V_1\cap V_2$ is a swing agent in $\pi_1 \in \Pi_1$ in $\mathcal{G}_{\mathcal{E}_1}$. Then, the total number of permutations that $i$ is swing agent in both $\mathcal{G}_{\mathcal{E}_1} \lor \mathcal{G}_{\mathcal{E}_2}$ and $\mathcal{G}_{\mathcal{E}_1} \land \mathcal{G}_{\mathcal{E}_2}$ is greater than or equal to $\frac{n!}{n_1!}$ regardless of whether $i$ is swing agent in these permutations $\pi_{\pi_1}$ of $V_1 \cup V_2$ in $\mathcal{G}_{\mathcal{E}_2}$. Let $\pi_1 \in \Pi_1$ and $\pi_2 \in \Pi_2$. Also, we can see that there exists a permutation $\pi'$ of $V_1 \cup V_2$ for which $i$ is swing agent in both $\mathcal{G}_{\mathcal{E}_1} \lor \mathcal{G}_{\mathcal{E}_2}$ and $\mathcal{G}_{\mathcal{E}_1} \land \mathcal{G}_{\mathcal{E}_2}$ if there are two permutations $\pi_1$ and $\pi_2$, where $i$ is swing agent in $\pi'_{\pi_1}$ and $\pi'_{\pi_2}$ in $\mathcal{G}_{\mathcal{E}_1}$ and $\mathcal{G}_{\mathcal{E}_2}$, respectively. This implies that for any $i \in V_1 \cap V_2$, we have

%\begin{align}\label{alignSPGeneral}
%    |P_{i}^{\mathcal{E}_1 \lor \mathcal{E}_2} |= \frac{n!}{n_1!}|P_i^{\mathcal{E}_1}| + \frac{n!}{n_2!} |P_i^{\mathcal{E}_2}| - |P_{i}^{\mathcal{E}_1 \land \mathcal{E}_2}|.
%\end{align}

Now if we divide each side of Equation~\ref{alignSPGeneral} by $n!$, then we have 
\begin{equation*}
    \frac{|P_i^{\mathcal{E}_1 \lor \mathcal{E}_2}|}{n!}=\frac{|P_i^{\mathcal{E}_1}|}{n_1!} + \frac{|P_i^{\mathcal{E}_2}|}{n_2!}-\frac{|P_i^{\mathcal{E}_1 \land \mathcal{E}_2}|}{n!}
\end{equation*}
This implies that for any $i \in V_1 \cup V_2$, we have $DS_i(\mathcal{E}_1 \lor \mathcal{E}_2)+DS_i(\mathcal{E}_1 \land \mathcal{E}_2)=DS_i(\mathcal{E}_1)+DS_i(\mathcal{E}_2)$ and the proof is complete.

Last, we turn to axiom \textbf{MDD}. Consider two LDEs $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$ and $\mathcal{E}' = \langle D', \omega', d', q' \rangle$ and two agents $i,j \in V$ such that $j \not\in  c_d(i,d_i^*)$,  $D=D'$, $\omega = \omega'$, $q=q'$, $d'(j)=i$ and $d(l) = d'(l)$ for $l\neq j$. Let us consider a coalition $C\subseteq V\setminus\{i\}$ such that $\nu_{\mathcal{E}}(C \cup\{ i \}) - \nu_{\mathcal{E}}(C) = 1$. This implies that $c_d(i,d_i^*)\subseteq C\cup\{i\}$. 
From $\nu_{\mathcal{E}}(C \cup\{ i \}) = 1$, it is straightforward that $\nu_{\mathcal{E}'}(C \cup\{ i \}) = 1$ as $d(l) = d'(l)$ for $l\neq j$, $d'(j)=i$ and $c_d(i,d_i^*)\subseteq C\cup\{ i \}$. Moreover, from $\nu_{\mathcal{E}}(C) = 0$, it is also easy to see that $\nu_{\mathcal{E}'}(C) = 0$ as $d(l) = d'(l)$ for $l\neq j$, $d'(j)=i$ and $i\not\in C$. 
Because this reasoning holds for any coalition for which $i$ is a swing agent, we obtain that  $DS_i(\mathcal{E}') \ge DS_i(\mathcal{E})$. 
%To show that $DS$ satisfies \textbf{AD}, we proceed as follows. Let $\nu^{+}=\nu+\nu'$ be the characteristic function of a game $V^+=V(v^{+})$. Consider an agent $i \in N$ and a permutation $\pi \in \Pi$, recall that $m^{\nu^+}_{\pi}(i)=\nu^{+}_V(C_{\pi}(i)\cup \{i\})-\nu^{+}_V(C_{\pi}(i))$. For any $C \subseteq N$, since $\nu^{+}(C)=\nu_V(C)+\nu'_V(C)$, $m^{+}_{\pi}(i)=m^{\nu}_{\pi}(i)+m^{\nu'}_{\pi}(i)$. We have 

%\begin{align*}
 %    DS_i(V^+)=\frac{1}{n!}\sum_{\pi \in \Pi} m^{\nu^+}_{\pi}(i)= \frac{1}{n!}\sum_{\pi \in \Pi} (m^{\nu}_{\pi}(i)+ m^{\nu'}_{\pi}(i))=DS_i(V^\nu)+ DS_i(V(\nu')).
%\end{align*}
%This implies that $DS$ satisfies \textbf{AD} and the proof is complete.

\end{proof}
\end{lemma}

In the following we aim to show that $DS$ does not satisfy axiom $\textbf{BP}$ nor $\textbf{MD}$.

\begin{obs}
$DS$ does not satisfy axiom \textbf{BP}.

\begin{proof}

Consider an LDE $\mathcal{E}=\langle D=(V,A), \omega, d,q\rangle$, where $V=\{1,2,3,4\}$ is a set of $4$ agents delegating through a social network with delegation profile $d=\langle2,2,4,4\rangle$ illustrated in Fig.~\ref{figBlocPinciple}, all voting weights being equal to one and $q=3$. To compute $DS_4(\mathcal{E})$, for $s=2$, $N_s=2$ (two sets $\{2,1\}$ and $\{2,3\}$) and for $s=3$, $N_s=1$ (one set $\{1,2,3\}$). Obviously, $N_s=0$, when $s=0,1,4$. Thus, $DS_4(\mathcal{E})=DS_2(\mathcal{E})=\frac{5}{12}$.

Let $\mathcal{E}'=\langle D' = (V',A'),\omega', d',q \rangle$ be the bloc LDE joining $2$ and $4$ into a new agent $24$ with weight $\omega'(24)=2$. So, $V'=\{1,3,24\}$ and $d'=\langle24,24,24\rangle$ illustrated in Fig.~\ref{figBlocPinciple}. We can easily find that $DS_{24}(\mathcal{E}')=\frac{2}{3}$. Therefore, $DS_{24}(\mathcal{E}') < DS_2(\mathcal{E})+DS_4(\mathcal{E})$, which implies that $DS$ does not satisfy axiom \textbf{BP}. 
\end{proof}
\begin{figure}[!h]
		\centering
		
		\begin{minipage}{.4\textwidth}
		\begin{tikzpicture}
				\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white}}
				\tikzset{edge/.style = {->,> = latex'}}
				
				\node[vertex] (4) at  (0,0) {$4$};
				\node[vertex] (3) at  (0,-1.3) {$3$};
				\node[vertex] (2) at  (1.5,0) {$2$};
				\node[vertex] (1) at  (1.5,-1.3) {$1$};
				
				%edges
				\draw[edge] (3) to (4);
				\draw[edge] (1) to (2);
			
		\end{tikzpicture}
		\end{minipage}
		\begin{minipage}{.4\textwidth}
		\begin{tikzpicture}
				\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white}}
				\tikzset{edge/.style = {->,> = latex'}}
				
				\node[vertex] (24) at  (0.75,0) {$24$};
				\node[vertex] (3) at  (0,-1.3) {$3$};
				\node[vertex] (1) at  (1.5,-1.3) {$1$};
				
				%edges
				\draw[edge] (3) to (24);
				\draw[edge] (1) to (24);
			
		\end{tikzpicture}
		\end{minipage}
		\caption{ The LDE $\mathcal{E}= \langle D=(V,A), \omega, d,q\rangle$, where $V=\{1,2,3,4\}$, $q=3$ and $Gu_d=\{2,4\}$ (left) and the bloc LDE $V'$ that joins $2$ and $4$ and makes a new agent $24$ with weight $\omega'(24)=2$ (right).} \label{figBlocPinciple}
\end{figure}
\end{obs}

\begin{obs}\label{obs:md}
$DS$ does not satisfy axiom \textbf{MD}.
\end{obs}
\begin{proof}
Consider an LDE $\mathcal{E}=\langle D=(V,A), \omega, d,q\rangle$, where $V=\{1,2,3\}$ is a set of $3$ agents delegating through a complete social network $D$ ($A$ contain all possible arcs) with delegations $d(2)=d(1)=1$ and $d(3)=3$, all weights equal to one, and $q=3$. In $\mathcal{E}$ voter $1$ is a swing agent for sets in $\{\{2\},\{3\},\{2,3\}\}$. Now consider the LDE $\mathcal{E}'$ which is identical to $\mathcal{E}$ except that $d(3)=2$. In $\mathcal{E}'$ voter $1$ is a swing agent for sets in $\{\{2\},\{2,3\}\}$. Hence, $DS_1(\mathcal{E}') < DS_1(\mathcal{E})$.
\end{proof}

Hence, Obervation~\ref{obs:md} shows that while the delegative Shapley-Shubik index satisfies axiom \textbf{MDD} it does not satisfy axiom \textbf{MD}. A similar observation can be made for the delegative Banzhaf index. This is a paradox for these indices, a voter who receives more voting power can become less powerful because of the delegation structure underlying the delegative simple game. 

\begin{comment}
To characterize $DS$, we need the following lemma.




\begin{lemma}\label{lmDSUniqu}
A power index $f$ for delegative simple games satisfies \textbf{DP}, \textbf{EI}, \textbf{SA} and \textbf{SP}, only if it is $DS$. 



\begin{proof}


The proof includes two steps. In the first step, we show that $f$ is $DS$ for any unanimity delegative simple game. In the second step, we show that if $f$ is $DS$ for any unanimity simple delegative game, it is $DS$ for any delegative simple game.

\paragraph{The First Step.} To prove the first step's claim, we follow the notations and techniques by Dubey~\cite{dubey1975uniqueness}. Consider an LDE $\mathcal{E}= \langle D, \omega, d, q \rangle$ and the delegative simple game $\mathcal{G}_{\mathcal{E}}$. We say that a set $S$ is carrier for $\mathcal{G}_\mathcal{E}$ with a characterization function $\nu_\mathcal{E}$ if $\nu_\mathcal{E}(C)=\nu_\mathcal{E}(C \cap S)$ for all $C \subset V$. As $DS$ satisfies \textbf{DP} and \textbf{EI}, if $S$ is a carrier for $\mathcal{G}_\mathcal{E}$, then $\sum_{i \in S}DS_i(\mathcal{E})=\nu_\mathcal{E}(S)$. 

For each coalition $S \subseteq V$, let $\mathcal{E}^S$ be an LDE that induces the delegative game $\mathcal{G}_{\mathcal{E}^{S}}$, where for any $C \subseteq V$, $\nu_{\mathcal{E}^{S}}(C)=1$ if $S \subseteq C$, and $\nu_{\mathcal{E}^{S}}(C)=0$ otherwise (note that weights of agents and the quota can always be set to create such an LDE). As $S$ and its supersets are all carriers for $\mathcal{G}_{\mathcal{E}^{S}}$, thus, by \textbf{EI}, $\sum_{i \in S}f_i(\mathcal{E}^{S})=1$ %=\sum_{i \in S}DS_i(\mathcal{G}^{S,c}_\mathcal{E})$
and $\sum_{i \in S \cup \{j\}}f_i(\mathcal{E}^{S})=1$ whenever $j \notin S$.
%=\sum_{i \in S \cup \{j\}}DS_i(\mathcal{G}^{S,c}_\mathcal{E})$ 
It is not hard to see that for any two distinct agents $i, j\in S$, by \textbf{SA}, $f_i(\mathcal{E}^{S})=f_j(\mathcal{E}^{S})$. %As a result, $f(\mathcal{G}^{S,c}_\mathcal{E})$ is unique and identical to $DS(\mathcal{G}^{S,c}_\mathcal{E})$%we have $f_i(\mathcal{G}^{S,c}_\mathcal{E})=0=DS_i(\mathcal{G}^{S,c}_\mathcal{E})$ for every $i \notin S$ and $f_i(\mathcal{G}^{S,c}_\mathcal{E})=c/|S|=DS_i(\mathcal{G}^{S,c}_\mathcal{E})$ for every $i \in S$.
This leads to the uniqueness of $f(\mathcal{E}^{S})$, i.e., $f(\mathcal{E}^{S})=DS(\mathcal{E}^{S})$.

Let $\mathcal{UE}^S$ be a unanimity LDE that induces a unanimity delegative simple game $\mathcal{G}_{\mathcal{UE}^{S}}$ defined on $S$, where $\nu_{\mathcal{UE}^{S}}(C)=1$ if $C=S$; $\nu_{\mathcal{UE}^{S}}(C)=0$ otherwise. We know that any delegative simple game can be written as a disjunction of finitely many unanimity games (by considering the minimally winning coalitions). Now we want to show that a power index $f$ satisfying \textbf{DP}, \textbf{EI}, \textbf{SA} and \textbf{SP} is unique on unanimity delegative simple games. 
%Hence $f$ is $DS$, using $\textbf{SP}$, if we can show that each $f(\mathcal{UG}^{S,c}_\mathcal{E})$ is $DS(\mathcal{UG}^{S,c}_\mathcal{E})$ \HG{WHY?}.
By induction, suppose that $f(\mathcal{UE}^{S})=DS(\mathcal{UE}^{S})$, where $|S|=k+1,\ldots,n$. Obviously, this holds when $|S|=n$, since $f(\mathcal{UE}^{S})=f(\mathcal{E}^{S})$ and $f(\mathcal{E}^{S})$ is unique. 

Let $S_1, S_2, \dots, S_l$ be all of the proper super sets of $S$. Note that $|S_i| > k$ for any $i \in [l]$, so by inductive assumption $f(\mathcal{UE}^{S_i})$ is $DS(\mathcal{UE}^{S_i})$. $\mathcal{E}^{S}$ can be written as the disjunction of a finite number of unanimity LDEs. %According to $\nu_{\mathcal{E}^{S,c}}$'s definition in $\mathcal{G}_{\mathcal{E}^{S,c}}$
So, for $|S|=k$, we have 

$$\mathcal{E}^{S}=\mathcal{UE}^{S} \lor \mathcal{UE}^{S_1} \lor \dots \lor \mathcal{UE}^{S_l}.$$

By \textbf{SP},
\begin{equation}\label{alignClaim2SP}
    \begin{split}
        f(\mathcal{E}^{S}) =& f(\mathcal{UE}^{S} \lor \mathcal{UE}^{S_1} \lor \dots \lor \mathcal{UE}^{S_l})=f(\mathcal{UE}^{S_1} \lor \dots \lor \mathcal{UE}^{S_l})\\+& f(\mathcal{UE}^{S})-f((\mathcal{UE}^{S_1} \lor \dots \lor \mathcal{UE}^{S_l}) \land \mathcal{UE}^{S}).
    \end{split}
\end{equation}


We can rewrite the last summand in Equation~\ref{alignClaim2SP} as $f((\mathcal{UE}^{S_1} \lor \dots \lor \mathcal{UE}^{S_l}) \land \mathcal{UE}^{S}) = f((\mathcal{UG}^{S_1}_\mathcal{E}\lor \ldots \lor \mathcal{UG}^{S_l}_\mathcal{E}))$ because in $\mathcal{G}_{(\mathcal{UE}^{S_1} \lor \dots \lor \mathcal{UE}^{S_l}) \land \mathcal{UE}^{S}}$, $C$ is a winning coalition if $C$ is a winning coalition in at least one of the unanimity games $\mathcal{G}_{\mathcal{UE}^{S_i}}$ for $i \in [l]$. By induction, all expressions except $f(\mathcal{UE}^{S})$ are unique in Equation~\ref{alignClaim2SP}, which results in the uniqueness of $f(\mathcal{UE}^{S})$, i.e., $f(\mathcal{UE}^{S})=DS(\mathcal{UE}^{S})$. 
%$f(\mathcal{UG}^{S,c}_\mathcal{E} \land \mathcal{UG}^{S_i,c}_\mathcal{E})=0$ for any $i\in [l]$ \HG{I am sorry I don't see why}.
\HG{Maybe you mean that $f((\mathcal{UG}^{S_1}_\mathcal{E}\lor \ldots \lor \mathcal{UG}^{S_l}_\mathcal{E}) \land \mathcal{UG}^{S}_\mathcal{E}) = f((\mathcal{UG}^{S_1}_\mathcal{E}\lor \ldots \lor \mathcal{UG}^{S_l}_\mathcal{E}))$.} 

%\begin{align}\label{alignClaim2Sum}
 %   f(\mathcal{G}^{S,c}_\mathcal{E})=f(\mathcal{UG}^{S,c}_\mathcal{E})+f(\mathcal{UG}^{S_1,c}_\mathcal{E}) + \ldots + f(\mathcal{UG}^{S_l,c}_\mathcal{E}).
%\end{align}

%By induction, all expressions except $f(\mathcal{UG}^{S,c}_\mathcal{E})$ are unique, which implies that $f(\mathcal{UG}^{S,c}_\mathcal{E})$ is unique too and equal to $DS(\mathcal{UG}^{S,c}_\mathcal{E})$. 


\paragraph{The Second Step.} \HG{I don't understand this part.} To prove the second step's claim we follow Einy and Haimanko~\cite{einy2011characterization}. Recall that in this step, we aim to show that $f$ is unique for any delegative simple game as it is unique for any unanimity game (by previous step). %For $s=|S|=k+1, \dots, n$, suppose that 

%\begin{align*}
%f_i(\mathcal{UG}^{S,c}_\mathcal{E})\!=\! \left\{ \begin{array}{c c}
%\frac{(s-1)!(n-s)!}{n!}.c & \text{ if } i \in S \\
%- \frac{s!(n-s-1)!}{n!}.c & \text{ otherwise.}
%\end{array} \right.
%\end{align*}

%Clearly, this is true for $|S|=n$, since $f(\mathcal{UG}^{S,c}_\mathcal{E})=f(\mathcal{G}^{S,c}_\mathcal{E})$. Using Equation~\ref{alignClaim2SP} (i.e., by uniqueness of $f(\mathcal{UG}^{S,c}_\mathcal{E}$), for $|S|=k$, we have 

%\begin{align*}
%f_i(\mathcal{UG}^{S,c}_\mathcal{E})\!=\! \left\{ \begin{array}{c c}
%\frac{(s-1)!(n-s)!}{n!}.c & \text{ if } i \in S \\
%- \frac{s!(n-s-1)!}{n!}.c & \text{ otherwise.}
%\end{array} \right.
%\end{align*}

%Now we can obtain $f(\mathcal{G}_\mathcal{E})$, for any $\mathcal{G}_\mathcal{E}$. 
Let $S_1, S_2, ..., S_k$ be all the minimal winning coalitions in $\mathcal{G}_{\mathcal{E}}$. So, we have 
\HG{What do you mean by a sum of games ?}
\begin{align*}%\label{alignUnionOfUnanimityGames}
    \mathcal{E}=\bigvee_{i}^{k} \mathcal{UE}^{S_i}.
\end{align*}

%For simplicity, we write $\mathcal{UE}^{S_i}$ instead of $\mathcal{UE}^{S_i,\nu_\mathcal{E}(S_i)}$ in what follows.
As $f$ satisfies the \textbf{SP}, using Lemma 2.3 of Einy~\cite{einy1987semivalues},  we can have \HG{But that is not what SP says.}

\begin{align}\label{equationEiny}
    f(\mathcal{E})= f(\bigvee_{i}^{k} \mathcal{UE}^{S_i})= \sum_{I \subset \{1,2,..,k\}} (-1)^{|I|+1} f(\mathcal{UE}^{\bigcup_{m \in I} S_m})
\end{align}
, where $\mathcal{UE}^{\bigcup_{m \in I}S_m}= \bigwedge_{i=1}^{m}\mathcal{UE}^{S_i}$. Note that by induction on the number of unanimity games that a simple game contains, Einy~\cite{einy1987semivalues} showed that if a solution $f$ satisfies the \textbf{SP} in simple games, Equation~\ref{equationEiny} holds in a more general case (when $\mathcal{E}= \bigvee_{i}^{k} \mathcal{E}^{S_i}$, where $\mathcal{E}$ is the disjunction of $k$ LDEs).
Equation~\ref{equationEiny} implies that $f$ is unique as each unanimity game is unique. %, so is the sum of these unanimity games. %$f(\mathcal{G}_\mathcal{E})= f(\bigvee_{\emptyset \ne S \subset N} \mathcal{UG}^{S,\nu_\mathcal{E}(S)}_\mathcal{E}).$
%From Equation~\ref{equationEiny}, we can see that the power of any voter $i$ can be determined by the following $n$ values: $f(\mathcal{UG}^{S_i,\nu_\mathcal{E}(S_i)})$
Now for any $s=0,1, ..., n-1$ and $i \in N$, let

\begin{align}\label{alignFDimensions}
    f^s_i(\mathcal{E})=\sum_{\substack{C \subset N \setminus\{i\}, |C|=s}} [\nu(C)-\nu(C\setminus \{i\})].
\end{align}

Note that for any $s \in [n-1]$, $f^s$ satisfies \textbf{SP}, \textbf{DP}, \textbf{SA} and \textbf{EI}. It is not hard to see that $f^0, f^1, ..., f^{n-1}$ are linearly independent. Thus, for any $s \in [n-1]$, we have a coefficient $p^s$ such that $f=\sum_{s=0}^{n-1} p^sf^s$. Using Equation~\ref{alignFDimensions}, we have

\begin{align}\label{alignLinearIndependent}
    f_i(\mathcal{E})=\sum_{\substack{C \subset N \setminus\{i\}, |C|=s}} p^s [\nu(C)-\nu(C\setminus \{i\})].
\end{align}

Let $\mathcal{E}^s$ be the LDE inducing a delegative simple game $\mathcal{G}_{\mathcal{E}^s}$, where for any $C \subseteq V$, $\nu_{\mathcal{E}^s}(C)=1$ if $|C| > s$ and $\nu_{\mathcal{E}^s}(C)=0$ otherwise. By \textbf{DP}, \textbf{SA} and \textbf{EI}, we can easily show that $f(\mathcal{E}^s)=DS(\mathcal{E}^s)$. Using Equation~\ref{alignLinearIndependent} for $\mathcal{G}_{\mathcal{E}^s}$, for any $i \in V$ and $s \in [n-1]$, we have 

$$f_i(\mathcal{E}^s)={n-1 \choose s} p^s.$$

As $f(\mathcal{E}^s)$ is unique, by \textbf{SA}, we have

\begin{align}\label{alignCoefficient}
    p^s=\frac{1}{n} {n-1 \choose s}^{-1}=\frac{s!(n-s-1)!}{n!}.
\end{align}

By uniqueness of $f$ (Equation~\ref{equationEiny}), we can substitute Equation~\ref{alignCoefficient} in Equation~\ref{alignLinearIndependent} and have

$$f_i(\mathcal{E})=\sum_{\substack{C \subset N \setminus\{i\}, |C|=s}} \frac{s!(n-s-1)!}{n!} [\nu(C)-\nu(C\setminus \{i\})].$$

, which is the delegative Shapley value of voter $i$. 
\end{proof}

%\begin{proof}[The second proof]

%To prove the lemma, we shall borrow ideas and notations from Neyman~\cite{neyman1989uniqueness}. %For any two characterization functions $\nu$, $\nu'$ and any $C\subseteq N$, let $(\nu \pm \nu')(C)=\nu(C)\pm \nu'(C)$. Let $V^\nu=\langleN,d,q_{\nu}>$ be a delegative simple game, where $\nu_V(C) = 1$ iff $\sum_{i\in \hat{D}(C)} w(i) \ge q_{\nu}$. 
%For a coalition $S \subseteq V$, consider a delegative simple game $\mathcal{G}^{S}_{\mathcal{E}}$ induced by an LDE $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$, where its characterization $\nu^S_\mathcal{E}$ is a real valued function $\nu^S_\mathcal{E}:2^{V} \rightarrow \mathbb{R}$ given by $\nu^S_\mathcal{E}(C)=\nu^S_\mathcal{E}(S \cap C)$ for any $C \subseteq V$. 
%Note that in our setting $\nu^S_\mathcal{E}(S \cap C)=1$ if the number of active agents in $S \cap C$ exceeds the quota. 
%So, $\mathcal{G}^{S}_{\mathcal{E}}$ is only the restriction of $\mathcal{G}_{\mathcal{E}}$ to subsets of $S$. For any delegative game $\mathcal{G}_{\mathcal{E}}$, let $I(\nu_\mathcal{E})=\{S \subset N| \exists C \subset S \text{ with } \nu_\mathcal{E}(C) \ne 0\}$. Hence, for any minimal coalition $S$ in $I(\nu_\mathcal{E})$, $\nu_\mathcal{E}(S) \ne 0$. Now we prove that $f$ is $DS$ by induction on $|I(\nu_\mathcal{E})|$. 
%If $|I(\nu_\mathcal{E})|=0$ then by \textbf{DP} for any $i \in N$, $f_i=0=DS_i$. 
%Then we assume that $f(\mathcal{G}_\mathcal{E})=DS(\mathcal{G}_\mathcal{E})$ when $|I(v)| \le k$. 
%Now we want to prove that $f(\mathcal{G}_\mathcal{E})=DS(\mathcal{G}_\mathcal{E})$ when $|I(\nu_\mathcal{E})| \le k+1$. Let $S$ be a minimal winning set in $I(\nu_\mathcal{E})$. 
%Then $\mathcal{G}^{S}$ is a unanimity delegative game and, thus by assumption, \textbf{EI}, \textbf{SA} and \textbf{DP}, we have $f_i(\mathcal{G}^{S}_\mathcal{E})=0=DS_i(\mathcal{G}^{S}_\mathcal{E})$ for every $i \notin S$ and $f_i(\mathcal{G}^{S}_\mathcal{E})=\nu^S_\mathcal{E}(S)/|S|=DS_i(\mathcal{G}^{S}_\mathcal{E})$ for every $i \in S$. Let $\mathcal{G}^{-}_\mathcal{E}$ be the delegative simple game where its characterization function $\nu^-_{\mathcal{E}}=\nu_\mathcal{E}-\nu^S_\mathcal{E}$. Recall that $I(\nu^-_\mathcal{E})=I(\nu_\mathcal{E}-\nu^S_\mathcal{E})=\{C' \subset N| \exists C \subset C' \text{ with } \nu_\mathcal{E}(C)- \nu_\mathcal{E}^S(C') \ne 0\}$. Clearly, $|I(\nu^-_\mathcal{E})|< I(\nu_\mathcal{E})$. Furthermore, consider an agent $i \in N$ and a permutation $\pi \in \Pi$, recall that $m^{\nu^-_\mathcal{E}}_{\pi}(i)=\nu^{-}_\mathcal{E}(C_{\pi}(i)\cup \{i\})-\nu^{-}_\mathcal{E}(C_{\pi}(i))$. For any $C \subseteq N$, since $\nu^{-}_\mathcal{E}(C)=\nu_\mathcal{E}(C)-\nu_\mathcal{E}^S(C)$, $m^{\nu^-_\mathcal{E}}_{\pi}(i)=m^{\nu_\mathcal{E}}_{\pi}(i)-m^{\nu_\mathcal{E}^S}_{\pi}(i)$. Thus, we have 

%\begin{align}\label{alignAdditivityDS}
 %    DS_i(\mathcal{G}^-_\mathcal{E})=\frac{1}{n!}\sum_{\pi \in \Pi} m^{\nu^-_\mathcal{E}}_{\pi}(i)= \frac{1}{n!}\sum_{\pi \in \Pi} (m^{\nu_\mathcal{E}}_{\pi}(i)- m^{\nu_\mathcal{E}^S}_{\pi}(i))=DS_i(\mathcal{G}_\mathcal{E})- DS_i(\mathcal{G}^S_\mathcal{E}).
%\end{align}

%By \textbf{SP}, $f(\mathcal{G}^-_\mathcal{E} \lor \mathcal{G}^S_\mathcal{E})=f(\mathcal{G}^-_\mathcal{E})+f(\mathcal{G}^S_\mathcal{E})-f(\mathcal{G}^-_\mathcal{E} \land \mathcal{G}^S_\mathcal{E})$. Clearly, $f(\mathcal{G}^-_\mathcal{E} \land \mathcal{G}^S_\mathcal{E})=0$ because $I(\nu^-_\mathcal{E}) \cap I(\nu^S_\mathcal{E})=\emptyset$. Hence, by induction hypothesis and Equation~\ref{alignAdditivityDS}, $f(\mathcal{G}_\mathcal{E})=f(\mathcal{G}^-_\mathcal{E} \lor \mathcal{G}^S_\mathcal{E})=f(\mathcal{G}^-_\mathcal{E})+f(\mathcal{G}^S_\mathcal{E})=DS(\mathcal{G}^S_\mathcal{E})+DS(\mathcal{G}^-_\mathcal{E})=DS(\mathcal{G}_\mathcal{E})$, which proves the lemma.
%So, by induction hypothesis $f(V(\nu-\nu^S))=DS(V(\nu-\nu^S))$ and by \textbf{SP}, $f(V^\nu)=f(V(\nu-\nu^S) \lor V(\nu^S))=f(V(\nu^S))+f(V(\nu-\nu^S))=DS(V(\nu^S))+DS(V\nu-\nu^S))=DS(V^\nu)$, which proves Claim 2 and the lemma.
%\end{proof}
\end{lemma}

\begin{theorem}
A power measure $f$ is equal to $DS$ iff it satisfies \textbf{DP}, \textbf{EI}, \textbf{SA} and \textbf{SP}.

\begin{proof}
The theorem follows from Lemmas~\ref{lmAxiomsSatisfaction} and~\ref{lmDSUniqu}.
\end{proof}
\end{theorem}

\end{comment}

==> old/Contribution/Distribution/powerdistribution.tex <==

\section{Power Distribution}

The structure of a delegation graph has a considerable impact on the power distribution among agents. In this section, we aim to find a delegation graph with a fixed number of gurus to maximize the minimum power an agent can have. 
Such delegation graph could for instance be useful to determine a committee within the set of voters in such a way that all voters feel important. 
Ensuring that all voters have a ``high'' relative importance incentives participation and prevents some voters to accumulate too much power.

More formally, given a digraph $D$, and a delegation graph $H \in \Delta(D)$, we denote by $f^{H}_i$ the power index of voter $i$ in $H$. The value of $f^{H}_i$ may be computed using the delegative Banzhaf index or the delegative Shapley-Shubik-index. Hence, the weakest agents in $H$ have a power index worth:

$$ \text{(weakest)}\ \ \mu(H):=\min_{i\in V} f^{H}_i.$$
%More formally, suppose we are give a digraph $D$ and a non-negative integer $k$. Consider a delegation graph $H \in \Delta(D)$ with $k$ gurus. Let $f^{H}_i$ be the power index of voter $i$ in $H$, the weakest agent in $H$ are:

The goal here is to organize the delegations in $H$ to maximize $\mu(H)$. We term this problem the MaxiMin Weight Problem (\textbf{MMWP} for short). Formally,

\begin{center}

\noindent\fbox{\parbox{12.7cm}{
		\textbf{MMWP}\\
		\emph{Input}: A graph $D$, a weight function $\omega$, a quota $q$ and an integer $k$.\\
		\emph{Feasible Solution}: A delegation graph $H = (V, E)\in \Delta(D)$ with $k$ gurus. \\
		\emph{Measure for \textbf{MWP}}: $\mu(H)$ to maximize, where $\mu(H)$ can be computed using either the delegative Banzhaf value or the delegative Shapley-Shubik value. 
}}\\
\end{center}

Consider the following observation from Zang and Grossi~\cite{zhang2020power},

\begin{fact}[Fact 2 in~\cite{zhang2020power}]\label{factMonotonocity}
For any pair of agents $i, j \in V(D)$, such that $d_i=j$, $DB_i \le DB_j$.
\end{fact}

Let us assume that $f^{H}_i$ is computed using the delegative Banzhaf value. 
Hence, using Fact~\ref{factMonotonocity}, it is worth noting that to give an optimal solution to \textbf{MMWP}, we only need to find a delegation graph $H_d$ in which $\min_{l \in Leaves(H_d)}f_l^{H_d}$ is maximized where $Leaves(H_d)$ is the set of all leaves in $H_d$. In the following, we will show that \textbf{MMWP} is NP-hard. 

\begin{theorem}\label{thMWP}
Problem \textbf{MMWP} is NP-hard.
\end{theorem}

To prove Theorem~\ref{thMWP}, we will give a reduction from the NP-complete $3$D-Matching problem~\cite{kleinberg2006algorithmdesign}. 
This problem is defined as follows. Let $X$, $Y$, and $Z$ be finite, disjoint sets, and $T \subseteq X \times Y \times Z$ be a set of ordered triples. That is, $T$ consists of triples $(x, y, z)$ such that $x \in X$, $y \in Y$, and $z \in Z$. Now $M \subseteq T$ is a $3$D-Matching if the following holds: for any two distinct triples $(x_1, y_1, z_1) \in M$ and $(x_2, y_2, z_2) \in M$, we have $x_1 \ne x_2$, $y_1 \ne y_2$, and $z_1 \ne z_2$.  In an instance $I=(T,k)$ of $3$D-Matching, the goal is to find a $3$D-Matching $M \subseteq T$ of size $|M|=k$. The resulting decision problem is NP-complete even when $|X|=|Y|=|Z|=k$.

From an instance $I=(T,k)$ of $3$D-Matching, we create an instance $I'=(D,\omega, q, k')$ of \textbf{MMWP} as follows. 
For any $x \in X$, $y \in Y$ and $z \in Z$, we create voters $v_x$, $v_y$ and $v_z$, respectively. 
We let $V_X := \{v_x : x \in X\}$, $V_Y := \{v_y : y \in Y\}$ and $V_Z = := \{v_z : z \in Z\}$ respectively. 
For any triple $(x,y,z) \in T$, we create two directed edges: one from $v_x \in V_X$ to $v_y \in V_Y$, and the other one from $v_y \in V_Y$ to $v_z \in V_Z$. We set the budget $k'$ to $k$ and the quota $q$ to $3$. All voters have voting weight 1. The power index which is used is the delegative Banzhaf index. 

We need the following observation to prove Theorem~\ref{thMWP}.

\begin{obs}\label{obsMWP}
Given an instance $I'=(D, \omega, q,k')$ resulting from our reduction, $\mu(H_d) \ge 2^{-k-1}$ iff for any subtree $T$ of $H_d$ rooted in a vertex in $V_Z$, $|T|=3$.
\begin{proof}
Since $k'=|Z|$, in a solution of \textbf{MMWP}, all voters $v_z \in V_Z$ should vote and all other voters $v_y \in V_Y$ and $v_x \in V_X$ should delegate to voters in $V_Z$ (directly or indirectly). Let $NS(v_x)$ be the set of coalitions $C$ that $v_x$ is a swing agent in. 
As $q=3$, any voter $v_x$ is a swing agent for a coalition $C$ iff:
\begin{itemize}
    \item $(c_d(v_x,d^*_{v_x})\setminus\{x\}) \subseteq C$, where $d^*_{v_x} \in V_Z$. ;
    \item the other voters of $C$ in $V_X \setminus c_d(v_x,d^*_{v_x})$ and $V_Y \setminus c_d(v_x,d^*_{v_x})$ are inactive agents in $C$;
    \item the coalition $C$ does not include another voter from $V_Z$ than $d^*_{v_x}$.
\end{itemize} 
Hence for any $v_x$, $|NS(v_x)| \le 2^{2k-2}$ as $NS(v_x) \subseteq \{(c_d(v_x,d^*_{v_x})\setminus\{x\}) \cup S : S \subseteq (V_Y\setminus\{d_{v_x}\})\cup (V_X\setminus\{v_x\})\}$. 
Moreover, for any $v_x$, $|NS(v_x)|=2^{2k-2}$ if $NS(v_x) = \{(c_d(v_x,d^*_{v_x})\setminus\{x\}) \cup S : S \in (V_Y\setminus\{d_{v_x}\})\cup (V_X\setminus\{v_x\})\}$. 
Stated otherwise, all voters in $V_X \setminus \{v_x\}$ and $V_Y \setminus \{d_{v_x}\}$ are always inactive agents in a coalition containing $c_d(v_x,d^*_{v_x})$ and no other voters in $V_Z$ than $d^*_{v_x}$.  
It is easy to realize that this condition is met in a delegation graph $H_d$ iff all subtrees rooted in a vertex of $V_Z$ in $H_d$ have size equal to $3$. This proves the obervation as the delegative Banzhaf index of a voter $v_x\in V_X$ is then equal to $|NS(v_x)|/2^{n-1} = 2^{-k-1}$  which proves the observation.
%Now imagine a delegation graph $H_d$ in which for any vertex $v_x$, all voters $(V_X\cup V_Y) \setminus c_d(v_x,d^*_{v_x})$ can join a coalition $S$ as inactive agent such that $c_d(v_x,d^*_{v_x}) \subseteq S$. The necessary condition for such a delegation graph $H_d$ is that 
\end{proof}
\end{obs}

We are now ready to prove Theorem~\ref{thMWP}.

\begin{proof}[Proof of Theorem~\ref{thMWP}]
Let $I=(T,k)$ be an instance of $3$D-Matching, and $I'=(D,\omega, q, k')$ be the instance of \textbf{MMWP} resulting from our reduction. 
We want to show that $I$ is a yes instance iff we can find a solution $H_d$ in $I'$ such that $\mu(H_d) \ge 2^{-k-1}$. 
For the first direction, suppose that we have a 3D-Matching $M \subseteq T$ of size $k=|X|=|Y|=|Z|$. 
Consider the delegation graph, where for any $(x,y,z) \in M$, $x$ delegates to $y$ and $y$ delegates to $z$, respectively. 
Hence, in the resulting delegation graph $H_d$, all subtrees rooted in a vertex of $V_Z$ are of size equal to $3$. Using Observation~\ref{obsMWP}, we obtain the desired conclusion. 
Let $H_d$ be a solution in $I'$ such that $\mu(H_d) \ge 2^{-k-1}$. Using Observation~\ref{obsMWP}, we obtain that all subtrees rooted in a vertex of $V_Z$ are of size equal to $3$. Notably, each of these subtrees necessarily contain one element of $V_X$, one element of $V_Y$ and one element of $V_Z$. There are $k$ of them and they do not share any vertex. Hence, they correspond to a 3D-Matching of size $k$. 
\end{proof}


%In the next step, we will show that \textbf{MSP} is NP-hard even when $k=1$. Note that for any $g \in Gu_d$, $f_g \ge f_v$, where $v \in T_d(g)$. Thus to give an optimal solution to \textbf{MSP}, it is enough to minimize $\max_{g\in Gu_d} f^{H_d}_g$. We will give a reduction from the Hamiltonian path problem to \textbf{MSP}.

%\begin{theorem}\label{thMSP}
%\textbf{MSP} is NP-hard even when $k=1$.

%\begin{proof}
%We prove the hardness via a reduction from the Hamiltonian path problem.Consider an instance $I=(V,E)$ of the Hamiltonian path problem, where $V$ is the set of voters and $E$ is the set of edges. To relate the Hamiltonian path problem and \textbf{MSP}, we need to create a graph $G'$ obtained from $I$ by adding a new voter $u$ and connecting all voters $V$ of $I$ to $u$. This means that $G'=(V',E')$, where $V'=V \cup \{u\}$ and $E'=E \cup \{(v,u)| v\in V\}$. Since $k=1$, obviously the only choice we have is to select $u$ as the guru for all voters. Let $H_d \in \Delta(G')$ be a delegation graph such that $u$ is the only guru and it only contains a path, starting from an arbitrary voter $v \in V'\setminus \{u\}$, passing all voters once and ending in $u$. We denote by $\mathcal{J}(G') \subset \Delta(G')$ the set of all such delegation graphs. As $k=1$, we see that for any $H'_d \in \mathcal{J}(G')$, $u$ has the minimum possible power index. It is easy to see that $I$ is a ``yes''-instance of the Hamiltonian path problem if and only $|\mathcal{J}(G')| \ge 1$. This implies that \textbf{MSP} is NP-hard.
%\end{proof}
%\end{theorem}

==> old/Contribution/DynamicProgramming/banzafindex.tex <==

\section{Banzhaf Index}


In what follows, we provide a dynamic programming approach to compute the Banzaf index in polynomial time when voters all start with weight one. 


\begin{theorem}\label{thShBaPolynomial}
Given a delegative simple game of $V=<N, d, q>$ and a voter $i \in N$, $DB_i$ can be computed in $O(n^3)$, respectively. 
\end{theorem}

\begin{proof}

We decompose the proof in two sub-cases : 

\paragraph{Case 1: voter $n$ is a guru.} 
Consider a guru $n$ with weight $w_d(n)$. For every $k \in \{0, ..., w_d(n)-1\}$, let $T_d(n,k)$ be the set of all subtrees $T$ rooted in $n$ such that $|T|=k+1$, i.e., each subtree $T \in T_d(n,k)$ represents a possible way that $n$ obtains a weight $k+1$ by getting $k$ delegations. It is worth noticing that there may be more than one subtree $T \in T_d(n,k)$ in which voter $n$ receives weight $k+1$. For instance, in Example~\ref{exNotations}, $T_d(8)$ has two subtrees with weight $3$ and rooted in $8$ : the first (resp. second) subtree is composed of vertices in $\{6,7,8\}$ (resp. $\{4,7,8\}$). Given a sub-tree $T$, let $ch(T)$ be the set of children of nodes in $T$. To compute $DB_n$, we need to compute, for every $T \in T_d(n,k)$, $N^k(T)$ the number of subsets of $N\setminus (T \cup ch(T))$ that have weight in $\{q-k-1, ..., q-1\}$, where $k=0, ..., w_n-1$. More formally,  for every $T \in T_d(n,k)$, we have 

$$N^k(T)=\sum_{\substack{C\subseteq N\setminus (T \cup ch(T))}} \mathbbm{1}_{q-k-1 \le w_{d}(C) \le q-1},$$

where $\mathbbm{1}_{\phi}$ is equal to $1$ if $\phi$ is true, and $0$ otherwise. %Note that for every $j\in C$, if $j$ is an active agent in $C$, $w(j)=1$, otherwise $w(j)=0$. Furthermore, each voter $j\in T_d(n)\setminus T$ could only join $C$ as inactive voter except when $k\ge q$. It means that when $k\ge q$, voters in $T_d(n)\setminus T$ could join $C$ as active or inactive agents. We highlight this point later. 
Let $N^k =\sum_{T \in T_d(n,k)} N^k(T)$. %\sum^{w_n}_{k=1}\sum_{T \in T_d(n,k)} N^k_s(T)$. 
Now we can compute the $DB_n$ as follows. 

\begin{align}\label{alignShapely}
    DB_n = \frac{1}{2^{n-1}}\sum_{k=0}^{w_d(n)-1}N^k.
\end{align}

Let $t_j=|T_d(j)|$, i.e., the size of the tree $T_d(j)$ rooted in $j$. 
Moreover, let $Anc(j)$ be the set of ancestors of $j$ in the delegation graph.
To compute $DB_n$ efficiently, we use a dynamic programming approach. 
Given a forest $\mathcal{F}$ with $n$ vertices, we define a table $X_{\mathcal{F}}$ where $X_{\mathcal{F}}[j, w]$ is the number of sets $C\subset \{1,...,j\}$ such that $w_d(Anc(j)\cup C) = w_d(Anc(j)) + w$, where $j$ range from $0$ to $n$ and $w$ ranges from $0$ to $n$. In words, we count the number of subsets in $\{1,...,j\}$ who will contribute a weight $w$ when added to a coalition containing all ancestors of $j$. This table entries will be filled as follows.

First, for $j=0$, we have
\begin{align*}
X_{\mathcal{F}}[0, w] \!=\! \left\{ \begin{array}{c c}
1 & \text{ if } w= 0\\
0 & \text{ otherwise.}
\end{array} \right.
\end{align*}
%More generally, $X_{\mathcal{F}}[j, w] = 0$ if $s > j$ or $w > s$. Second, if $s = 0$, then $F_{\mathcal{F}}[j, w, s] = 0$ if $w > 0$ and $1$ otherwise.
In the special case $w=0$, we have
\begin{align}\label{alignWZeroVoters}
         X_{\mathcal{F}}[j, 0]&=\sum_{x = 0}^{ t_j-1} {t_j-1 \choose x}X_{\mathcal{F}}[j - t_j, 0]
\end{align}

Now for $j=1,\ldots, n$, and $w=1, \ldots, q-1$, $F[j, w]$ will be computed as follows.

\begin{equation}\label{eqRecursiveFB}
      \begin{split}
         X_{\mathcal{F}}[j, w]&=\sum_{x = 0}^{ t_j-1} {t_j - 1 \choose x}X_{\mathcal{F}}[j - t_j, w]\\&+ X_{\mathcal{F}}[j-1,w-1]
      \end{split}
\end{equation}
We recall that $X_{\mathcal{F}}[j, w]$ is the number of sets $C\subset \{1,...,j\}$ such that $w_d(Anc(j)\cup C) = w_d(Anc(j)) + w$. Here, the two summands correspond to the cases $j\notin C$ and $j\in C$ respectively.  Note that in the first case, successors of $j$ can only join $C$ as inactive agents. Hence in the first summand, we consider all possible ways of adding to $C$ inactive agents from the tree rooted in $j$ before moving to the next subtree (rooted in $j - t_j$).

We use this dynamic programming equations considering two forests $\mathcal{F}_1 = \{T_d(n)\}$ and $\mathcal{F}_2 = H_d - T_d(n)$ of sizes $n$ and $n-t_n$, respectively. We conclude by noticing that:
\begin{equation}
N^k = \sum_{w = q-k-1}^{q-1} X_{\mathcal{F}_2}[n-t_n,w] (X_{\mathcal{F}_1}[t_n,k]).\label{eq:Nk computation}
\end{equation}

\paragraph{Case 2: voter $n$ is a delegator.}
If $n$ is a delegator, then $n$ can only be a swing agent for coalition $C$ if $Anc(n) \subseteq C$. 
Hence, we should count only coalitions which meet this condition. 
To take this fact into account we use our dynamic programming approach on the delegation graph $H_d[V\setminus Anc(n)]$. 
Moreover, in this case $N^k$ is obtained by a different formula. Let $\alpha = |Anc(n)|$, then  we use the formula:   
\begin{equation} \label{eq:Nk computation2}
N^k = \sum_{w =q_\alpha-k-1 }^{q_\alpha-1} X_{\mathcal{F}_2}[n-t_n,w] (X_{\mathcal{F}_1}[t_n,k]),
\end{equation}
where $q_\alpha = q - \alpha$.

We move to the complexity analysis. Equation \ref{eqRecursiveFB} can be computed in $O(n)$ operations. This leads to a complexity of $O(n^3)$ for computing tables $F_{\mathcal{F}_1}$ and $F_{\mathcal{F}_2}$. As Equations \ref{eq:Nk computation} and \ref{eq:Nk computation2} can be computed in $O(n)$, computing all values $N^k$ can be performed with $O(n^2)$ operations. Therefore, computing the Banzaf value requires $O(n^3)$ operations.
\end{proof}


==> old/Contribution/DynamicProgramming/indexvalue.tex <==

\section{Pseudo-Polynomial Algorithm for $DB$ and $DS$}

In weighted voting games, evaluating the Banzhaf and Shapley-Shubik indices is computationally challenging. 
Indeed, computing each of them in weighted voting games is \#P-complete~\cite{deng1994complexity,prasad1990np} and several decision problems related to their computation are NP-complete or coNP-complete~\cite{chalkiadakis2011computational,matsui2001np,prasad1990np}. 
As delegative simple games include weighted voting games as a subcase (consider the restriction when each voter votes herself), these hardness results also hold for delegative simple games. 

However, it is known that these indices can be computed by a pseudo-polynomial algorithm~\cite{matsui2001np} in weighted voting games, that is an algorithm running in time $poly(n, w_{\max})$, where $w_{\max}:=\max_{i\in V} \omega(i)$ is the maximal weight of an agent. 
In what follows, we provide a similar dynamic programming approach to compute the delegative Shapley-Shubik and Banzhaf indices in pseudo-polynomial time.

\begin{theorem}\label{thShBaPolynomial}
Given a delegative simple game $\mathcal{G}_{\mathcal{E}}$ induced by an LDE $\mathcal{E} = \langle D = (V,A), \omega, d, q \rangle$ and a voter $i \in V$, $DB_i$ and $DS_i$ can be computed in $O(n^2 w_{max}\max\{n, w_{\max}\})$ and $O(n^4w_{max}^2)$, respectively. 
\end{theorem}

\begin{proof}
Consider a coalition $C \subseteq V$. Observe first that when a coalition $C$ does not include voter $j$, a subset $S$ of $j$'s followers (i.e., $S \subseteq T_d(j) \setminus \{j\}$) could join $C$ only as inactive agents and are not able to increase the total weight of $C$. For instance in Example~\ref{exNotations}, in the case voter $7$ does not join a coalition $C$ (i.e., $\alpha_{d,C}(8)=1$), all of her followers could join $C$ as inactive agents.

By relabeling the vertices we can make the assumption that the vertex we consider is voter $n$.

We run a depth-first search of $H_d$ starting from voter $n$. 
Let $\pi_d$ be the ordering of voters in $H_d$ such that voters are sorted in decreasing order of their discovering times in the depth first search. 
As $n$ is first visited in the depth first search, it is the last voter in the ordering $\pi_d$. In Example~\ref{exNotations}, voters are sorted in such a way (i.e., $\pi_d=<1, 2, 3, 4, 5, 6, 7, 8>$), when computing $DB_8(\mathcal{E})$. We first show how to compute the delegative shapely value.
We decompose the proof in two sub-cases : 

\paragraph{Case 1: voter $n$ is a guru.} 
Consider a guru $n$ with accumulated weight $\alpha_d(n)$. %For every $k \in \{0, ..., \alpha_d(n)-w_n\}$, let $T_d(n,k)$ be the set of all subtrees $T$ rooted in $n$ such that $\sum_{i \in T}w_i=k+w_n$, i.e., each subtree $T \in T_d(n,k)$ represents a possible way that $n$ obtains an accumulated weight $k+w_n$. 
%It is worth noticing that there may be more than one subtree $T \in T_d(n,k)$ in which voter $n$ receives weight $k+w_n$. For instance, in Example~\ref{exNotations}, $T_d(8)$ has two subtrees with accumulated weight $3$ and rooted in $8$ : the first (resp. second) subtree is composed of vertices in $\{6,7,8\}$ (resp. $\{4,7,8\}$). Given a subtree $T$, let $ch(T)$ be the set of children of nodes in $T$. To compute $DS_n$, we need to compute, for every $T \in T_d(n,k)$, $N^k_s(T)$ the number of $s$-element subsets of $V\setminus (T \cup ch(T))$ that have weight in $\{q-k-w_n, ..., q-1\}$, where $s=0, 1, ..., n-|T|-1$ and $k=0, ..., \alpha_n(d)-w_n$. 
Recall that $w_n$ is the initial weight that voter $n$ is endowed with before starting the delegation process and $\alpha_d(n)$ is the total weight that voter $n$ receives through delegations in $H_d$. 
%More formally,  for every $T \in T_d(n,k)$, we have 
%$$N^k_s(T)=\sum_{\substack{C\subseteq V\setminus (T \cup ch(T))\\ 
%|C|=s}} \mathbbm{1}_{q-k-w_n \le \alpha_{d}(C) \le q-1},$$

%where $\mathbbm{1}_{\phi}$ is equal to $1$ if $\phi$ is true, and $0$ otherwise. 
%Let $N_s = \sum^{ \alpha_n(d)-w_n }_{k = 0}\sum_{T \in T_d(n,k)} N^k_{s}(T)$. 
Let $N_s$ denote the number of coalitions $C$ of size $s$ for which $n$ is a swing agent. 
%Now we can compute $DS_n$ as follows. 
Then $DS_n$ can be rewritten as follows.
\begin{align}\label{alignShapely}
    DS_n = \sum_{s=0}^{n-1}\frac{s!(n-s-1)!}{n!}N_s. 
\end{align}

Let $t_j=|T_d(j)|$, i.e., the size of the tree $T_d(j)$ rooted in a vertex $j$. 
Moreover, let $Del(j) = c_d(j,d^*(j))\setminus\{j\}$ be the set of voters to which $j$ delegates to directly or indirectly (not to be confused with the guru of $j$).
To compute $DS_n$ efficiently, we use a dynamic programming approach. 
Given a forest $\mathcal{F}$ with $n$ vertices, we define a table $F_{\mathcal{F}}$ where $F_{\mathcal{F}}[j, w, s]$ is the number of sets $C\subset \{1,...,j\}$ such that $|C| = s$ and $\alpha_d(Del(j)\cup C) = \alpha_d(Del(j)) + w$, where $j$ and $s$ range from $0$ to $n$ and $w$ ranges from $0$ to $\sum_{i \in V}w_i$. In words, we count the number of s-element subsets in $\{1,...,j\}$ who will contribute a weight $w$ when added to a coalition containing all elements of $Del(j)$ (this ensures that $j$ will be an active agent). These table entries will be filled as follows.

First, for $j=0$, we have
\begin{align*}
F_{\mathcal{F}}[0, w, s] \!=\! \left\{ \begin{array}{c c}
1 & \text{ if } w= 0 \text{ and } s=0\\
0 & \text{ otherwise.}
\end{array} \right.
\end{align*}
More generally, $F_{\mathcal{F}}[j, w, s] = 0$ if $s > j$ or $w > \sum_{l=1}^j w_{l}$. Second, if $s = 0$, then $F_{\mathcal{F}}[j, w, s] = 0$ if $w > 0$ and $1$ otherwise. Third, in the special case $w=0$, and $j\ge s > 0$, we have
\begin{align}\label{alignWZeroVoters}
         F_{\mathcal{F}}[j, 0, s]&=\sum_{x = 0}^{ t_j-1} {t_j-1 \choose x}F_{\mathcal{F}}[j - t_j, 0, s - x].
\end{align}
Indeed, in this case $j$ cannot be part of the coalition as she would contribute a positive weight. Conversely, as $j$ is not part of the coalition, any subset of vertices in $T_d(j) \setminus\{j\}$ may be part of the coalition as a set of inactive agents. We consider each possible cardinality (variable $x$) for such a subset before moving to the next tree rooted in $j-t_j$. 


Now for $j=1,\ldots, n$, $s=1,\ldots, j$, and $w=1, \ldots, q-w_n$, $F[j, w, s]$ will be computed  as follows.

\begin{equation}\label{eqRecursiveF}
      \begin{split}
         F_{\mathcal{F}}[j, w, s]&=\sum_{x = 0}^{ t_j-1} {t_j - 1 \choose x}F_{\mathcal{F}}[j - t_j, w, s - x]\\&+ F_{\mathcal{F}}[j-1,w-w_j, s-1]
      \end{split}
\end{equation}
We recall that $F_{\mathcal{F}}[j, w, s]$ is the number of sets $C\subset \{1,...,j\}$ such that $|C| = s$ and $\alpha_d(Del(j)\cup C) = \alpha_d(Del(j)) + w$. Here, the two summands correspond to the cases $j\notin C$ and $j\in C$ respectively.  Note that in the first case, voters in $T_d(j)$ can only join $C$ as inactive agents. Hence in the first summand, we consider all possible ways of adding to $C$ inactive agents from the tree rooted in $j$ before moving to the next subtree (rooted in $j - t_j$).

We use this dynamic programming equations considering two forests $\mathcal{F}_1 = \{T_d(n)\}$ and $\mathcal{F}_2 = H_d - T_d(n)$ of sizes $t_n$ and $n-t_n$, respectively. We conclude by noticing that:
\begin{equation}
N_s = \sum_{k = 0}^s \sum_{w = 0}^{q-1} F_{\mathcal{F}_2}[n-t_n,w,k] (\sum_{w' = q - w}^{\alpha_d(n)} F_{\mathcal{F}_1}[t_n,w',s-k+1]).\label{eq:Ns computation}
\end{equation}

\paragraph{Case 2: voter $n$ is a delegator.}
If $n$ is a delegator, then $n$ can only be a swing agent for coalition $C$ if $Del(n) \subseteq C$. 
Hence, we should count only coalitions which meet this condition. 
To take this fact into account we use our dynamic programming approach on the delegation graph $H_d[V\setminus Del(n)]$. 
Moreover, in this case $N_s$ is obtained by a different formula. Let $C_\delta = Del(n)$, then  we use the formula:   
\begin{equation} \label{eq:Ns computation2}
N_s = \sum_{k = 0}^{s_\delta} \sum_{w = 0}^{q_\delta-1} F_{\mathcal{F}_2}[n-t_n,w,k] (\sum_{w' = q_{\delta} - w}^{\alpha_d(n)} F_{\mathcal{F}_1}[t_n,w',s_{\delta}-k+1]),
\end{equation}
where $s_\delta = s - |C_\delta|$ and $q_\delta = q - \alpha_d(C_\delta)$.

We move to the complexity analysis. %All values $(l \choose k)$ and $k!$ (for $0\le k \le l\le n$) can be computed in $O(n^2)$ and $O(n)$ respectively by dynamic programming. 
The running time of this algorithm is bounded by the time required to fill out the tables $F_{\mathcal{F}_1}$ and $F_{\mathcal{F}_2}$. The size of each table is bounded by $n \times nw_{max} \times n$ and Equation \ref{eqRecursiveF} can be computed in $O(n)$ operations (if values $n\choose k$ are precomputed). This leads to a complexity of $O(n^4w_{max})$ for computing tables $F_{\mathcal{F}_1}$ and $F_{\mathcal{F}_2}$. As Equations \ref{eq:Ns computation} and \ref{eq:Ns computation2} can be computed in $O(n^3w_{max}^2)$, %$O(n^3)$
computing all values $N_s$ can be performed with $O(n^4w_{max}^2)$ operations. Last, we compute the Shapley value which requires $O(n)$ operations. 

For the Banzhaf index, we can simply adapt the dynamic program and omit the third index $s$. Thus, the complexity to fill out both adapted tables $F_{\mathcal{F}_1}$ and $F_{\mathcal{F}_2}$ in this case will be upper bounded by $O(n^3w_{max})$. To compute the Banzhaf index of each agent $n$, we need to find the number of subsets $N\setminus T_d(n)$ having weight at least $q-\alpha_d(n)$ and at most $q-1$. This leads to a complexity of $O(n^2w_{max}\max\{n, w_{max}\})$ for computing the Banzhaf index.
\end{proof}

==> old/Contribution/DynamicProgramming/oldindexvalue.tex <==

%In the first term, $F[j-t_j,w, s-x] $ counts the number of subsets in $\{1, \ldots, j-t_j\}$ that have weight $w$ and size $s-x$ ($0\le x\le t_j-1$) and do not contain $j$ nor her followers. Note that in the case voter $j$ does not join a coalition $C$, each possible subset $S$ of her followers (i.e., $S \subseteq T_d(j)\setminus \{j\}$) could join $C$ as inactive agents. $F[j-1,w-1, s-1]$ counts the number of subsets $C' \subset \{1,\ldots, j-1\}$ such that $|C'| = s$ $w_d(C'\cup C) = w_d(C)+ w$ and size $s$ that contain $j$.

%For instance in Example~\ref{exNotations}, when $C=\{2,3,8\}$, we can move to the subtree $T_d(1)$, $1$ cannot join $C$, but her followers could join $C$ as inactive voters. In this case, $|T_d(1)\setminus\{1\}|=0$.
  
In order to add a subtree $T$ of $T_d(n)$ rooted in $n$ to the resulting coalitions of table $F$, we use another table $X[j',w',s']$ to be the number of $s'$-element subsets of $\{1,..., n-t_n,..., j'\}$ in which voters in $\{1,...,n-t_n\}$ have weight $y'\in \{w',...,q-1\}$, i.e., each $s'$-element subset contains $w'\le y'\le q-1$ active voters of $\{1,...,n-t_n\}$. Here, $j'$ ranges from $t_n$ to $n-1$, $s$ ranges from $0$ to $n-1$ and $w'$ ranges from $0$ to $q-1$. Note that $t_n$ is the last child of $n$.

For $j'=t_n,...,n-1$, $w'=1,...,q-1$ and $s'=1,...,n-1$, $X[j',w',s']$ will be filled as follows. We distinguish two cases.

\begin{enumerate}
    \item $j'-t_{j'}=t_n$. Let $y=q-w'-1$. In this case, we have
    \begin{equation}\label{eqRecursiveHCase1}
      \begin{split}
         X[j', w', s']&=\sum_{y'=0}^{y}\sum_{x = 0}^{ t_{j'}-1} {t_{j'}-1 \choose x}F[n-t_n, w'+y', s' - x] \\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation}
     Let us explain each term separately.
     \paragraph{First term.}  $F[n-t_n,w'+y', s'-x] $ counts the number of subsets that have weight $w'+y'$ ($0\le y' \le y$) and size $s-x$ ($0\le x \le t_j-1$) and do not contain $j'$ nor her followers. Note that if voter $j'$ does not join a coalition $C$, each possible subset $S$ of her followers (i.e., $S \subseteq T_d(j)\setminus \{j\}$) could join $C$ as inactive agents. Furthermore, the interpretation of the first summation that is over weight $y'$ ranges from $0$ to $y$ is as follows. $j'-t_{j'}=t_n$ means that the the rest of voters $\{t_n,...,j'\} \in T_d(n)$ do not join, so a subset of voters in $\{j'+1,..., t_n-1\} \subseteq T_d(n)$ with weight $q-w'$ could join a subset of voters in $\{1,...,n-t_n\}$ with weight $w'+y'$ such that $0\le y'\le q-w'-1$. In other words, when $n$ has a weight $q-w'$ in a $s'$-element subset $C$, all possible subsets of the gurus in $Gu_d\setminus \{n\}$ and their followers that have a weight $y'\in \{w',...,q-1\}$ could join $C$. 
     
     \paragraph{Second term.}The second term $X[j'-1,w'-1, s'-1]$ counts the number of subsets that contain $j'$ and voters in $\{1,...,n-t_n\}$ have weight $y'\in \{w',...,q-1\}$. 
     
     To illustrate the two terms, consider Example~\ref{exNotations}. To compute $DB_8$, when $C=\{8\}$, for $s'=1,...,7$, we have
     \begin{equation*}
      \begin{split}
         X[7, 2, s']&=\sum_{y'=0}^{0}\sum_{x = 0}^{ 3} {3\choose x}F[3, 2+y', s' - x] + X[6,1, s'-1]
      \end{split}
     \end{equation*}
    The first term shows that if voters $7$ does not join $C$ (i.e., $w_8(C)=1$), the rest of voters in $\{1,2,3,4,5,6\}$ with a weight of $2$ could join $C$. Note that voters in $\{4,5,6\}$ could only join $C$ as inactive voters. The second term shows the case where voter $7$ joins $C$.  
       
     \item Otherwise (i.e., $ j'-t_{j'} > t_n$),
     \begin{equation}\label{eqRecursiveHCase2}
      \begin{split}
         X[j', w', s']&=\sum_{x = 0}^{ t_{j'}-1} {t_{j'} - 1 \choose x}X[j' - t_{j'}, w', s' - x]\\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation}
     
     This case concerns those cases in which we move from a subtree in $T_d(n)$ to another subtree in $T_d(n)$. The first term counts the number of $s'$-element subsets a subtree $T \in T_d(n,q-w')$ and $j'\notin T$ (but contain the followers of $j'$ as inactive voters). The second term counts the number of $s'$-element subsets that contain a subtree $T \in T_d(n,q-w')$ and $j'\in T$. voter As an instance, in Example~\ref{exNotations} when $C=\{7,8\}$, we have
     
     \begin{equation*}
      \begin{split}
         X[6,1, s']&=\sum_{x = 0}^{ 1} {1 \choose x}X[4, 1, s' - x]+ X[5,0, s'-1]
      \end{split}
     \end{equation*}
     The first term represents the case where voter $6$ does not join $C$. In this case, voter $5$ could join $C$ as inactive voters and we move to subtree $T_d(4)$. The second term shows the case where $6$ joins $C$.
\end{enumerate}

We need to examine the especial case $w=0$, $j$ ranges from $t_n$ to $n-1$ and $s'$ range from $0$ to $n-1$ separately. Let $y=q-1$, we distinguish three cases.

\begin{enumerate}

 \item $j'- T_d(j')>0$. In this case, we have
     \begin{align}\label{alignWZeroCase1}
         X[j', 0, s']&=\sum_{x = 0}^{ t_{j'}} {t_{j'} \choose x}X[j' - t_{j'}, 0, s' - x]
      \end{align}
     As an example, when $C=\{6,7,8\}$ in Example~\ref{exNotations}, we can move from $5$ to subtree $T_d(4)$, however all voters in subtree $T_d(5)$ could join $C$. 
     \HG{At this point it becomes quite clear that $F[j, 0, s]$ is not well defined !}
   \item $j'-t_{j'}=t_n$. In this case, we have
    \begin{align}\label{alignWZeroCase2}
         X[j', 0, s']&=\sum_{y'=0}^{y}\sum_{x = 0}^{ t_{j'}} {t_{j'} \choose x}F[n-t_n, y', s' - x]
    \end{align}
     For instance in Example~\ref{exNotations}, when going from $5$ to subtree $T_d(4)$, we have this coalition $C=\{6,7,8\}$ ($5$ and her followers may join $C$). Now from $4$ we can move to subtree $T_d(3)$. In this case, voter $8$ could have weight greater than $q=3$ (by joining $5$ and $4$ to $C$), so $4$'s followers and a subtree of $T_d(3)$ with weight $y' \in \{0,1,2\}$ could join $C$.
     
     \item  $j'=t_n$ and $T_d(j')=\emptyset $, i.e., the last child of $T_d(n)$ in the ordering $\pi_d$.
        \begin{align}\label{alignWZeroCase3}
         X[t_n, 0, s']=\sum_{y'=0}^{y} F[n-t_n, y',s]
       \end{align}
        This term shows those cases where the last child of $T_d(n)$ joins a coalition $C\subseteq T_d(n)\setminus \{j'\}$ and $w_n(C)=q$. So a subset of $\{1,..., n-t_n\}$ with weight of $y'=\{0,1,...,q-1\}$ could join $C$. For instance in Example~\ref{exNotations}, when we have this coalition $C=\{7,8\}$ and if $4$ which is the last child of $8$ joins $C$, voters in $\{1,..., n-T_d(n)\}$ with weight of $y' \in \{0, 1,2\}$ could join $C$.
\end{enumerate}

Now, $N_s$, for $s=0, 1, ..., n-1$, can be computed as 

\begin{align*}
    N_s=X[t_n-1, q-1, s].
\end{align*}

In the case $n \notin Gu_d$, in order for $n$ to be an active agent in a coalition $C$, voters $\delta_d(n, d^{*}_n) \cup \{d^{*}_n\}$ have to be contained in $C$. To do so, we consider the set $c_d(n, d^{*}_n)$ as a new node $n'$ and define a new delegation profile $d'$ as follows. For every voter $j$, if $d_j\in c_d(n, d^{*}_n)$, we set $d'_j=n'$; $d'_j=d_j$ otherwise. So, we consider $n'$ as a guru in $H_{d'}$ and the last voter in the ordering $\pi_{d'}$ of $H_{d'}$. For simplicity, we assume that voters $T_d(n)\setminus \{n\}$ precede $n'$ in $\pi_{d'}$, meaning that voters in $T_d(n)\setminus \{n\}$ visited after $n'$ in a depth-first search of $H_{d'}$ starting from $n'$. Also, in this case, we define new quota $q'=q-|\delta_d(n, d^{*}_n) \cup \{d^{*}_n\}|$. Hence, to compute the index value for a voter $n \notin Gu_d$, we can simply consider the delegative simple game of $V'=<N', d', q'>$, where $N'=N \cup \{i'\}\setminus c_d(n, d^{*}_n)$. For instance, to compute $B_6$ in Fig.~\ref{figNotation}, we consider the set $\{6, 7, 8\}$ as a new voter $6'$ and define a new delegation profile $d'=(3,3,3,6',6',6')$ ( see Fig.~\ref{figDelegator'sIndex}). Also, $\pi_{d'}=<1,2,3,4,5,6'>$ in which set $T_d(6)\setminus\{6\}=\{5\}$ precede $6'$. %Therefore, in the rest of the proof, for the sake of simplicity, we assume that $n \in Gu_d$. %One last piece of assumption: here for the sake of simplicity, we assume that voters in $c_d(n, d^{*}_n)$ are first visited in a depth first search, meaning that $\delta_d(n, d^{*}_n)\cup \{n\}$ precede $d^{*}_n$ in $\pi_d$. 

\begin{figure}[h]
		\centering
		\begin{tikzpicture}
				\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white}}
				\tikzset{edge/.style = {->,> = latex'}}
				
				\node[vertex] (6') at  (0,3) {$6'$};
				\node[vertex] (5) at  (-.5,2) {$5$};
				\node[vertex] (4) at (.5,2) {$4$};
				
				\node[vertex] (3) at  (2.5,3) {$3$};
				\node[vertex] (2) at  (2,2) {$2$};
				\node[vertex] (1) at  (3,2) {$1$};
				
				
				
				%edges
				\draw[edge] (5) to (6');
				\draw[edge] (4) to (6');
				
				\draw[edge] (1) to (3);
				\draw[edge] (2) to (3);
		\end{tikzpicture}

		\caption{ The new delegation graph $H_{d'}$ with $q'=1$ is used to compute the voter $6$'s (i.e., the original voter $6$) index power in Example~\ref{exNotations}.} \label{figDelegator'sIndex}
	\end{figure}


 In this case, the table $X$ is only defined on $T_d(n)$. So, Equation~\ref{eqRecursiveHCase1} and~\ref{eqRecursiveHCase2} should respect the delegation profile $d$, meaning that for $j'$ ranges from $t_d(n), ..., n'-1$, $w'=1, ..., q'-1$ and $s'$ ranges from $1$ to $n'-1$, we have:


\begin{enumerate}
    \item $j'- t_{j'}=t_n$. Let $y=q'-1-w'$. In this case, we have
    \begin{equation*}
      \begin{split}
         X[j', w', s']&=\sum_{y'=0}^{y}\sum_{x = 0}^{ t_{j'}-1} {t_{j'} - 1 \choose x}F[j' - t_{j'}, w+y', s' - x] \\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation*}
    For instance in Example~\ref{exNotations}, to compute $B_6$, if voter $5$ does not join the coalition $C=\{6,7,8\}$, we can move to subtree $T_d(4)$ rooted in voter $4 \notin T_d(6) \cap T_d(6')$ (see Figures~\ref{figDelegator'sIndex} and~\ref{figNotation}), but since $q=3$, voter $4$ (and voter $3$) cannot join $C$. However, voters $1$, $2$ and $5$ could join $C$.
     
     \item Otherwise (i.e., $ j'-t_{j'} > t_n$),
     \begin{equation*}
      \begin{split}
         X[j', w', s']&=\sum_{x = 0}^{ t_{j'}-1} {t_{j'}- 1 \choose x}X[j' - t_{j'}, w', s' - x]\\&+ X[j'-1,w'-1, s'-1]
      \end{split}
     \end{equation*}
     
\end{enumerate}

In the same way, in the special case $w'=0$, $j'$ ranges from $t_n$ to $n'-1$ and $s'$ range from $1$ to $n'-1$, Equations~\ref{alignWZeroCase1},~\ref{alignWZeroCase2} and~\ref{alignWZeroCase3} have to respect the delegation function $d$ too. 



Recall that $q'=q-|\delta_d(i, d^{*}_i) \cup \{d^{*}_i\}|$. Now, $N_s$, for $s=0, 1, ..., n-1$, can be computed as follows:

\begin{align*}
 N_s \!=\! \left\{ \begin{array}{c c}
0 & \text{ if } q'\le 0\\
X[n'-1, q'-1, s-|\delta_d(i, d^{*}_i) \cup \{d^{*}_i\}|] & \text{ otherwise.}
\end{array} \right.
\end{align*}

Note that in the case $q' \le 0$, $i'$ is a distant voter and will not be a swing agent for any coalition. For instance, in Example~\ref{exNotations}, voter $5$ is a distant voter since a necessary condition for her to be in any coalition $C$ is that $\{6,7,8\}\subseteq C$, meaning that $\sum_{j \in \hat{D}(C)\setminus \{5\}}w(j) \ge 3$. Thus, $B_5=Sh_5=0$.

We can now compute the shapely value of voter $i=n$. Thus, with memoization, the Shapley value of a voter can be computed in $O(n^{5})$. Because two tables $F$ and $X$ have $n^3$ entries in total and in the worst case, it takes $O(n^2)$ for each entry to be filled.

For the Banzaf index, we can simply omit the third parameter $s$ and compute a voter value, which can be computed in $O(n^{3})$.

%We denote by $d^*(i)$ the guru of voter $i$, i.e., the guru that is found by following delegations from $i$.
%For $C \subseteq N$, let $C^d = \{i\in C| d(i) = i\}$. 
%For any $C \subseteq N$, we write $D(C) = \{j\in N | \exists k\in C, d^*(j) = k\}$.

==> old/Contribution/Modification/delegationmodification.tex <==

\section{Bribery by Delegation Modifications}
\subsection{Power index modification by bribery}
The support structure in delegative simple games induces the following natural question:  which voters should one influence under a budget constraint to maximize/minimize the voting power of a given voter? 
This question leads to the following computational bribery problems.

\begin{center}
\noindent\fbox{\parbox{12cm}{
		\emph{Problems}: \textbf{BMinP}, \textbf{SMinP}, \textbf{BMaxP} and \textbf{SMaxP}\\
		\emph{Input}: An LDE $\mathcal{E} = \langle D= (V, A), \omega, d , q \rangle$, a voter $u \in V$, a budget $k \in \mathbb{N}$, and a threshold $\tau\in\mathbb{Q}_+$.\\
		\emph{Feasible solution}: A delegation function $d'$ s.t. $|\{i\in V : d(i)\neq d'(i)\}|\le k$ leading to an LDE $\mathcal{E}' = \langle D, \omega, d', q \rangle$. \\
		\emph{Question}: Can we find a feasible solution $d'$ such that:
		\begin{center}
		\begin{tabular}{cc}
		     \textbf{BMinP}: $DB_u(\mathcal{E}') \le \tau$? & \textbf{BMaxP}: $DB_u(\mathcal{E}') \ge \tau$?\\
		     \textbf{SMinP}: $DS_u(\mathcal{E}') \le \tau$? & \textbf{SMaxP}: $DS_u(\mathcal{E}') \ge \tau$?\\
		\end{tabular}
		\end{center}
}}\\
\end{center}

Stated otherwise, in the Banzhaf Minimization (resp. Maximization) Problem, \textbf{BMinP} (resp. \textbf{BMaxP}) for short, we wish to determine if we can make the Banzhaf index of voter $u$ lower (resp. greater) than or equal to a given threshold, by only modifying $k$ delegations. This cardinality constraint can be justified by the fact that influencing each voter is costly. 
\textbf{SMinP} and \textbf{SMaxP} are similar problems corresponding to the Shapley-Shubik index.  
While \textbf{BMaxP} and \textbf{SMaxP} correspond to the constructive variant of the bribery problem, \textbf{BMinP} and \textbf{SMinP} correspond to its destructive variant. These bribery problems are natural in the setting of LD, where one voter could for instance try to get the delegations of several other voters to increase her influence on the election. Moreover, we believe these bribery problems are also relevant in more traditional elections where several politicians or political parties could seek which alliances to foster as to increase their centrality or to make an opponent powerless. 


\input{Contribution/Modification/iminp}
\input{Contribution/Modification/imaxp}

\input{Contribution/Modification/wtp}

%\input{Contribution/Modification/iminpbis}

==> old/Contribution/Modification/imaxp.tex <==
%\subsection{Problem IMaxP}
%We show that \textbf{IMaxP} is NP-hard. //Complete by explaining that the result holds with weights in unary. 

\begin{theorem}\label{thIMaxP}
    \textbf{BMaxP} and \textbf{SMaxP} with voters' weights and the quota given in unary are NP-complete.   
\end{theorem}
\begin{proof}
Membership in NP is induced by Theorem~\ref{thShBaPolynomial}. 
For the hardness part, we make a reduction from the NP-complete exact cover by 3-sets problem (X3C)~\cite{garey1979computers}. 
In the X3C problem, we are given a universe $U = \{x_1,\ldots, x_{3n}\}$ of $3n$ elements and a collection $T = \{S_1,\ldots, S_m\} \subset U^3 $ of $m$ subsets of $U$, each containing 3 elements.
The question asked is to determine if there exists a subcollection of $T$ which covers each element of $U$ exactly once.  

Given an instance $(U,T )$ of X3C, with $|U| = 3n$ and $|T| = m$, we create the following instance which is the same (up to the threshold $\tau$) for problems \textbf{BMaxP} and \textbf{SMaxP}. 
The voter set $V= \{v^*,v_d\} \cup V_U \cup V_T$ is composed of one voter $v_d$ with weight $N = 9n^2m + 9 n$, $3n$ element voters $V_U = \{v_{x} : x \in U\}$ with weight $\bar N = 3nm + 3 $, $3mn$ set voters $V_T = \{v_{S^{i}} : S \in T, i\in [3n]\}$ with weight 1, and one voter $v^*$ with weight 1. 
Remark that weights depend only polynomially on $n$.
The digraph $D = (V,A)$ has the following arcs. 
We have arcs from each element voter $v_x$ to each set voter $v_{S^{1}}$ for which $x \in S$, one arc from each set voter $v_{S^{i}}$ to set voter $v_{S^{i+1}}$ for $i\in[3n-1]$ and one arc from each set voter $v_{S^{3n}}$ to $v^*$. The initial delegation graph has no delegations, i.e., $\forall i\in V, d(i)=i$. 
The quota $q$ is set to $9n^2m+3nm+9n+2$. This value is chosen such that 1) $N+\bar N > q$, 2) $3n \bar N + 3nm + 1  < q$, and 3) $N+3nm+1 < q$. Lastly, the budget $k$ is set to $3n + 3n^2$. 

Let us first observe that a coalition $C$ will be successful iff it includes $v_d$ and at least one element voter as active voters. 
Hence, if $v^*$ is a swing agent for a coalition $C$ then first $v_d\in C$, second no element voter is active in $C$, and third $C$ should contain an element voter and a path from this element voter to $v^*$ through a path $(v_{S^1},v_{S^2}, \ldots,v_{S^{3n}},v^*)$ for some set $S\in T$. 

Let $H = (V,L)$ be a delegation graph which is a feasible solution in the \textbf{BMaxP} (resp. \textbf{SMaxP}) instance resulting from the reduction. 
We will say that the $S$-path is active in $H$, if $(v_{S^i},v_{S^{i+1}})\in L$ for $i\in [3n-1]$, and  $(v_{S^{3n}},v^*)\in L$. 
Note that the number of active paths in $H$ is at most $n$ (we do not consider the only feasible solution $H$ with $n+1$ active paths, as $v^*$ is never a swing agent for this solution). 
%For a coalition $C$, let $P(C) \subseteq T$ be the subset of sets $S\in T$ for which the $S$-path is active. 
For a set $S\in T$, we denote by $E_H(S)$ the set of element voters $v_x$ such that $(v_x, v_{S^1})\in L$.

 
Let us assume that there exists an exact cover by 3 sets $\{T_{i_1},\ldots, T_{i_n}\}$. 
Note that by relabeling the indices we can assume that $\{T_{i_1},\ldots, T_{i_n}\} = \{T_{1},\ldots, T_{n}\}$ and $T_i = \{x_{3(i-1)+1}, x_{3(i-1)+2}, x_{3i}\}$. 
We create the following delegation graph $H$. 
We make all voters $v_{x_i}$ delegate to $v_{T_{\lceil i/3 \rceil}^{1}}$ for $i\in[3n]$, all voters $v_{T_i^j}$ delegate to $v_{T_i^{j+1}}$ for $i\in[n]$ and $j\in [3n-1]$ and all voters $v_{T_i}^{3n}$ for $i \in [n]$ to $v^*$. 
Note that (up to the relabeling) $H$ does not depend on the specific exact cover by 3 set. However, such a solution $H$ is feasible only if the X3C instance is a yes instance. Let us show that such a solution $H$ achieves the highest possible delegative Banzhaf and Shapley-Shubik indices for agent $v^*$. Indeed, let us consider another feasible solution $H'$ and let $\{T_{i_1},\ldots,T_{i_t}\}$ be the sets in $T$ whose paths are active in $H'$. By relabeling, we can assume that $\{T_{i_1},\ldots,T_{i_t}\} \subseteq \{T_{1},\ldots,T_{n}\}$ and $E_{H'}(T_i)\subseteq \{x_{3(i-1)+1}, x_{3(i-1)+2}, x_{3i}\}$. The claim then follows by noticing that the set of coalitions for which $v^*$ is a swing agent in $H'$ is a subset of the set of coalitions for which $v^*$ is a swing agent in $H$ and is even a proper subset if $H \neq H'$ (after relabeling).   

We conclude by noticing that the delegative Banzhaf and Shapley-Shubik indices of a solution $H$ corresponding to an exact cover by 3-set can be easily computed. Indeed, this is simply implied by Theorem~\ref{thShBaPolynomial}.

\begin{comment}
\paragraph{Banzhaf value.} Given such a solution $H$, $v^*$ will be a swing agent for all coalitions that contain an element voter $x$ and an $S$-active path such that $x\in E_H(S)$. The number of such coalitions is
\begin{equation*}
    \sum_{k=1}^n {n \choose k} (2^{3n} - 1)^{n-k} 2^{3n(m-n)} (2^{3k}-1)2^{3(n-k)}.
\end{equation*}

Let us explain this formula. We count coalitions which include $k$ active-paths out of the $n$ active paths of $H$, and sum the obtained values for $k$ ranging from 1 to $n$. For a given $k$, these coalitions cannot include completely any of the $n-k$ other active paths. Hence, the number of possible intersections with the set of elements in these $n-k$ paths is of $(2^{3n} - 1)^{n-k}$. 
Conversely there is no constraint on set elements $v_{T_i^j}$ for $i\notin[n]$. Hence, the number of possible intersections with these set elements is worth $2^{3n(m-n)}$. The $k$ active paths in the coalition makes it possible to connect $3k$ element voters to $v^*$. As at least one of them should be included in the coalition, this leaves $(2^{3k}-1)$ possibilities. There are no constraints on the $3(n-k)$ other element voters explaining the last $2^{3(n-k)}$ term. This induces the Banzhaf value of voter $i^*$ for solution $H$. 

\paragraph{Shapley-Shubik value.} We introduce the Table $\Lambda$ where $\Lambda[i,j]$ counts the number of ways we can choose $i$ elements in a set of the form $\{v_{S_l^{t}}, l\in [j], t\in [3n]\}$ without taking all $3n$ elements $\{v_{S^{t}}, t\in [3n]\}$ of a same set $S$. Table $\Lambda$ can be computed efficiently using the following dynamic programming equations: 
\begin{align*}
    \Lambda[i,1]   &= {3n \choose i} \text{ if } i < 3n \text{ and } 0 \text{ otherwise}\\
    \Lambda[i,j>1] &= \sum\limits_{\substack{l=0\\l \le i}}^{3n-1} {3n \choose l} F[i-l,j-1].
\end{align*}
The Shapley value of voter $i^*$ for a solution $H$ corresponding to an exact cover by 3 set can then be derived by the following formula:
\begin{align*}
N_S =& \sum\limits_{\substack{k=1\\ 3nk \le S-2}}^n {n \choose k} \sum\limits_{\substack{i=1\\ 3nk+i \le S-1}}^{3k}{3k\choose i} \\
&\sum\limits_{\substack{j=0\\3nk+i+j\le S-1}}^{3(n-k)} {3(n-k) \choose j} \sum\limits_{\substack{l=0\\3nk+i+j+l\le S-1}}^{3n(m-n)}  {3n(m-n) \choose l} \Lambda[S-1-3nk-i-j-l,n-k]
\end{align*}
Let us explain this formula. We are counting the number of coalitions $C\subset V$ of size $S$ for which $i^*$ is a swing voter. A necessary condition is that $v_d\in C$. Hence, the complement is composed of only $S-1$ voters. We distinguish these coalitions by the number of active paths that they fully include, each such path adds $3n$ voters and at list one should be fully contained. Let us consider coalitions that include $k$ active paths. Then, this makes it possible for $v^*$ to be reachable by $3k$ element voters. We count the number of coalitions that include $i$ such voters (at least one must be included). The rest of voters in the coalition may be arbitrary voters in the rest of element voters, arbitrary voters in paths $\{v_{S^{t}}, t\in [3n]\}$ for $S\not\in\{T_1,\ldots,T_n\}$ or other voters in paths corresponding to sets $S\in\{T_1,\ldots,T_n\}$ given that a full path is not taken. 
\end{comment}
\end{proof}


==> old/Contribution/Modification/iminp.tex <==
%\subsection{Problem IMinP}
We show that all four problems are NP-hard. Note that computing the delegative Banzhaf or Shapley-Shubik indices in these problems is already intractable unless the voters' weights are given in unary. However, our hardness results hold even if voters' weights are given in unary (resp. even if all voters have weight one) for \textbf{BMaxP} and \textbf{SMaxP} (resp. for \textbf{BMinP} and \textbf{SMinP}). 

\begin{theorem}\label{thrm : IMinP is NP-Hard}
    The restriction of \textbf{BMinP} and \textbf{SMinP} to the case where all voters have weight 1, i.e., when $\forall i\in V, \omega(i) = 1$, is NP-complete. 
\end{theorem}
\begin{proof}
The membership in NP is implied by theorem~\ref{thShBaPolynomial}. 
For the hardness part, we use a reduction from the NP-complete Hamiltonian path problem~\cite{garey1979computers}. Recall that in the Hamiltonian path problem, the goal is to determine if there exists a path in an undirected graph that visits each vertex exactly once.  
Consider an instance $I = (V,E)$ of the Hamiltonian path problem, where $V$ is the set of vertices and $E$ is the set of edges.  
We create the following instance from $I$ which is the same for both \textbf{SMinP} and \textbf{BMinP}. We create a digraph $D = (\bar V, \bar E)$ where $\bar V = V\cup\{u\}$ is obtained from $V$ by adding an additional vertex and $\bar E = \{(i,j),(j,i) : \{i,j\} \in E \} \cup \{ (u,i) : i \in V\}$ is obtained from $E$ by adding an arc from $u$ to every other vertex (and making the graph directed). Now consider the delegation graph $H_d \in \Delta(D)$, where all voters vote directly, i.e., $\forall i\in \bar V, d(i) = i$. We set $w_i=1$, for every voter $v_i \in \bar V$. Also, we set $k=|V|$, $q=|V|$ and $\mathcal{E} = \langle D, \omega, d , q \rangle$. Suppose that the goal is to modify $d$ (yielding another delegation function $d'$) in order to make $u$ a distant agent. Indeed, note that $DB_u(\mathcal{G}_{\mathcal{E}'}) = 0$ (resp. $DS_u(\mathcal{G}_{\mathcal{E}'}) = 0$) iff $u$ is a distant agent. We can make $u$ a distant agent in $\mathcal{E}'$ iff there exists a Hamiltonian path in $I$. Indeed, if there exists an Hamiltonian path $(v_1,v_2,\ldots, v_n)$ in $G$ we can make $u$ a distant agent by adding delegations $d'(v_i) = v_{i+1}, \forall i\in [n-1]$  and making $u$ delegate to $v_1$. Conversely, if we can make $u$ a distant agent, then $u$ is at the end of a simple path of length $|V|$ implying that there exists a Hamiltonian path in $I$.
    \end{proof}




==> old/Contribution/Modification/iminpbis.tex <==
\HG{//TO CORRECT AND THEN PUT BACK IN PLACE}
More positively, \textbf{IMinP} becomes tractable when $D$ is complete. We start with the following observation from Zhang and Grossi~\cite{zhang2020power}.


%\begin{fact}[Fact 2 in~\cite{zhang2020power}]\label{factMonotonocity}
%For any pair of agents $i, j \in V(D)$, such that $d_i=j$, $DB_i \le DB_j$.
%\end{fact}

\begin{fact}[Fact 3 in~\cite{zhang2020power}]\label{Direct vs. Indirect Delegation}
given a delegative simple game $V=<N,d,q>$, in
which there exists three agents $i, j, k \in N$, such that $d_i =
j$ and $d_k = i$. Let then $V=<N,d',q>$, such that for any $v \in N\setminus \{k\}$
$d'_v=d_v$ and $d'_k=j$. Then, $DB_k(V')\ge DB_k(V)$.
\end{fact}

The following two modifying operations will be helpful.
\begin{definition}[$Cut(V, j)$]
A modifying operation that, given a delegative simple game $V=<N,d,q>$ in which there exists a follower $j$, outputs another delegative simple game $V=<N,d',q>$ such that for any $i \in N\setminus \{j\}$ $d'_i=d_i$, and $d'_j=j$.
\end{definition}

\begin{definition}[$Join(V,g,j)$]
A modifying operation that, given a delegative simple game $V=<N,d,q>$ in which there exists a guru $g \in Gu_d$, a voter $j$ and $j \notin T_d(g)$, outputs another delegative simple game $V=<N,d',q>$ such that for any $i \in N\setminus \{g\}$ $d'_i=d_i$, and $d'_g=j$. 
\end{definition}

Let $\Delta$ be the running time of computing the index power $f_i(\mathcal{E})$ of any voter $i$ . Let $Leaves(H)$ be the set of all leaves in $H$. 

 The following observation implies that during the procedure of minimizing $f_u$, when it comes to applying the Join operation, we only perform $Join(V,d^*_u,j)$, where $j \in Leaves(H_d)\setminus T_d(d^*_u)$.

\begin{obs}\label{obsDelegatingtoLeaves}
Consider a delegative simple game $V=<N,d,q>$, a voter $u$ and a leaf $l \in Leaves(H_d) \setminus T_d(d^*_u)$. $Join(V,d^*_u,l)$ minimizes $f_u$ more than $Join(V,d^*_u,v)$, where $v \in c_d(l,d^*_l)$.
\end{obs}
\begin{proof}
By the same argument as Zhang and Garossi Showed in Fact 3 in ~\cite{zhang2020power}, we can show that Fact~\ref{Direct vs. Indirect Delegation} holds when $f=DS$. Then, using Fact~\ref{Direct vs. Indirect Delegation}, we see that delegating $d^*_u$ to $l$ results in another delegative simple game in which $f_u \le f_l \le ...\le f_{d^*_l}$. This concludes the proof.
\end{proof}

The following lemma says that $Join(V,d^*_u,j)$ minimizes $f_u$ more than $Join(V,g,j)$, where $g \ne d^*_u$.
\begin{lemma}\label{lmDelegatingu}
Consider a delegative simple game $V=<N,d,q>$, and three voters $u, j$ and $g$, where $d^*_g \ne d^*_u \ne d^*_j$. Consider two delegative simple games $V_1=Join(H_d,d^*_u,j)$ and $V_2=Join(H_d,g,j)$. Then $f_u(V_1) \le f_u(V_2)$.
\end{lemma}
\begin{proof}
Let $C$ be a coalition in $V_1$ for which $u$ is a swing agent. Then, we must have $c(j,d^*_j) \subset C$.  The proof follows by noticing that the active voters in $C$ and $C\setminus\{u\}$ are the same.  
\end{proof}

Consider two gurus $g_1, g_2$ in a delegation graph $H_d$. The following observation says that if $d^*_u$ delegates to a leaf $l_1 \in T_d(g_1)$ and then $g_1$ delegates to a leaf $l_2 \in T_d(g_2)$ decreases $f_u$ as much as $d^*_u$ first delegates to a leaf $l_2 \in T_d(g_2)$ and then $g_2$ delegates to a leaf $l_1 \in T_d(g_1)$.
\begin{obs}\label{obsOrderOfSubtree}
Consider a delegative simple game $V=<N,d,q>$, in which there exists a follower $u$ and two gurus $g_1, g_2$, where $g_1 \ne g_2 \ne d^*_u$. Consider two leaves $l_1 \in T_d(g_1)$ and $l_2 \in T_d(g_2)$. Suppose $V_1=<N,d_1,q>=Join(Join(V, d^*_u, l_1), g_1,l_2)$ and $V_2=<N,d_2,q>=Join(Join(V, d^*_u, l_2), g_2,l_1)$. Then $f_u(V_1) = f_u(V_2)$.
\end{obs}
\begin{proof}
It is easy to see that in both $V_1$ and $V_2$, $c_{d_1}(u,d^*_u)=c_{d_2}(u,d^*_u)$. So, the number of coalitions that $u$ is swing is the same in both $V_1$ and $V_2$.
\end{proof}


\begin{obs}\label{obsUnnecessaryCutIntermediate}
Consider a delegative simple game $V=<N,d,q>$, in which there exists a follower $u$. During the procedure of minimizing $f_u$, it is unnecessary to apply the $Cut(V,j)$ operation, where $j \in c_d(u, d^*_u)$.
\end{obs}

\HG{Why ?}
\begin{proof}
Let $\mathcal{A}$ be an algorithm that applies the $Cut(V,j)$ operation for some $j \in c_d(u, d^*_u)$ at some point to minimize $f_u$. Let $H_{d'}$ be the resulting delegation graph after applying $Cut(V,j)$. Keep in mind that $j$ is now the guru of $u$ in $H_{d'}$, i.e., $d'^*_u=j$ and $d'^*_u \ne d^*_u$. The only reason $\mathcal{A}$ would apply this operation is that to delegate $j$ to another leaf in subtree $T_d(d^*_u) \setminus T_d(j)$ in the future. Suppose that this is not the case, i.e., $\mathcal{A}$ will not delegate $j$ to another leaf $l \in T_d(d^*_u)\setminus T_d(j)$ in the next steps. So, $\mathcal{A}$ will delegate $j$ to some other leaves $l \in Leaves(H_d) \setminus T_d(d^*_u)$. Now let $\mathcal{A'}$ be another algorithm that does not apply $Cut(V,j)$ and follows the same sequence of operations as $\mathcal{A}$ after performing $Cut(V,j)$ does. We see that $f_u$ is decreased by $\mathcal{A'}$ more than by $\mathcal{A}$, as the number of intermediate voters between $u$ and her guru in the delegation graph resulting from $\mathcal{A'}$ is more than the number of intermediate voters between $u$ and her guru in the resulting graph from $\mathcal{A}$. This implies that the only reason $\mathcal{A}$ would perform the operation $Cut(V,j)$ in $H_d$ is that to delegate $j$ to another leaf in subtree $T_d(d^*_u) \setminus T_d(j)$ in the future. Consider the graph $H_{d'}$ resulting from $Cut(V,j)$. After applying $Cut(V,j)$, using Observation~\ref{obsOrderOfSubtree}, suppose that $\mathcal{A}$ delegates $d'^*_u=j$ to one of the leaves $l \in T_d(d^*_u) \setminus T_d(j)$. Let $i$ be the voter where $d_i \in c_d(u, d^*_u)$ and $l \in T_d(i)$. Let $\mathcal{A''}$ be the algorithm that does not apply $Cut(V,j)$ and instead applies $Cut(V,i)$ and then delegates $d^*_u$ to $l$. Let $H_{d''}$ be the resulting graph. We see that $c_{d''}(u,d''^*_u)=c_{d'}(u, d'^*_u)$. After this, suppose that $\mathcal{A''}$ would follow the same sequence of operations as $\mathcal{A}$ does. This concludes the proof.
\end{proof}


The following observation implies that to minimize $f_u$, it is unnecessary to execute the $Cut(V,j)$ operation for $j \in V \setminus T_d(d^*_u)$.
\begin{obs}\label{obsUnnecessaryCut}
Consider a delegative simple game $V=<N,d,q>$, in which there exists a follower $u$. During the procedure of minimizing $f_u$, it is unnecessary to apply the $Cut(V,j)$ operation, where $j \notin T_d(d^*_u)$ and the budget $k \ge 2$.
\end{obs}

\begin{proof}
Let $\mathcal{A}$ be the algorithm that applies $Cut(V,j)$ for some $j \notin T_d(d^*_u)$ at some point when $k \ge 2$. We distinguish two cases:
\begin{enumerate}
    \item $\mathcal{A}$ would perform $Cut(V,j)$ to delegate the guru of $u$ to a leaf $l \in T_d(j)$ in the future, using Observation~\ref{obsDelegatingtoLeaves}. After applying $Cut(V,j)$, using Observation~\ref{obsOrderOfSubtree}, $\mathcal{A}$ would delegate $j$ to a leaf $l \in T_d(d^*_j) \setminus T_d(j)$ and then delegates the guru of $u$ to a $l' \in T_d(j)$ (or, using Observation~\ref{obsOrderOfSubtree}, first delegates the guru of $u$ to $l$ and then delegates $d^*_j$ to $l'$). We see that we can first delegate the guru of $u$ to $l'$, so now $j$ is in the same subtree $T$ as $u$ is and then delegates $j$ to $l$, which concludes the proof.
    
    \item After applying $Cut(V,j)$, $\mathcal{A}$ would \textbf{not} delegate the guru of $u$ to a leaf $l \in T_d(j)$ in the next steps. Let $\mathcal{A'}$ be another algorithm that instead of applying $Cut(V,j)$, performs $Join(V,d^*_u,l)$ and then follows the same sequence of operations that $\mathcal{A}$ would perform after applying the $Cut(V,j)$ operation. It is easy to see that $\mathcal{A'}$ works better, which implies the observation.
\end{enumerate}
 %
\end{proof}
Now we are ready to present the greedy algorithm that minimizes $f_u$. We term this algorithm GreedyMin. GreedyMin considers the following sub-cases:

\begin{enumerate}
    \item If $k=1$. Using Lemma~\ref{lmDelegatingu}, Observation~\ref{obsDelegatingtoLeaves},~\ref{obsOrderOfSubtree},~\ref{obsUnnecessaryCutIntermediate},~\ref{obsUnnecessaryCut}, GreedyMin only has two options: it should either apply $Cut(V, j)$ for any $j \in V \setminus c(u, d^*_u)$ \HG{Why not $Cut(V, j)$ for $j \in V \setminus T_d(d^*_u)$} or perform $Join(V, d^*_u, l)$ for any $l \in Leaves(H_d) \setminus T_d(d^*_u)$. \HG{Why not $Join(V, t, l)$ for $t\in T_d(d^*_u)$. (this is not taken into account in your lemma)} \HG{It is not proven also that we must also consider leaves}. Now it can compare in which option $f_u$ is minimized the most. This step takes $O(n\Delta)$. \label{casePowerMin: k=1}
    
    \item $k=2$. Using Lemma~\ref{lmDelegatingu}, Observation~\ref{obsDelegatingtoLeaves},~\ref{obsOrderOfSubtree},~\ref{obsUnnecessaryCutIntermediate},~\ref{obsUnnecessaryCut}, GreedyMin follows two strategies. In the first strategy, it first performs $Join(V, d^*_u, l)$ for any leaf $l \in Leaves(H_d) \setminus T_d(d^*_u)$. Now, it follows Case~\ref{casePowerMin: k=1}. In the second strategy, for any $j \in T_d(d^*_u)$, it first performs the $Cut(V, j)$ operation and now proceeds as Case~\ref{casePowerMin: k=1}. \HG{I don't get why this would be optimal.} It takes $O(n^2\Delta)$ to realize which strategy minimizes $f_u$ the most. \label{casePowerMin: k=2} \HG{In any case, if $k\le 2$, you can try all possibilities.}
    
     \item If $k \ge 3$. In this case, GreedyMin first assumes that $k=2$ and then follows the same strategy stated in Case~\ref{casePowerMin: k=2}. Then it decreases the budget $k$ by $2$, i.e., $k=k-2$. Now if $k=1$, it follows Case~\ref{casePowerMin: k=1}; it follows Case~\ref{casePowerMin: k=2} otherwise. GreedyMin repeats this strategy until $k=0$. This takes $O(kn^2\Delta)$. 
\end{enumerate}



\begin{lemma}\label{lmIMinComplete}
GreedyMin solves \textbf{IMinP} optimally in $O(n^3\Delta)$ time when the social network is complete.
\end{lemma}

\begin{proof}
Using Lemma~\ref{lmDelegatingu}, Observation~\ref{obsDelegatingtoLeaves},~\ref{obsUnnecessaryCutIntermediate},~\ref{obsUnnecessaryCut}, to minimize $f_u$, we only need to apply a sequence of operations $Cut(V, j)$ and $Join(V,g,j)$, where in the first operation $j \in T_d(d^*_u) \setminus c_d(u, d^*_u)$, and in the second operation $g=d^*_u$ and $j \in Leaves(H_d) \setminus T_d(d^*_u)$. Keep in mind that after each delegation, the guru of $u$ will be updated. So, in each step, we only need to check which possible operation makes $u$ more powerless as GreedyMin does. Note that maybe there exists another algorithm $\mathcal{A}$ that delegates the guru of $u$ to the same set of subtrees as GreedyMin does but in a different order. Using Observation~\ref{obsOrderOfSubtree}, both GreedyMin and $\mathcal{A}$ work the same. Thus GreedyMin returns an optimal solution for \textbf{IMinP} in $O(n^3\Delta)$ as $k \le n$. 
\end{proof}

%GreedyMin returns an optimal solution to \textbf{IMinP} when $k=1,2$. It remains to show that this holds when $k \ge 3$. In the following, by having $d^*_u$ delegating to a subtree $T$, we mean that $d^*_u$ will delegate to one of the leaves $l \in T$ that minimizes $f_u$ the most. Let $T_i$ be the tree that $d^*_u$ delegating to it in the $i$'s step. Suppose that $T_1, T_2, ..., T_{k'}$ be the sequence of trees that GreedyMin selects to have $d^*_u$ delegating to them. Keep in mind that after each delegation, $d^*_u$ will be updated. Let $f^{T_i}_u$ be the index power of voter $u$ after delegating to subtree $ T_i$ in $i$'s step. Consider an optimal algorithm $\mathcal{A}$ for \textbf{IMinP}. Let $T'_1, T'_2, ..., T'_{k''}$ be the sequence of trees that algorithm $\mathcal{A}$ picks to have $d^*_u$ delegating to them. For the sake of simplicity, we suppose that $k'=k''$. Suppose that for any $j <i< k$, $T_j=T'_j$ in both GreedyMin and algorithm $\mathcal{A}$. Now assume that at step $j+1$, $T'_{j+1} \ne T_{j+1}$. We distinguish two cases.
%\begin{enumerate}
 %   \item $f^{T'_{j+1}}_u=f^{T_{j+1}}_u$. In this case, GreedyMin works optimally \HG{I would say this is wrong. Because even if $f^{T'_{j+1}}_u=f^{T_{j+1}}_u$, the fact that $T_{j+1}\neq T'_{j+1}$ could have an impact at further iterations of the algorithm.}.
    
  %  \item Otherwise, since GreedyMin selects each subtree with respect to $f^{T_i}_u$, $f^{T_{j+1}}_u < f^{T'_{j+1}}_u$. Since algorithm $\mathcal{A}$ is an optimal algorithm, it will select $T_{j+1}$ in the future \HG{Again this argument seems wrong to me or not explained because it is unclear that $f^{T_j+1}_u$ does not depend on previous choices}. By contradiction, suppose that for any $i \in j+2, \dots, k''$, $T'_{i} \ne T_{j+1}$. We see that $\mathcal{A}$ can replace one of $T'_{i}$ by $T_{j+1}$ to decrease $f_u$ more, which contradicts the assumption that $\mathcal{A}$ is an optimal algorithm. So, there exists $T'_{i}=T_{j+1}$ and by using Observation~\ref{obsOrderOfSubtree}$, \mathcal{A}$ could first have $u$ delegating to $T_{j+1}$ and then to $T'_{j+1}, T'_{j+2}, \dots, T'_{i-1}$.
%\end{enumerate}

==> old/Contribution/Modification/wtp.tex <==
\subsection{Problem \textbf{WMaxP}}
As shown by  Theorems~\ref{thrm : IMinP is NP-Hard} and \ref{thIMaxP}, problems \textbf{BMinP}, \textbf{SMinP}, \textbf{BMaxP} and \textbf{SMaxP} are NP-hard. We also believe that these problems are complex in the sense that the power indices they rely on can be hard to grasp for people not used to solution concepts from cooperative game theory. In this subsection, instead of maximizing the power index of a voter, we study a problem with a related but conceptually simpler objective. Indeed, we investigate if we can modify at most $k$ delegation choices to make the accumulated weight of a given voter $i^*$ (i.e., the size of the delegation tree rooted in her) greater than or equal to a given threshold $\tau$. 
%A voter could indeed be interested in obtaining a given accumulated weight $\tau$. 
Possible interesting values for $\tau$ can be $q$ or $\sum_{i\in V} \omega(i) - q + 1$. In the first case, $i^*$ and her supporters do not need the support of anyone else to reach the election quota. In the second case, $i^*$ is sure that she has enough weight to veto the election. We term this optimization problem \textbf{WMaxP} for Weight Maximization Problem. It is clear that problems \textbf{WMaxP}, \textbf{BMaxP} and \textbf{SMaxP}  are related in the sense that a greater voting weight may result in a greater power index value. 
However, it is well known from the literature in weighted voting games that this relation is limited as voters with sensibly different weights may have the same relative importance in the election. It is worth mentioning that if the given voter receives too much weight, we may end up in a situation where the voter's power gets decreased (see Observation~\ref{obs:md}).

We now formally introduce the \textbf{WMaxP} problem. Note that this problem does not require to know the quota of the election. Hence, we define a Partial LDE (PLDE) as a tuple $\mathcal{E} = \langle D= (V, A), \omega, d \rangle$, i.e., an LDE without a quota value.

\begin{center}
\noindent\fbox{\parbox{12cm}{
		\emph{Problems}: \textbf{WMaxP}\\
		\emph{Input}: A PLDE $\mathcal{E} = \langle D= (V, A), \omega, d \rangle$, a voter $i^* \in V$, a budget $k\in\mathbb{N}$, and a threshold $\tau \in \mathbb{N} $.\\
		\emph{Feasible Solution}: A delegation function $d'$ s.t. $|\{i\in V : d(i)\neq d'(i)\}|\le k$ leading to a PLDE $\mathcal{E}' = \langle D, \omega, d'\rangle$. \\
		%\emph{Feasible Solution}: A delegation graph $H^{'} = (V, A^{'})\in \Delta(D)$ corresponding to a delegation function $d'$ s.t. $|A^{'} \setminus A|\le k$. \\
		\emph{Question}: Can we find a feasible solution $d'$ such that $\alpha_{d'}(i^*) \ge \tau$.
		%\emph{Question}: Does there exist  delegation graph $H' = (V, A^{'})\in \Delta(G)$ s.t. $|A^{'} \setminus A|\le k$ and $u\in Gu_{d'}$ such that $w_{d'}(u) \ge \tau$.
}}\\
\end{center}


We first show that \textbf{WMaxP} is NP-complete and that the optimization variant of the problem  cannot be approximated with an approximation ratio better than $1-1/e$ if $P\neq NP$.

\begin{theorem}\label{thWTP}
	\textbf{WMaxP} is NP-complete and the optimization variant of the problem cannot be approximated with an approximation ratio better than $1-1/e$ if $P\neq NP$, even when all voters have weight one.
\end{theorem}	
\begin{proof}
The membership in NP is straightforward. 
Let us prove the approximation hardness result (the NP-hardness result can be proved by a similar reduction).
\begin{comment}
We give a reduction from an instance $I$ of the set cover problem to an instance $ I^{'} $ of \textbf{WTP}. Recall that in the set cover problem, we are given a universe $ U = \{x_1,\ldots, x_N\}$ of $N$ elements, a collection $ S=\left\lbrace S_1, S_2, ..., S_M \right\rbrace $ of subsets of $ U $, and an integer $k$. We wish to determine if we can pick at most $k$ sets such that all elements are covered. 
	    
\paragraph{The reduction.} 
          From an instance $I = (U,S,k)$ of the set cover problem, we create an instance $I'$ of \textbf{WTP} as follows. 
          As illustrated in Figure~\ref{figIMPhardness}, the graph $G = (V,E)$ is compounded of the following elements:
          \begin{itemize}
           \item{Voter $v_{i}$ for each element $ x_i \in U $. These voters will be called element voters or element nodes in the following.}
    	  \item{One node $ v_{S_j} $ is created for each $ S_j \in S $. These voters will be called set voters or set nodes in the following.
	      For every $ i \in [N] $ and $ j \in [M] $, we create a directed edge from $ v_i $ to $ v_{S_j} $ if  $ x_i \in S_j$.}
	      \item We create a voter $u$. For every $ j \in [M] $, we create a directed edge from $v_{S_j}$ to $u$.
	      \item For every $i \in [N]$, we create a set $\mathcal{V}_i$ with $M$ nodes. We create a directed edge from each node in set $\mathcal{V}_i$ to element voter $v_i$.
    	  \item We define a budget $\bar{k}=N+k$.
    	  \item We define a threshold $\tau=N(M+1)+k+1$.
     \end{itemize}		 

		
      \paragraph{The delegation graph $H_d$.}
      Consider the delegation graph $ H_d \in \Delta(G)$ induced by $d$, where 
      all set voters, all element voters and voter $u$ vote directly. Also, for each $i \in [N]$, each voter in set $ \mathcal{V}_i$ delegates to element voter $v_i$. 
      
      Now suppose the goal is to change at most $\bar{k}$ delegations in $H_d$ in order to find another delegation graph $H_{d'}$ in which the number of voters who support $u$ is equal to $\tau$. Clearly, voter $u$'s weight will reach the threshold $\tau$ if all element voters delegate to $k$ set voters, so these set voters could delegate to $u$ and transfer their weights to voter $u$. It is easy to see that finding such $k$ set voters $S_j \in S$ in $H_d$ is equivalent to pick $k$ sets in the instance $I = (U,S,k)$ of the set cover problem to cover all elements in $U$. Therefore, \textbf{WTP} is NP-complete.
%\end{proof}


\begin{figure}[t]
\centering
\scalebox{0.75}{
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white,minimum size = 4mm}}
\tikzset{edge/.style = {->,> = latex'}}

\node[vertex][minimum size=1.1cm] (u) at  (1,1.7) {$u$};
\node[vertex][minimum size=1.1cm] (vs1) at  (-.5,0) {$v_{S_1}$};
\node[vertex][minimum size=1.1cm] (vs2) at  (1,0) {$v_{S_2}$};
\node[vertex][minimum size=1.1cm] (vs3) at  (2.7,0) {$v_{S_M}$};

%\node[vertex][minimum size=2cm] (Clique) at (5.5,0.5)  {$\mathcal{I}$};

\node[vertex][minimum size=1.1cm] (v1) at  (-2,-1.5) {$v_{1}$};
\node[vertex][minimum size=1.1cm] (v2) at (1,-1.5) {$v_{2}$};
\node[vertex][minimum size=1.1cm] (vn) at (4.2,-1.5) {$v_{N}$};

\node[vertex][minimum size=1.5cm] (v21) at  (-2,-3.3) {$\mathcal{V}_1$};
\node[vertex][minimum size=1.5cm] (v22) at (1,-3.3) {$\mathcal{V}_2$};
\node[vertex][minimum size=1.5cm] (v2n) at (4.2,-3.3) {$\mathcal{V}_N$};



\path (vs2) to node {\dots} (vs3);
\path (v2) to node {\dots} (vn);
\path (v22) to node {\dots} (v2n);

\draw[edge] (vs1) to (u);
\draw[edge] (vs2) to (u);
\draw[edge] (vs3) to (u);

\draw[edge] (v1) to (vs1);
\draw[edge] (v1)[bend right = 10] to (vs3);
\draw[edge] (v2) to (vs1);
\draw[edge] (v2) to (vs2);
\draw[edge] (vn) [bend left = 10] to (vs1);
\draw[edge] (vn)  to (vs3);

\draw[edge] (v21) to (v1);
\draw[edge] (v22) to (v2);
\draw[edge] (v2n) to (vn);

\end{tikzpicture}}
\caption{An example of graph $G$ resulting from the reduction. %The set $\mathcal{I}$ includes $K$ isolated nodes.
For every $i\in [N]$, each set $\mathcal{V}_i$ includes $M$ nodes, where there exists a directed edge from each node in $\mathcal{V}_i$ to the element voter $v_i$.} \label{figIMPhardness}
\end{figure}

%\begin{theorem}\label{thCAP}
%	There is an approximation factor preserving reduction from the maximum coverage problem to \textbf{WTP}.
%\end{theorem}
% \begin{proof}
\end{comment} 
	    We design a reduction from the maximum coverage problem. 
	    In the maximum coverage problem, we are given a universe $ U = \{x_1,\ldots, x_n\}$ of $n$ elements, a collection $ P=\{ S_1, S_2, ..., S_m \} $ of $m$ subsets of $U$, and an integer $k$. The goal is to pick at most $k$ sets $S_{i_1},\ldots,S_{i_k}$ such that $|\bigcup_{j=1}^{k} S_{i_j}|$ is maximized. Stated otherwise, we want to cover the maximum number of elements in $U$.
	    This problem is known to be hard to approximate better than $1 - 1/e$~\cite{feige1998threshold}. 

	    \paragraph{The reduction.} 
          From an instance $I = (U,P,k)$ of the maximum coverage problem, we create the following instance $I'$ of the optimization variant of \textbf{WMaxP}. 
          As illustrated in Figure~\ref{figPreservinghardness}, the graph $D = (V,A)$ is compounded of the following elements:
          \begin{itemize}
           \item{For each element $x \in U$, we create a voter $v_{x}$. These voters will be called element voters or element vertices in the following.}
    	  \item{For each set $S \in P$, we create $(n+1)$ voters $v_{S^{1}}, \dots, v_{S^{(n+1)}}$. We create an arc from $v_{S^{i}}$ to $v_{S^{(i+1)}}$ for $i\in [n]$. These voters will be called set voters or set vertices in the following.
	      \item For every $ x \in U$ and $ S \in P $, we create an arc from $v_x$ to $v_{S^{1}}$ if  $x \in S$.}
	      \item We create a voter $v^*$. For every $ S \in P$, we create an arc from $v_{S^{(n+1)}}$ to $v^*$.
	      \item For every $x \in U$, we create a set $\mathcal{V}_x$ with $M-1$ vertices where $M:= ((n+1)m+1)T$ and $T$ is a constant the value of which will be discussed later on. We create an arc from each vertex in $\mathcal{V}_x$ to element voter $v_x$.
    	  \item We define a budget $\bar{k}=(n+1)k+n$.
     \end{itemize}		 
     All voters have weight equal to one. In the initial delegation function, we have that $\forall x \in U, d(v_x) = v_x$, $\forall S \in P,\forall i\in [n+1], d(v_{S^{i}}) = v_{S^{i}}$, and $d(v^*) = v^*$. Last, we have that $\forall x \in U$, and $\forall u\in \mathcal{V}_x, d(u) = v_x$.
	
	Let us consider a delegation function $d'$, such that $|\{i\in V:d(i)\neq d'(i)\}|\le \bar k$.
	We say that the $S$-path is active for $d'$ if $d'(v_{S^{i}}) = v_{S^{(i+1)}}$ for $i\in [n]$ and $d'(v_{S^{(n+1)}}) = v^*$. Note that the budget only allows $k$ $S$-paths to be active and we denote by $\mathcal{S}(d')$ the set of sets $S$ such that the $S$-path is active for $d'$. 
	Moreover, we will say that an element $x$ is covered by $d'$ if $d'(v_x) = v_{S^{1}}$ for some set $S\in P$ such that the $S$-path is active for $d'$. We denote by $\mathcal{U}(d')$ the set of elements covered by $d'$.
	
	It is easy to notice that $|\mathcal{U}(d')|M \le \alpha_{d'}(v^*) \le |\mathcal{U}(d')|M + M/T$ (we assume that delegations from voters in sets $\mathcal{V}_i$ do not change as this can only  be counter-productive for the problem at hand). Let us assume we have a $c$-approximation algorithm for \textbf{WMaxP}. Let $d'$ be the solution returned by this algorithm and $d^*$ be the optimal solution. Then,
	$(|\mathcal{U}(d')| + 1/T)M \ge \alpha_{d'}(v^*) \ge c \alpha_{d^*}(v^*)$.  
	
	Let $OPT$ be the optimal value of the maximum coverage instance and $X^*$ be an optimal solution. Consider the delegation function $d_{X^*}$ obtained from $d$ by making each $S$-path for which $S\in X^*$ active and making each element voters $v_x$ delegate to $v_{S^1}$ if $x$ is covered by $S$ in solution $X^*$ (the choice of $S$ can be made arbitrarily if several sets cover $x$ in $X^*$). It is clear that $d_{X^*}$ is a valid solution such that $|\mathcal{U}(d_{X^*})| = OPT$. Hence, $\alpha_{d^*}(v^*) \ge \alpha_{d_{X^*}}(v^*) \ge |\mathcal{U}(d_{X^*})|M = OPT \cdot M$. Hence, we obtain that $|\mathcal{U}(d')| + 1/T \ge c OPT$. We conclude by noticing that $\mathcal{S}(d')$ provides a solution in the maximum coverage instance covering the elements in $\mathcal{U}(d')$ and that by making $1/T$ tend towards $0$, we would obtain a $c(1-\epsilon)$ approximation algorithm for the maximum coverage problem with $\epsilon$ as close to 0 as wanted. 
	
      %Now suppose the goal is to change at most $\bar{k}$ delegations in $H_d$ in order to find another delegation graph $H_{d'}$ in which the number of voters who support $u$ is maximized. %is a critical agent for any $C$ in $H'_d$.
      %Note that voters in $\mathcal{I}$ with total weight $K = N (M-k+1)-M+2k$ are isolated from the rest of graph. Clearly, voter $u$ will be a critical agent for any $C \subseteq V$ if all element voters and their followers delegate to $u$ through set voters indirectly. 
      %As $M-k > N$, voter $u$'s weight will be maximized if all element voters delegate to $k$ set voters, so in this way, the voting power of their followers can be transferred to $u$. Since $\bar{k}=Nk+n$, the number of voters who can support $u$ is 
      %\begin{align*}
      %    \bar{N} &=(M-k+1)n+Nk\\
      %    &\ge (M-k+1)n+nk  \quad \text{ as $n < N$}\\
      %    &=(M+1)n
      %  \end{align*}
    %Let $OPT$ be the maximum number of elements that is covered by selecting $k$ sets in instance $I$, then in the worst case $\bar{N} = (M+1)OPT$, i.e., $\bar{N}$ is proportional to the number of elements that is covered in the maximum coverage problem. 
        
     %\HG{You do not show the soundness of the reduction you have to show that an $\alpha$-approximation algorithm for \textbf{WTP} provides the same for Maximum Coverage.}
    %Now Let $\mathcal{A}$ be an algorithm for the Max-coverage problem with approximation ratio $0 \le c \le 1$. Now after running the algorithm $\mathcal{A}$ on instance $I$, the maximum number of elements that is covered is equal to or greater than $c.OPT$. Let $\mathcal{A'}$ be an algorithm that, given the delegation graph $H_d$, runs $\mathcal{A}$ to select a subset of set voters to delegate the maximum number of element voters to these set voters. Using the fact that $\bar{N} = (M+1)OPT$, $\mathcal{A'}$ constructs a solution (i.e., a delegation graph $H_{d'}$) to \textbf{WTP} in which $w_{d'}(u) \ge c.(M+1)OPT$. Therefore, $\mathcal{A'}$ is a $c$-approximation algorithm. 
\end{proof}


\begin{figure}[t]
\centering
\scalebox{0.75}{
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white,minimum size = 4mm}}
\tikzset{edge/.style = {->,> = latex'}}

\node[vertex][minimum size=.6cm, label=left:{$v^*$}] (u) at  (1,2.8) {};
\node[vertex][minimum size=.6cm, label=left:{$v_{S_{1}^{n+1}}$}] (vs1N) at  (-.6,1.3) {};
\node[vertex][minimum size=.6cm, label=left:{$v_{S_{1}^2}$}] (vs12) at  (-1.1,.2) {};
\node[vertex][minimum size=.6cm, label=left:{$v_{S_{1}^1}$}] (vs11) at  (-1.5,-.7) {};

\node[vertex][minimum size=.6cm, label=left:{$v_{S_{2}^{n+1}}$}] (vs2N) at  (1,1.3) {};
\node[vertex][minimum size=.6cm, label=left:{$v_{S_{2}^2}$}] (vs22) at  (1,.2) {};
\node[vertex][minimum size=.6cm, label=left:{$v_{S_{2}^1}$}] (vs21) at  (1,-.7) {};

\node[vertex][minimum size=.6cm, label=right:{$v_{S_{m}^{n+1}}$}] (vsmN) at  (2.6,1.3) {};
\node[vertex][minimum size=.6cm, label=right:{$v_{S_{m}^2}$}] (vsm2) at  (3.2,.2) {};
\node[vertex][minimum size=.6cm, label=right:{$v_{S_{m}^1}$}] (vsm1) at  (3.7,-.7) {};

%\node[vertex][minimum size=.6cm] (vs2) at  (1,0) {$v_{S_2}$};
%\node[vertex][minimum size=.6cm] (vs3) at  (2.7,0) {$v_{S_M}$};

%\node[vertex][minimum size=2cm] (Clique) at (5.5,0.5)  {$\mathcal{I}$};

\node[vertex][minimum size=.6cm, label=left:{$v_{x_1}$}] (v1) at  (-2,-1.8) {};
\node[vertex][minimum size=.6cm, label=left:{$v_{x_2}$}] (v2) at (1,-1.8) {};
\node[vertex][minimum size=.6cm, label=right:{$v_{x_n}$}] (vn) at (4.2,-1.8) {};

\node[vertex][minimum size=1.5cm, label=left:{$\mathcal{V}_{x_1}$}] (v21) at  (-2,-3.3) {};
\node[vertex][minimum size=1.5cm, label=left:{$\mathcal{V}_{x_2}$}] (v22) at (1,-3.3) {};
\node[vertex][minimum size=1.5cm, label=right:{$\mathcal{V}_{x_n}$}] (v2n) at (4.2,-3.3) {};



\path (vs21) to node {\dots} (vsm1);
\path (vs22) to node {\dots} (vsm2);
\path (vs2N) to node {\dots} (vsmN);
\path (v2) to node {\dots} (vn);
\path (v22) to node {\dots} (v2n);


\draw[edge] (vs1N) to (u);
\draw[edge] (vs2N) to (u);
\draw[edge] (vsmN) to (u);

\draw[edge] (v1) to (vs11);
\draw[edge] (vs11) to (vs12);
\draw[edge] (vs21) to (vs22);
\draw[edge] (vsm1) to (vsm2);
\path[draw, dotted] (vs12) edge (vs1N);
\path[draw, dotted] (vs22) edge (vs2N);
\path[draw, dotted] (vsm2) edge (vsmN);

\draw[edge] (v1)[bend right = 10] to (vsm1);
\draw[edge] (v2) to (vs11);
\draw[edge] (v2) to (vs21);
\draw[edge] (vn) [bend left = 10] to (vs11);
\draw[edge] (vn)  to (vsm1);

\draw[edge] (v21) to (v1);
\draw[edge] (v22) to (v2);
\draw[edge] (v2n) to (vn);

\end{tikzpicture}}
\caption{An example of digraph $D$ resulting from the reduction. For every $x\in U$, each set $\mathcal{V}_x$ includes $M-1$ vertices, where there exists an arc from each vertex in $\mathcal{V}_x$ to the element voter $v_x$. For each $S \in P$, there exists a directed path $(v_{S^1}, v_{S^2}, \dots, v_{S^{n+1}}, v^*)$.} \label{figPreservinghardness}
\end{figure} 

\paragraph{A parameterized complexity point of view.} We now define the two following parameters: 
\begin{itemize}
    \item We denote by $\bar{\mathtt{req}} = \sum_{i\in V} \omega(i) - \tau$ the amount of voting weight that $i^*$ does not need to reach the threshold $\tau$;
    \item We denote by $\mathtt{req} = \tau - \alpha_d(i^*)$ the amount of additional voting weight that $i^*$ needs to reach the threshold $\tau$.
\end{itemize} 
We study the parameterized complexity of \textbf{WMaxP} with respect to these two parameters. It can indeed be expected that the problem becomes easier if one of them is small. If $\bar{\mathtt{req}}$ is small, then the combinations of voters that may not delegate to $i^*$ in a solution $d$, such that $\alpha_d(i^*)\ge \tau$, are probably limited.  Conversely, if $\mathtt{req}$ is small, then the number of voters that $i^*$ needs an additional support of to reach $\tau$ is small. These intuitions indeed yield positive parameterized complexity results (Theorems~\ref{thrm: XP for req bar} and \ref{thrm: FPT for req}). These two parameters seem to be opposite from one another. Indeed a small value for parameter $\bar{\mathtt{req}}$ (resp. $\mathtt{req}$) indicates that reaching the threshold $\tau$ is probably hard (resp. easy). Parameter $\bar{\mathtt{req}}$ could for instance be small if $\tau = q$ and the election is conservative (i.e., $q$ is close to $\sum_{i \in V} \omega(i)$). Meanwhile, parameter $\mathtt{req}$ can be small if %$\tau = \sum_{i\in V} \omega(i) - q + 1$, and 
$i^*$ has already a large voting power.\\

We start with parameter $\bar{\mathtt{req}}$.
\begin{theorem}\label{thrm: XP for req bar}
	\textbf{WMaxP} is in XP with respect to parameter $\bar{\mathtt{req}}$.
\end{theorem}
To prove this theorem we fist show that \textbf{WMaxP} can be solved in polynomial time if $\bar{\mathtt{req}} = 0$. 
\begin{lemma}\label{lemma : WTP req bar is 0}
\textbf{WMaxP} can be solved in polynomial time if $\bar{\mathtt{req}} = 0$. 
\end{lemma}
\begin{proof}[Proof sketch]
Let $I = (\langle D = (V,A),\omega, d , k\rangle, i^*, k, \tau)$ be an instance of \textbf{WMaxP} where $\bar{\mathtt{req}} = 0$. Note that to reach the threshold in this case, we should make all voters delegate to $i^*$ by modifying at most $k$ delegations. %Let us denote by $H_d = \{T_d(v_{1}), \ldots, T_d(v_l)\}$ the forest of initial delegations given in input, where $T_d(v_i)$ denotes a tree rooted in $v_i$ (i.e., with guru $v_i$). 

Let us consider a delegation function $d'$ such that $|\{i : d(i)\neq d'(i)\}| \le k$, and $\alpha_{d'}(i^*) = \tau$ (assuming such a solution exists). 
Even if $i^*$ is not a guru in $d$, notice that $i^*$ is necessarily a guru in $d'$. Indeed, $i^*$ needs the delegations of every other voters including the ones in $c_d(i^*, d^*_{i^*})$, and we should not have a cycle in $d'$. Hence, we can assume that $i^*$ is a guru in $d$, decreasing the budget $k$ by one if it is not the case. Now consider the weighted digraph $\bar D = (V, \bar A, \lambda)$, where 
\begin{itemize}
    \item $\bar A$ is obtained from $A$ by removing the outgoing edges from $i^*$ and then reversing all the other edges;
    \item $\lambda((u,v)) = n + 1 $ if $d(v) = u$ and $\lambda((u,v)) = n$, otherwise.  
\end{itemize}
A branching $b$ of $\bar D$ is a set of edges such that (i) if $(x_1,y_1)$, $(x_2,y_2)$ are distinct edges of $b$ then $y_1 \neq y_2$ (nodes have in-degree at most one); and (ii) $b$ does not contain a cycle. An optimum branching $b$ of  $\bar D$ is one that maximizes $\sum_{e \in b} \lambda(e)$. 
We run Edmond's algorithm on $\bar D$~\cite{edmonds1967optimum} to find an optimum branching $b$. 
Let $\Gamma(b)$ be the number of edges in $b$, and $\Omega(b)$ be the number of edges $(u,v)$ in $b$ such that $d(v) = u$. 
It is clear that $\sum_{e \in b} \lambda(e) = \Gamma(b) n + \Omega(b)$. 
As $\Omega(b) \le n-1$, an optimum branching lexicographically maximizes the value of $\Gamma$ and then the one of $\Omega$. We claim that $I$ is a yes instance iff $\Gamma(b) = n-1$, and  $\Omega(b) \ge n-1-k$.  Indeed, notice that one obtains a one to one correspondence between branchings and delegation graphs by simply reversing the arcs. Having $\Gamma(b) = n-1$, implies that there is only one root in the branching, i.e., only one vertex with no incoming edge, and hence only one guru in the corresponding delegation function. As we have removed possible delegations of $i^*$, this guru is necessarily $i^*$. Additionally, $\Omega(b) \ge n-1-k$ implies that at most $k$ delegations choices are changed w.r.t. $d$. 
\end{proof}

\begin{proof}[Proof of Theorem \ref{thrm: XP for req bar}]
As voters' weights are positive integers, the maximum number of voters that $i^*$ does not necessarily need the support of to reach the threshold is bounded by $\bar{\mathtt{req}}$. One can hence guess the set $C$ of voters that are not required with $|C|\le \bar{\mathtt{req}}$. Indeed, the number of possible guesses is bounded by $\frac{|V|^{\bar{\mathtt{req}}+1}- |V|}{|V| - 1}$. Let $X\subset V$ be one such guess. Once these voters are removed from the instance, we obtain another instance of \textbf{WMaxP} in which (if the guess is correct) $i^*$ should obtain the support of all other voters. This amounts to solving an instance of \textbf{WMaxP} where $\bar{\mathtt{req}} = 0$. Hence, it can be solved in polynomial time by Lemma~\ref{lemma : WTP req bar is 0}.
\end{proof}

Hence, interestingly \textbf{WMaxP} can be solved in polynomial time if $\bar{\mathtt{req}}$ is bounded by a constant. However, unfortunately, \textbf{WMaxP} is W[1]-hard w.r.t. $\bar{\mathtt{req}}$ and hence is unlikely to be FPT for this parameter. 

\begin{theorem}
	\textbf{WMaxP} is W[1]-hard with respect to $\bar{\mathtt{req}}$, even when all voters have weight one.
\end{theorem}
\begin{proof}
We design a parameterized reduction from the Independent Set problem. In the Independent Set problem, we are given a graph $G = (V,E)$ and an integer $k$ and we are asked if there exists an independent set of size $k$. The Independent Set problem is W[1]-hard parameterized by $k$. From an instance $I = (G= (V,E),k)$ of the Independence Set problem, we create the following \textbf{WMaxP} instance. We create a digraph $D = (\bar V, \bar A)$ where: 
\begin{itemize}
    \item $\bar V = U \cup W \cup \{i^*\} $ with $U = \{u_v : v\in V\}$ and $W = \{w_e, w_e^1,\ldots, w_e^{k} : e \in E\}$.
    \item $\bar A = \{(u_v,i^*) : v\in V\} \cup \{(w_e,u_v) : e\in E, v\in V, v \in e\}\cup \{(w_e^1,w_e),\ldots,(w_e^k,w_e) : e \in E\}$.
\end{itemize}
All voters have weight one. The initial delegation function is such that $d(x) = x$ for $x\in U \cup \{i^*\}\cup\{w_e : e \in E\}$ and  $d(w_e^j) = w_e$ for each $j\in [k]$ and $e \in E$. The budget $\bar k = |E|+|V| - k$ and $\tau$ is set to $(k+1)|E| + |V| - k + 1$. Hence, $\bar{\mathtt{req}} = k$. We show that the instance of the Independent Set problem is a yes instance iff the instance of the \textbf{WMaxP} problem is a yes instance. To reach the threshold of $\tau$, $i^*$ necessarily needs the delegations of all voters $w_e$. This requires spending a budget of $|E|$ to make all voters $w_e$ delegate to some voters in $U$ (which should then delegate to $i^*$). Then, there only remains a budget $|V|-k$ to make these voters in $U$ delegate to $i^*$. Hence, we can reach the threshold $\tau$ iff we can make all voters in $\{w_e : e \in E\}$ delegate to less than $|V|-k$ voters in $U$. This is possible iff $I$ is a yes instance.        
\end{proof}

Let us now consider parameter $\mathtt{req}$. Interestingly, \textbf{WMaxP} is FPT with respect to $\mathtt{req}$. 
\begin{theorem} \label{thrm: FPT for req}
	\textbf{WMaxP} is FPT with respect to $\mathtt{req}$.
\end{theorem}
\begin{proof}
Let $I = (\langle D = (V,A),\omega, d , k\rangle, i^*, k, \tau)$ be an instance of \textbf{WMaxP}. 
As voters' weights are positive integers, the maximum number of additional voters that $i^*$ needs the support of to reach the threshold is bounded by $\mathtt{req}$. 
We first note that one can collapse the tree $T_d(i^*)$ in one vertex with weight $\alpha_d(i^*)$.  
Let us consider a delegation function $d'$ such that $|\{i : d(i)\neq d'(i)\}| \le k$, and $\alpha_{d'}(i^*) \ge \tau$ (assuming such a solution exists). 
A subtree of $T_{d'}(i^*)$ rooted in $i^*$ with at most $\mathtt{req}+1$ voters accumulates a voting weight greater than or equal to $\tau$. We denote this tree simply by $T$. 
One can guess the shape of $T$ and  then look for this tree in $D$. Note that $T$ should be a directed tree with all vertices delegating directly or indirectly to $i^*$. 
This can be done in FPT time by adapting a color coding technique~\cite{alon1995color}. 
The idea is to color the graph randomly with $\mathtt{req}+1$ colors. 
If the tree that we are looking for is present in graph $D$, it will be colored with the $\mathtt{req}+1$ colors (i.e., one color per vertex) with some probability only dependent of $\mathtt{req}$. We say that such a tree is colorful. Let $r$ be an arbitrary vertex in $T$. 
In $O(2^{O(\mathtt{req})}k^2|A|)$ time, we find, for each vertex $v\in V$, all color sets that appear on colorful copies of $T$ in $G$ in which $v$ plays the role of $r$. 
More precisely, for each colorset $C$, we do not only keep one element but rather at most $k+1$ elements. Indeed, two trees $T_C$ and $T_C'$ rooted in $r$ with colors $C$ are not equivalent in the sense that one may have a higher accumulated weight than the other; we use $\alpha(T_C)$ to denote this weight in tree $T_C$. Moreover $T_C$ may only be part of a valid solution for \textbf{WMaxP} if $|(u,v) \in T_C, d(u) \neq v| \le k$;  we use $\delta(T_C)$ to denote $|(u,v) \in T_C, d(u) \neq v|$. Hence, for each color set $C$, we keep at most $k+1$ elements: For each $i\in[k]_0$, we keep the tree $T_C$ with highest value $\alpha(T_C)$ for $\delta(T_C) = i$. 
This is done by dynamic programming. If $T$ contains only a single vertex, this is trivial.  Otherwise, let $e = (r,r')$ be an arc in $T$.  The removal of $e$ from $T$ breaks $T$ into two subtrees $T'$ and $T''$. We recursively find, for each vertex $v \in V$, the color sets that appear on colorful copies of $T'$ in which $v$ plays the role of $r$, and the color sets that appear on colorful copies of $T''$ in which $v$ plays the role of $r'$. 
For every arc $e = (u,v)\in A$, if $C'$ is a color set that appears in $u$'s collection corresponding to $T'$ and $(\alpha(T_{C'}), \delta(T_{C'}))$ is one of the $k+1$ elements recorded for $C'$, if $C''$ is a color set that appears in $v$'s collection (corresponding to $T''$), and $(\alpha(T_{C''}), \delta(T_{C''}))$ is one of the $k+1$ elements recorded for $C''$. If $C'\cap C'' = \emptyset$ and $\delta(T_{C'})+ \delta(T_{C''}) + 1_{d(u) = v} \le k$, then $C'\cup C''$ is added to the collection of $u$ (corresponding to $T$) with pair $(\alpha(T_{C'}) + \alpha(T_{C''}), \delta(T_{C'}) + \delta(T_{C''}) + 1_{d(u) \neq v})$. Note that if an element already exists for $\delta(T_{C'}) + \delta(T_{C''}) + 1_{d(u) \neq v}$ and color set $C'\cup C''$, then this one only replaces it if it has a higher accumulated weight.  The algorithm succeeds with guess $T$ if one obtains in $i^*$ the complete set $C$ of $\mathtt{req}$ colors with an element $T_C$ with $\alpha(T_{C})\ge \tau$. 
This algorithm can then be derandomized using families of perfect hash functions~\cite{alon1995color,schmidt1990spatial}.

\end{proof}

==> old/Contribution/contribution.tex <==

\input{Contribution/DynamicProgramming/indexvalue}
\input{Contribution/Modification/delegationmodification}
\input{Contribution/Distribution/powerdistribution}
\input{Contribution/Characterisation/axiom}

==> old/Introduction.tex <==

\section{Introduction}\label{secIN}
Weighted voting games form a simple scheme to model situations in which voters must make a yes/no decision about accepting a given proposal~\cite{chalkiadakis2016weighted}. 
Each voter has a corresponding weight and the proposal is accepted if the sum of weights of agents supporting the proposal exceeds a fixed threshold also called the quota. 
In weighted voting game, weights of voters can represent an amount of resource and the quota represents the quantity of this resource which should be gathered to enforce the proposal. 
For instance, agents may be political parties and weights could be derived from the relative importance of each party in terms of number of votes received. 
There is a large literature in cooperative game theory to measure the relative importance of each agent in such a situation. 
Notably, the computational and axiomatic properties of two power indices, the Banzhaf and Shapley-Shubik indices~\cite{banzhaf1964weighted,shapley1953value}, have been extensively studied. 
The computational properties investigated obviously include the computational complexity of computing the power index of a given agent~\cite{deng1994complexity} but they also involve several manipulation problems, as computing the quota maximizing or minimizing the power index of a specific voter~\cite{zick2011,zuckerman2012manipulating} or  determining the impact of splitting an agent in two~\cite{aziz2011false,felsenthal1998measurement,laruelle2005critical}. These are only few examples of the many questions that have been investigated in weighted voting games, despite the apparent simplicity of these cooperative games. 

One possible limitation of weighted voting games is that they consider each agent as an indivisible entity. However, if the agents are corporations or political parties, then they do have some inner structure which may have an impact on the relative strength of each agent. 

\begin{exmp}\label{example: two political parties}
Let us consider two political parties $\Pi$ and $\Pi'$ represented in Figure~\ref{fig: parties pi and pip}. 
Each party has a political leader (agents $A$ and $A'$ respectively) and different inner political trends with subleaders (agents $B$, $C$, $D$, $E$ in $\Pi$ and agents $B'$, $C'$, and $D'$ in $\Pi'$). 
Each leader and subleader have their own supporters which provide them some voting weights, written next to each agent in Figure~\ref{fig: parties pi and pip}. 
In each party, the different agents form a directed tree structure of support, where each arc represents the fact that an agent supports another agent.  
For instance, in party $\Pi$, agent $D$ endorses agent $B$ which herself endorses agent $A$. 
In this way, agent $D$ implicitly supports agent $A$ and puts at her disposal her voting weight.  
Note however that it may not be possible for agent $D$ to directly endorse agent $A$. Indeed, if agent $D$ represents the most left-wing sensibility of the party whereas agent $A$ represents a more consensual political trend, it may be difficult for agent $D$ to publicly support agent $A$ without losing credibility in the eye of her supporters. 

The total weight accumulated by voters $A$ and $A'$ are respectively worth 12 and 11. Hence, the total weight gathered by $A$ is greater than the one of $A'$. Could this indicate that agent $A$ is at least as powerful as agent $A'$. The inner structures of parties $\Pi$ and $\Pi'$ suggest that it may not be the case. Indeed, agent $A$ receives a greater total weight and is endorsed (directly and indirectly) by more agents. However, agent $A'$ receives direct support from all other subleaders of her party  which is not the case of agent $A$. As a result, if agent $B$ decides to secede and create her own party, then agent $A$ would lose the support of agents $D$ and $E$ conceding a total weight lose of 5. Conversely, the most important weight lose that agent $A'$ can suffer from the secession of another agent is worth 3. Hence, the inner structure of political party $\Pi'$ which supports candidate $A'$ seems more robust than the one of candidate $A$.   

\begin{figure}
    \centering
\begin{tikzpicture}
				\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white}}
				\tikzset{edge/.style = {->,> = latex'}}
				
				\node[] (Pi) at  (-2,0) {$\Pi$};
				
				\node[vertex] (A) at  (0,0) {A};
				\node[] (Aw) at  (0.5,0) {3};
				\node[vertex] (B) at  (-1,-1) {B};
				\node[] (Bw) at  (-0.5,-1) {2};
				\node[vertex] (C) at  (1 ,-1) {C};
				\node[] (Cw) at  (1.5,-1) {4};
				\node[vertex] (D) at  (-2,-2) {D};
				\node[] (Dw) at  (-1.5,-2) {1};
				\node[vertex] (E) at  (0,-2) {E};
				\node[] (Ew) at  (0.5,-2) {2};
				
				\draw[] (-3,1) to (2,1) to (2,-3) to (-3,-3) to (-3,1);
				
				
				%edges
				\draw[edge] (B) to (A);
				\draw[edge] (C) to (A);
				\draw[edge] (D) to (B);
				\draw[edge] (E) to (B);
				
				
				\node[] (Pip) at  (4,0) {$\Pi'$};
				
				\node[vertex] (A') at  (5.5,0) {A'};
				\node[] (A'w) at  (6,0) {3};
				\node[vertex] (B') at  (4 , -1.5) {B'};
				\node[] (B'w) at  (4.5 , -1.5) {3};
				\node[vertex] (C') at  (5.5 ,-1.5) {C'};
				\node[] (C'w) at  (6,-1.5) {2};
				\node[vertex] (D') at  (7,-1.5) {D'};
				\node[] (D'w) at  (7.5,-1.5) {3};

				\draw[] (3,1) to (8,1) to (8,-3) to (3,-3) to (3,1);
				
				
				%edges
				\draw[edge] (B') to (A');
				\draw[edge] (C') to (A');
				\draw[edge] (D') to (A');
		\end{tikzpicture}
    \caption{Two political parties $\Pi$ and $\Pi'$ with two different inner structures.}
    \label{fig: parties pi and pip}
\end{figure}
\end{exmp}

Example~\ref{example: two political parties} suggests to study a more complex model than the one of weighted voting games where agents are backed up by an internal support structure with transitive supports. Studying this kind of model has been recently initiated by Zhang and Grossi~\cite{zhang2020power}. 
Indeed, the authors investigate how to measure the relative importance of voters in the framework of \emph{Liquid Democracy} (LD)~\cite{behrens2014principles,ford2020liquid}. 
LD is a collective decision paradigm in which agents can vote themselves or delegate their vote to another agent. 
One important feature, is that an agent who receives delegations can in turn delegate her vote and the ones that she has received to another agent which is exactly the kind of transitive support discussed in Example~\ref{example: two political parties}. 
In their work, Zhang and Grossi~\cite{zhang2020power} define \emph{delegative simple games}, a variant of weighted voting games in which the capacity of a subset of agents to reach the quota does not only depend on their voting weights but also on their delegations. 
Delegative simple games make it possible to take into account the support (delegation) structure underlying the game and to favor agents who receive more direct supports, compared to agents receiving more distant chains of support.  The authors notably study axiomatically the Banzhaf index applied to this kind of game which they term the \emph{delegative Banzhaf index}. 

\paragraph{Our contribution.} In this work, we study in more depth the delegative Banzhaf and Shapley-Shubik indices. While the computation of these indices is computationally hard, we show that they can be calculated by a pseudo-polynomial dynamic programming algorithm similar to the one of standard Banzhaf and Shapley-Shubik indices. %Second, we provide an axiomatic characterization of the delegative Shapley-Shubik index.
Second, we study a bribery problem, in which one tries to maximize/minimize the voting power/weight of a given agent by changing at most $k$ delegation choices. We show that these problems are NP-hard and provide several parameterized complexity results. Lastly, we investigate a power distribution problem in which one tries to find a delegation graph with a predefined number of gurus to maximize the minimum power index value of an agent. We show that this is an NP-hard problem even when the weight of each voter is $1$.

==> old/Problem/coalitiongames.tex <==
\section{Preliminaries} \label{sec : Preliminaries}
In this section, we formalize delegative simple games~\cite{zhang2020power} and specify our setting.  

\subsection{Weighted voting games and power indices}
A simple game is a tuple $\mathcal{G} = \langle V, \nu \rangle$, where $V = [n]$ is a set of $n$ agents and $\nu : 2^n\rightarrow\{0,1\}$ is a characteristic function which only takes values 0 and 1. The notation $[i]$ and $[i]_0$ will denote the sets $\{1,\ldots i\}$ and  $\{0,1,\ldots, i\}$ respectively.  
Moreover, a subset $C\subseteq V$ will also be called a coalition. 
For any coalition $C \subseteq V$, $C$ is said to be a winning coalition if $\nu(C) = 1$, otherwise, it is said to be a losing coalition. An agent $i$ is said to be a swing agent for coalition $C$ if $\delta_i(C):=\nu(C\cup\{i\}) - \nu(C)$ is equal to 1. 

Weighted voting games are particular simple games which admit a compact representation. In weighted voting games, there exists a quota $q$ and each agent (also called voter) $i$ is associated with a weight $w_i$. The characterization function $\nu$ is then defined by $\nu(C) = 1$ iff $\sum_{i \in C} w_i \ge q$. Stated otherwise, a coalition is winning if the sum of weights of agents in the coalition exceeds the threshold. Several power indices have been studied to measure the relative importance of an agent in weighted voting games. We recall two of the most well known power indices:

\begin{definition}
The Banzhaf index of a voter $i$ in a simple game $\mathcal{G}$ is defined as 
$$B_i(\mathcal{G}) = \sum_{C\subseteq V\setminus\{i\}} \frac{1}{2^{n-1}} \delta_i(C).$$
\end{definition}

\begin{definition}
The Shapley-Shubik voting index of a voter $i$ in a simple game $\mathcal{G}$ is defined as 
$$Sh_i(\mathcal{G}) = \sum_{C\subseteq V\setminus\{i\}}\frac{1}{n}\frac{(n - |C| - 1)!|C|!}{(n-1)!}\delta_i(C).$$
\end{definition}
In words, the Banzhaf and Shapley-Shubik indices of an agent $i$ measure how likely it is that $i$ is a swing agent for specific probability distributions on coalitions $C\subseteq V\setminus\{i\}$. For the Banzhaf index, each such coalition is equally likely. For the Shapley-Shubik index, the coalitions are drawn as follows: one first selects u.a.r. a number $s$ in $[n-1]_0$; then one selects a coalition $C\subseteq V\setminus\{i\}$ u.a.r. within coalitions of size $s$.

In a weighted voting game, voters debate on a given proposal and their weights can be seen as amounts of resource related to the proposal at hand.  
A coalition is then successful if it can gather enough of this resource to realize the proposal. For instance, voters may be heads of political parties and the weights could be derived from the relative importance of each party. However, as explained in the introduction, this simple intuition neglects the inner structure of each agent, which could be of importance.  Zhang and Grossi followed this intuition and defined delegative simple games, a variant of weighted voting games~\cite{zhang2020power} which makes it possible to take into account this structure. 
Delegative simple games are motivated by liquid democracy elections.  





==> old/Problem/liquidgames.tex <==
%\section{Simple Games and Liquid Democracy}
\subsection{Liquid democracy elections}
A finite set of agents $V = [n]$ will vote on a proposal. 
Each agent is associated with a weight $w_i$, i.e., there is a weight function $\omega: V \longrightarrow \mathbb{N}_{>0}$, assigning a positive weight $w_i$ to every agent $i$. 
In LD elections a special case of interest is the one where every voter has weight one. 
The rule used is a super-majority rule with quota $q \in (\frac{\sum_{i \in V}w_i}{2},\sum_{i \in V}w_i] \cap \mathbb{N}_{>0} $\footnote{In this work, we restrict the values of weights $w_i$ and $q$ to $\mathbb{N}_{>0}$. This restriction can be motivated by a result by Muroga~\cite{muroga1971threshold}. }. Stated otherwise, the proposal is accepted if the total voting weight in favor of it is at least worth $q$. 

We assume the election to follow the LD paradigm. Notably, we assume voters to be vertices of a Social Network (SN) modeled as a directed graph $D = (V, A) $, i.e., each node in the graph corresponds to a voter $i \in V$ and a directed edge $(i, j) \in A $ corresponds to a social relation between $i$ and $j$. More precisely, it specifies the fact that agent $i$ would accept to delegate her vote to $j$ or more generally speaking to endorse $j$.  The set of out-neighbors (resp.\ in-neighbors) of voter $i$ is denoted by $\mathtt{Nb}_{out}(i)= \left\lbrace j \in V | (i,j) \in A \right\rbrace$ (resp.\ $\mathtt{Nb}_{in}(i)= \left\lbrace j \in V | (j,i) \in A \right\rbrace$). Each agent $i$ has two possible choices: either she can vote directly, or she can delegate her vote to one of her neighbors in $\mathtt{Nb}_{out}(i)$. As usual in LD, delegations are transitive, meaning that if voter $i$ delegates to voter $j$, and voter $j$ delegates to voter $k$, then voter $i$ indirectly delegates to voter $k$. If an agent votes, she is called a \textit{guru} of the people she represents and has an \emph{accumulated voting weight} equal to the total weight of people who directly or indirectly delegated to her. If she delegates, she is called a \textit{follower} and has an accumulated voting weight worth  $0$. 
The information about delegation choices is formalized by a delegation function $d$, where
\begin{itemize}
	\item $ d(i)=j$ if voter $i$ delegates to voter $j \in \mathtt{Nb}_{out}(i)$,
	\item $d(i)=i$ if voter $i$ votes directly.
\end{itemize}
%Agents can vote themselves (in this case they are called gurus) or delegate to another agent (in this case they are called delegators). $d_i = j\neq i$ if $i$ delegates to $j$ and $d_i = i$ if voter $i$ votes.
We write $d=(d_1, d_2, ..., d_n)$ to denote a \textit{delegation profile}, representing each voter's delegation choice, i.e., $d_i=d(i)$ for any $i \in [n]$. The delegation digraph $H_d = (V,E)$ resulting from $d$ is the subgraph of $D$, where $(i,j)\in E$ iff $d(i) = j$. We assume that this digraph is acyclic. More precisely, we assume $H_d$ is a spanning forest of directed trees where all vertices have out-degree exactly one except the roots which have out-degree 0. In $H_d$, we denote by $c_d(i,j)$ the delegation chain between voters $i$ and $j$, which starts with voter $i$ and ends with voter $j$. Put another way, $c_d(i,j)$ is a sequence $((v_1,v_2),\ldots,(v_{k-1},v_k))$ of arcs such that $v_1 = i$, $v_k = j$ and $\forall l\in [k-1], d(v_l)=v_{l+1}$. By abuse of notation, we may also use this notation to denote the set $\{v_i,i\in[k]\}$ of voters in the chain of delegations from $i$ to $j$. For any digraph $D$, we write $\Delta(D)$ to denote the set of all acyclic delegation graphs $H_d$ that can be induced by delegation functions $d$ on $D$.

\subsection{Delegative Simple Games}
Consider a social network $D=(V,A)$ and a delegation graph $H_d=(V,E) \in \Delta(D)$. Let $T_d(i)$ be the directed subtree rooted in $i$ in delegation graph $H_d$, where $i$ has out-degree 0 and all other vertices have out-degree 1. 
Let $Gu_d=\{i \in V | d_i=i\}$ be the set of gurus induced by $d$, i.e., the roots of the directed trees in $H_d$. The voter who votes on behalf of voter $i$ is called the \textit{guru} of $i$ and denoted by $d^{*}_i$ in $H_d$. 
The delegation function $d$ induces an \emph{accumulated weight function} $\alpha_d$, such that $\alpha_d(i) = \sum_{j \in T_d(i)} w_j$ if $i\in Gu_d$ and 0 otherwise. 
We define another weight function. 
Given a set $C \subseteq V$, we denote by $T_d(i,C)$ the directed subtree rooted in $i$ in the delegation graph $H_d[C]$. 
The subtree $T_d(i,C)$ contains each voter $h$ such that $d^*_h = i$ and $c_d(h,i)$ only contains elements from $C$. 
Given a set $C \subseteq V$, we define the weight function $\alpha_{d,C}$, such that $\alpha_{d,C}(i) = \sum_{j \in T_d(i,C)} w_j$ if $i\in Gu_d$ and 0 otherwise.
Moreover, we denote by $\alpha_d(C) = \sum_{i\in C} \alpha_{d,C}(i)$.

We follow and slightly adapt some notations from Zhang and Grossi~\cite{zhang2020power}. 
We call a Liquid Democracy Election (LDE) a tuple $\mathcal{E} = \langle D, \omega, d, q \rangle$ or $\mathcal{E} = \langle D, \omega, H_d, q \rangle$ (by abuse of notation, we may use $H_d$ in place of $d$ when it is convenient). 
For $C \subseteq V$, we denote by $d^*_C(h) = j$ the fact that $j$ is the guru of $h$ and that $c_d(h,j)$ only contains elements from $C$. 
We write $\hat{D}(C) = \{j\in C| \exists k\in C, d^*_C(j) = k\}$ the set of voters that have a guru in $C$ and such that the chain of delegations leading to this guru is contained in $C$. 
In a delegation graph $H_d$, a voter $i$ is called a \textit{distant} agent if $\alpha_d(c_d(i, d^*_i) \setminus \{i\}) \ge q$. 

In the delegative simple game $\mathcal{G}_{\mathcal{E}}$ induced by an LDE $\mathcal{E}$, $\nu_{\mathcal{E}}(C) = 1$ iff $\alpha_{d}(C) \ge q$, i.e., a coalition $C$ is winning whenever the sum of weights accumulated by gurus in $C$ from agents in $C$ meets the quota. %The delegative Banzhaf index of an agent $i$ is defined as the Banzhaf index of $i$ in the delegative simple game of $V$, $DB_i(V) = B_i(G_V)$.  
This defines a new class of simple games which have a compact structure but different from the one of weighted games. 
In our case, the weights are not given in advance, but rather derived from a graph structure. 
The different power indices defined for simple games can of course be applied to this new class.  
It is worth noticing that in this new class of simple games the power of each voter $i$ does not only depend on the amount of delegations she receives through delegations, but also on the structure of the subtree rooted in her in the delegation graph. Notably, the more direct the supports of $i$ are, the more important she is in the delegation graph.


\begin{definition}[Active Agent]\label{defActiveAgent}
Consider a delegation graph $d$ and a coalition $C \subseteq V$. We say that a voter $i \in C$ is an \emph{active} agent in $C$, if $i \in \hat{D}(C)$; 
otherwise, $i$ is called an \emph{inactive} agent. 
\end{definition}

Notice that according to the definition of delegative simple game, an active (resp. inactive) agent $i \in C$ contributes weight $w_i$ (resp. $0$) to the coalition $C$ (see Example~\ref{exNotations}). Given a delegative simple game $\mathcal{G}_{\mathcal{E}}$, let $DB_i(\mathcal{E})$ and $DS_i(\mathcal{E})$ denote the Banzhaf and Shapley-Shubik values of voter $i$ in $\mathcal{G}_{\mathcal{E}}$, respectively. Sometimes we may write $B_i(\mathcal{G}_{\mathcal{E}})$ (resp. $S_i(\mathcal{G}_{\mathcal{E}})$) instead of $DB_i(\mathcal{E})$ (resp. $DS_i(\mathcal{E})$). When speaking about these indices, we drop parameter $\mathcal{E}$ (or $\mathcal{G}_{\mathcal{E}}$) when it is clear from the context. These values are referred to as the delegative Banzhaf and Shapley-Shubik indices of voter $i$. 
Let us give an illustrative example to understand all aspects and notations of our model.

\begin{exmp}\label{exNotations}
Consider an LDE $\mathcal{E} = \langle D = (V , A), \omega, d, q \rangle$, where $V=[8]$ is a set of $8$ voters delegating through a social network with  delegation profile $d=(3, 3, 3, 7, 6, 7, 8, 8)$ illustrated in Fig.~\ref{figNotation} and $q=3$. Each voter $i$ has weight $\omega(i) = 1$. The set of gurus is $Gu=\{3, 8\}$, so, $\alpha_d(3)=\sum_{j \in T_d(3)}w_j=3$, $\alpha_d(8)=\sum_{j \in T_d(8)}w_j=5$, and for any $i \in V\setminus\{3,8\}$, $\alpha_d(i)=0$ (as $i$ is a follower). Consider the set $C=\{3,5,7,8\}$. $T_d(8,C)$ (resp. $T_d(3,C)$) is the subtree rooted  in $8$ (resp. $3$) and  composed of voters $\{7,8\}$ (resp. $\{3\}$). Thus, $\alpha_{d,C}(3)=\sum_{j \in T_d(3, C)}w_j=1$, $\alpha_{d,C}(8)=\sum_{j \in T_d(8, C)}w_j=2$ and $\alpha_{d,C}(i)=0$ for $i \in \{5,7\}$, and then $\alpha_d(C)=\sum_{i \in C} \alpha_{d,C}(i)=3$. Also, $d^*_C(3)=3$, $d^*_C(7)=8$, $d^*_C(8)=8$ and $\hat{D}(C)=\{3,7,8\}$ as for any $i \in \{3,7,8\}$, $c_d(i,d^*_C(i)) \subseteq C$. Note that $5 \notin \hat{D}(C)$ as $c_d(5,8) \not \subseteq C$. Now we intend to compute $DB_8$ and $DB_6$. 

We first compute $DB_8$ by counting the coalitions $C \subseteq V\setminus\{8\}$ for which $8$ is a swing agent. 
Note that if $\{1,2,3\}\subseteq C$, then $8$ cannot be a swing agent for $C$. 
Second, if $\{1,2,3\}\cap C\in\{\{1,3\},\{2,3\}\}$, then $8$ will always be a swing agent for $C$. There are 32 such coalitions. 
Third, if $\{1,2,3\}\cap C = \{3\}$, then $8$ will be a swing agent for $C$ iff $7\in C$. There are 8 such coalitions. 
Last, if $3 \not\in (\{1,2,3\}\cap C)$, then $8$ will be a swing agent for $C$ iff $|C\cap\{4,6,7\}| \ge 2$. There are 24 such coalitions.
Hence $DB_8(V) = \frac{1}{2^{7}}\times 64=\frac{1}{2}$.

Now we compute $DB_6$. Note that in order for $6$ to be a swing agent in any coalition $C$, it is necessary that $\{7,8\}\subseteq C$. 
Hence, the coalitions $C$ for which $6$ is a swing agent are of the form $C = \{7,8\}\cup S$ where $S\subseteq \{1,2,5\}$. The number of such coalitions is 8. Hence, $DB_6=\frac{1}{2^{7}}\times 8=\frac{1}{16}$.

\begin{figure}[!h]
		\centering
		\begin{tikzpicture}
				\tikzset{vertex/.style = {shape=circle,draw = black,thick,fill = white}}
				\tikzset{edge/.style = {->,> = latex'}}
				\tikzset{edgebis/.style = {--}}
				
				\node[vertex] (8) at  (0,3) {$8$};
				\node[vertex] (7) at  (0,2) {$7$};
				\node[vertex] (6) at  (-.5,1) {$6$};
				\node[vertex] (5) at  (-1,0) {$5$};
				\node[vertex] (4) at (.5,1) {$4$};
				
				\node[vertex] (3) at  (2.5,3) {$3$};
				\node[vertex] (2) at  (2,2) {$2$};
				\node[vertex] (1) at  (3,2) {$1$};
				
				
				
				%edges
				\draw[edge] (7) to (8);
				\draw[edge] (6) to (7);
				\draw[edge] (5) to (6);
				\draw[edge] (4) to (7);
				
				\draw[edge] (1) to (3);
				\draw[edge] (2) to (3);
				
				\draw[edge,dotted,bend right] (6) to (5);
				\draw[edge,dotted,bend right] (7) to (4);
				\draw[edge,dotted,bend right] (2) to (7);
				\draw[edge,dotted,bend right] (3) to (2);
				\draw[edge,dotted,bend right] (3) to (8);
				
				\draw[edge,dotted,bend left] (1) to (4);
		\end{tikzpicture}

		\caption{ The delegation graph $H_d$ (dotted arcs are the other arcs of $D = (V,A)$) with the set of gurus $Gu_d=\{3,8\}$.} \label{figNotation}
	\end{figure}
\end{exmp}

In the upcoming section, we address the computational problem of computing the delegative Banzhaf and Shapley-Shubik indices of a given voter $i$.

==> old/Problem/researchquestions.tex <==
%\subsection{Research Questions}
%\begin{itemize}
%    \item upper and lower bounds on the changes in the individual player's power that can result from a change in quota ? which of two quotas make a voter more powerful ? Can we find the quota that minimizes the index of a voter, can it make it dummy ?
%\end{itemize}

==> old/RelatedWork.tex <==
\section{Related Work}\label{secRW}
Weighted voting games originated in the domain of cooperative game theory~\cite{chalkiadakis2011computational, chalkiadakis2016weighted}. 
Two well-known solutions to measure the voting power of an agent in a weighted voting game are the Shapley-Shubik and Banzhaf indices~\cite{banzhaf1964weighted, shapley1953value}. 
Both indices share several properties~\cite{dubey1979mathematical}. For instance, they both satisfy the well-known axioms \textit{Dummy Player}, \textit{Symmetry} and \textit{Additivity}. Several works characterize both indices in different ways which emphasize their differences~\cite{barua2005new, neyman1989uniqueness, shapley1953value, van2002axiomatization}. Computing the Shapley-Shubik and Banzhaf indices is \#P-Complete~\cite{deng1994complexity,prasad1990np}. 
However, Matsui and Matsui~\cite{matsui2000survey} showed that there exists pseudopolynomial algorithms that can compute the Shapley-Shubik and Banzhaf indices in time $O(n^3w_{\max})$ and $O(n^{2}w_{\max})$ respectively, where $n$ is the number of agents and $w_{\max}$ is the maximum weight of an agent. 
Several other works have been dedicated to the computation of these power indices, either to compute them exactly~\cite{brams1976power,conitzer2004computing,ieong2005marginal,ieong2006multi}, or approximately~\cite{bachrach2008approximating,fatima2008linear,fatima2010approximation,leech2003computing,mann1960values,merrill1982approximations,owen1988multilinear}. 
Moreover, several manipulation problems involving power indices have been investigated, as computing the quota maximizing or minimizing the power index of a specific voter~\cite{zick2011,zuckerman2012manipulating} or  determining the impact of splitting an agent in two~\cite{aziz2011false,felsenthal1998measurement,laruelle2005critical}.

Several works have studied the measurement of voters' relative importance in an LD election~\cite{boldi2009voting,boldi2011viscous,kling2015voting,zhang2020power}. %To the best of our knowledge, the idea of measuring the importance of voters in LD originated from the work by Boldi et. al~\cite{boldi2009voting} and Kling et. al~\cite{kling2015voting}. 
Boldi et al.~\cite{boldi2009voting,boldi2011viscous} proposed a way to measure the relative importance of each voter in a social network using a power index similar to PageRank. 
In their model, each voter can recommend one of her neighbor in the social network. 
The recommendations of the voters are then transitively delegated but are attenuated by using a multiplicative damping factor. 
The authors term the resulting system a viscous democracy election as the voting power does not flow completely but rather meets some resistance do to the damping factor. In this way, the model by Boldi et al.~\cite{boldi2009voting,boldi2011viscous} favors the voters who receive direct supports instead of more distant ones.
Kling et al.~\cite{kling2015voting} studied the behavior of voters using the LiquidFeedback software in the German Pirate Party. The authors studied the number and types of interactions with the software, the distribution in terms of number of delegations received per voter as well as the behavior of ``super-voters'' which receive a large number of delegations. The authors then apply several power indices from game theory (e.g., the Shapley-Shubik and Banzhaf indices) to analyze the power distribution in liquid democracy elections. This analyse led the authors to propose modifications to the existing power indices to fit better to the real world data they gathered. More precisely, the authors designed generalizations of the Banzhaf and Shapley-Shubik power indices which allow to model non-uniform distributions of approval rates\footnote{Stated otherwise, the assumption that voters vote with equal probability in favour or against a proposal is not made.}. Lastly, as detailed in the introduction, Zhang and Grossi~\cite{zhang2020power} have very recently proposed a formal way to measure the influence of voters in an LD election by introducing a variant of weighted voting games. This variant as well as the resulting power indices will be presented in Section~\ref{sec : Preliminaries}.

Other questions related to LD have been investigated. Several articles have investigated the stability of the delegation process in LD. This question was first studied by Bloembergen, Grossi and Lackner~\cite{bloembergen2019rational} and Escoffier, Gilbert and Pass-Lanneau~\cite{escoffier2018convergence,EscoffierGP20} by using standard concepts from game theory. Kavitha et al.~\cite{kavitha2020popular} also studied this problem but using popularity as the stability criterion. 
Christoff and Grossi~\cite{christoffbinary} studied other possible pitfalls of LD as delegation cycles or possible inconsistencies that can occur if voters should vote on different but connected issues. 
Brill and Talmon~\cite{brill2018pairwise} investigated a setting called \textit{pairwise liquid democracy}, in which each voter should provide a complete ranking over candidates. This work illustrated the difficulty of unraveling ballots arising from complex delegation processes, a problem that was tackled by Colley, Grandi and Novaro~\cite{colleysmart}. Kotsialou and Riley~\cite{kotsialou2018incentivising} attempted to incentive participation in the delegation/voting process in the LD setting using several delegation rules. The question of the expected accuracy of voters has been considered by Green-Armytage~\cite{green2005direct}, Kahng, Mackenzie and Procaccia~\cite{kahng2018liquid} as well as Caragiannis and Micha~\cite{caragianniscontribution}. Lastly, several articles considered a potential pitfall of LD being that some gurus could accumulate an undesirably high voting power~\cite{dey2020parameterized, golz2018fluid, kling2015voting}. The authors proposed optimization problems to mitigate this problem and obtained approximation and parameterized complexity results.
 

